Stochastic analysis of the Elo rating algorithm in round-robin tournaments

The Elo algorithm, renowned for its simplicity, is widely used for rating in sports tournaments and other applications. However, despite its widespread use, a detailed understanding of the convergence characteristics of the Elo algorithm is still lacking. Aiming to fill this gap, this paper presents a comprehensive (stochastic) analysis of the Elo algorithm, considering round-robin tournaments. Specifically, analytical expressions are derived describing the evolution of the skills and performance metrics. Then, taking into account the relationship between the behavior of the algorithm and the step-size value, which is a hyperparameter that can be controlled, design guidelines and discussions about the performance of the algorithm are provided. Experimental results are shown confirming the accuracy of the analysis and illustrating the applicability of the theoretical findings using real-world data obtained from SuperLega, the Italian volleyball league.

==> old/Analytical.tex <==
\section{Proposed stochastic analysis}\label{Sec:analysis}
In this section, a stochastic analysis of the Elo rating algorithm is presented. Specifically, we first introduce some statistical assumptions along with an approximate version of the rating algorithm, which are required to make the mathematical development tractable; next, mathematical expressions are derived to characterize the mean behavior of the skills, the mean-square deviation of the skills, the variance of the skills, and the mean behavior of the loss function.

\subsection{Assumptions}\label{Sec:assumptions}
%Since \eqref{eq:rating-sgd2} depends on realizations of random variables, it can only be analyzed in a probabilistic sense using expectations and this will be facilitated if all the other variables are treated as random as well.
Since the rating algorithm [given by \eqref{eq:rating-sgd2}] depends on the realizations of random variables, its analysis (in the stochastic sense) becomes feasible under the following assumptions:

First, although the sequence of scheduling vectors $\bx_k$ [see \eqref{eq:schedule_vector}] in round-robin tournaments is determined in advance, we assume that the indices $i_k$ and $j_k$ (which define $\bx_k$) are random, drawn uniformly and without repetition from the set $\set{1,\ld,M}$ (\ie each team plays at home and away against all the other teams with the same probability) so that\footnote{This can be approximately verified, for large $M$, by sampling twice (uniformly and without repetition) from set $\set{1,\ld,M}$.}
\begin{align} \label{eq:PR.schedules}
\nonumber
\PR{i_k = m} &= \PR{j_k = m} ,\quad \forall m\\
&= \frac{1}{M}
\end{align}
and
\begin{align} \label{eq:PR.schedules.cond}
\nonumber
\PR{j_k = n | i_k = m} &= \PR{i_k = n | j_k = m}, \quad \forall m \neq n\\
&= \frac{1}{M - 1}.
\end{align}
Thus, the correlation between the elements of $\bx_k$ can be expressed as
\begin{align} \label{eq:R.elements.generic}
\Ex[x_{k,m} x_{k,n}]
&=
\begin{cases}
\PR{i_k = m} + \PR{j_k = m}, &m = n\\
-\PR{i_k = m} \PR{j_k = n | i_k = m}  -\PR{j_k = m} \PR{i_k = n | j_k = m}, &\text{otherwise}
\end{cases}
\end{align}
which results [from \eqref{eq:PR.schedules} and \eqref{eq:PR.schedules.cond}] in
\begin{align} \label{eq:R.elements.uniform}
\Ex[x_{k,m} x_{k,n}]
&=
\begin{cases}
\displaystyle\frac{2}{M}, & m = n \\
-\displaystyle\frac{2}{M (M-1)},\quad  &\text{otherwise.}
\end{cases}
\end{align}
So, the autocorrelation matrix of $\bx_k$ can be compactly represented as
\begin{align}
\label{covariance.matrix}
\nonumber
\matR &= \Ex[\bx_k\bx_k\T]\\
      &= \frac{2}{M-1} \left(\bI - \frac{1}{M}\bone\bone\T\right)
\end{align}
which holds as $M \rightarrow \infty$.

Second, we assume that the Bradley-Terry model \eqref{Pr.y.1} describes exactly the distribution of $y_k$ when conditioned on hypothetical ``true'' skills $\btheta^*= [\theta_1^*,\ld,\theta_M^*]\T$, \ie
\begin{align} \label{Pr.y.star}
\PR{y_k=1|\btheta^*} &= \sigma(z_k^* + \eta)
\end{align}
in which
\begin{align*}
z_k^* &= \theta_{i_k}^* - \theta_{j_k}^*\\
&= \bx_k\T \btheta^* \numberthis \label{z_k*}
\end{align*}
with the scheduling vector $\bx_k$ given by \eqref{eq:schedule_vector}. Note in \eqref{Pr.y.star} that we have already assumed $s=1$ for simplicity.



%Although not necessary to perform the inference via \eqref{eq:rating-sgd2}, this assumption is important to simplify the analysis.


%Since there are in general many average teams (with skills close to zero), a small number of teams with very high skills, and a small number of poorly performing teams, the true skills vector $\btheta^*$ is assumed to be obtained from a Gaussian distribution with zero-mean and variance $v$ (as already appeared explicitly in \cite[Sec.~4.1]{Bock72} as well as in \cite{Gramacy13} when dealing with regularized rating problems). A direct consequence of this Gaussian model of the skills is that $v$ is the sole parameter which controls the uncertainty of the outcomes $y_k$. Particularly, large $v$ implies that the difference of skills between opponents $z_k$ [see \eqref{z_k}] is likely to be large and then the game result $y_k$ [generated randomly according to \eqref{Pr.y.1}] will be quasi-deterministic, \ie either $\PR{y_k=1|z_k}\approx 1$ or $\PR{y_k=1|z_k}\approx 0$. On the other hand, small $v$ leads to $z_k \approx 0$ which means that the uncertainty of the results conditioned on the skills is high, \ie $\PR{y_k=1|z_k} \approx 0.5$. As practical examples, consider the following two scenarios: i) in a professional league, where the teams are expected to perform similarly, a significant uncertainty in the game results is then modeled by small $v$; ii) for international tournaments/championships, where large disparities in the quality of players are observed, games between the strongest and the weakest teams are usually quite easy to predict, implying large $v$. Thereby, by changing $v$, we refer to different contexts in which the rating algorithm may be used.

Third, to remove the dependence on unknown $\btheta^*$, we assume that its elements are drawn from a Gaussian distribution with zero mean and variance $v$ as in \cite[Sec.~4.1]{Bock1972} and \cite{Gramacy13}. 
%\sout{A corollary assumption is that, if the number of teams $M$ is sufficiently large we may replace any function of $\btheta^*$ with its expectation exploiting the principle of ergodicity.}
As a consequence of this assumption on $\btheta^*$, the characteristics of a given tournament are uniquely defined by $v$ whose value refers to different contexts of competition. In particular, for $\eta=0$, large $v$ implies that the difference in skills between opponents $z_k^*$ [see \eqref{z_k*}] is likely to be large and, then, the game result $y_k$ [generated randomly according to \eqref{Pr.y.star}] will be quasi-deterministic, \ie either $\PR{y_k=1|\btheta^*} \approx 1$ or $\PR{y_k=1|\btheta^*} \approx 0$. On the other hand, a small $v$ leads to $z_k^* \approx 0$ which means that the uncertainty of the results conditioned on skills is high, \ie $\PR{y_k=1|\btheta^*} \approx 0.5$. As practical examples, consider that i) in a professional league, where teams are expected to perform similarly, a significant uncertainty in game results is then modeled by small $v$; while ii) for international tournaments/championships, where large disparities in player quality are observed, games between the strongest and weakest teams are usually quite easy to predict, which implies large $v$. 



% \ls{The meaning of large/small variance $v$ must be defined with respect to the scale, $s$ which, as we already said, is set to $s=1$ in our work. A a rule of thumb, we then say that $v=0.1$ is small and $v=1$ is large.}

Note that the assumptions introduced here regarding the scheduling vector $\bx_k$ and the vector of true skills $\btheta^*$ are somehow strong and debatable; nevertheless, such assumptions are required to make mathematical development tractable, leading to satisfactory results (as shown in Section~\ref{Sec:experimental_results}).

%In fact, the assumptions introduced here regarding the scheduling vector $\bx_k$ and the existence of the skills $\btheta^*$ are debatable but, introduced to make the mathematical development tractable, they lead to satisfactory results (as shown later in \secref{Sec:experimental_results}).

\subsection{Quadratic approximation of the rating problem}\label{Sec:approx.likelihood}

% \ls{To simplify the  analysis of \eqref{eq:rating-sgd2} let us approximate \eqref{eq:loss_k} using Taylor series centered at $\btheta^*$ as}

% \dz{A direct stochastic analysis of \eqref{eq:rating-sgd2} is very difficult, since it requires isolating $\btheta_k$ in the \gls{rhs} of the equation. This is not possible to be done analytically, since the term $\sigma(\bx\T\btheta_k+\eta)$ makes \eqref{eq:rating-sgd2} a transcendental equation.}

Analyzing \eqref{eq:rating-sgd2} is challenging due to the impossibility of isolating $\btheta_k$ on the \gls{rhs}, since the presence of the term $\sigma(\bx\T\btheta_k+\eta)$ makes the equation transcendental. So, aiming to make the mathematical development tractable, let us approximate \eqref{eq:loss_k} using a second-order Taylor series expansion around $\btheta^*$ as
\begin{align*}
\tilde{\ell}_k(\btheta) &= \ell_k(\btheta^*) + [\nabla \ell_k(\btheta^*)]\T (\btheta - \btheta^*) + \frac{1}{2} (\btheta - \btheta^*)\T \nabla^2 \ell_k(\btheta^*) (\btheta - \btheta^*)\\
\numberthis \label{eq:cost-taylor}
&= \ell_k(\btheta^*) + g_k\bx\T_k (\btheta - \btheta^*) + \frac{1}{2} h_k(\btheta - \btheta^*)\T \bx_k\bx_k\T (\btheta - \btheta^*)
\end{align*}
with
\begin{align}
\label{eq:gradient-optimal}
g_k &= y_k - \sigma(\bx_k\T\btheta^*+\eta)
\end{align}
and
\begin{align}
\label{eq:hessian-optimal2}
h_k &= \mcL(\bx_k\T \btheta^*+\eta)
\end{align}
where
\begin{align*}
\mcL(z) &= \sigma(z) [1 - \sigma(z)]\\
\numberthis \label{logistic.pdf}
&= \sigma(z) \sigma(-z)
\end{align*}
is the \gls{pdf} of the logistic distribution. Thereby, \eqref{eq:rating-sgd2} can be simplified using \eqref{eq:cost-taylor} as
\begin{align*}
%\label{eq:sgd-taylor}
\btheta_{k+1} 
&\approx \btheta_{k}-\beta\nabla\tilde\ell(\btheta_k)\\
\numberthis \label{eq:sgd-taylor.2}
&=\btheta_{k} - \beta h_k \bx_k\bx_k\T (\btheta_k - \btheta^*) + \beta g_k \bx_k.
\end{align*}

%Note that this approximation \dz{, which places us in the realm of adaptive filtering theory \cite{Haykin2002,book:Boroujeny},} is required since \eqref{eq:rating-sgd2} cannot be directly expressed as a function of \eqref{tilde.btheta}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Mean behavior of the skills}\label{Sec:skills.mean}

To characterize the mean behavior of the skills, we start by taking the expected value of both sides of \eqref{eq:sgd-taylor.2} such that
\begin{align} \label{eq:mean-weight}
\Ex[\btheta_{k+1}] &= \Ex[\btheta_k] - \beta \Ex[h_k \bx_k\bx_k\T \btheta_k] + \beta \Ex[h_k \bx_k\bx_k\T] \btheta^* + \beta \Ex[g_k \bx_k].
\end{align}
Then, recalling that $\bx_k$ is statistically independent from $\btheta_k$, the second and third-terms of the \gls{rhs} of \eqref{eq:mean-weight} can be rewritten as
\begin{align*}
\Ex[h_k \bx_k\bx_k\T \btheta_k] &= \Ex[h_k \bx_k\bx_k\T]\Ex[\btheta_k]\\
\numberthis \label{eq:independence-assumption}
&= \matH \Ex[\btheta_k]
\end{align*}
and
\begin{align} \label{eq:H_star}
\Ex[h_k \bx_k\bx_k\T] \btheta^* = \matH\btheta^*
\end{align}
where
\begin{align}\label{matrix_H}
\matH = \tr{diag}(\matH' \bone) - \matH'
\end{align}
is the Fisher information matrix \cite[Sec.~3.7]{book:mkay} whose elements are given by
\begin{align}
[\matH']_{m,n} &= \frac{1}{M(M-1)} [ \mcL(\theta^*_{m}-\theta^*_{n}+\eta)+\mcL(\theta^*_{n}-\theta^*_{m}+\eta) ].
\end{align}
In turn, due to the orthogonality principle \cite[Sec.~3.3]{book:Boroujeny}, the last term of the \gls{rhs} of \eqref{eq:mean-weight} reduces to
\begin{align*}
\Ex[g_k \bx_k] 
&= \Ex_{\bx_k,y_k}\{ [y_k - \sigma(\bx_k\T\btheta^* + \eta)] \bx_k \}\\
\numberthis \label{eq:g_kx_k}
&= \Ex_{\bx_k}\{ [\sigma(\bx_k\T \btheta^* + \eta)  - \sigma(\bx_k\T \btheta^* + \eta)] \bx_k \}\\ 
&= \bzero.
\end{align*}
Finally, substituting \eqref{eq:independence-assumption}, \eqref{eq:H_star}, and \eqref{eq:g_kx_k} into \eqref{eq:mean-weight}, we have
\begin{align}
\label{eq:weight-behavior}
\Ex[\btheta_{k+1}] = \Ex[\btheta_k] - \beta \matH (\Ex[\btheta_k] - \btheta^*).
\end{align}


Since \eqref{eq:weight-behavior} depends on the complete knowledge of $\btheta^*$ to determine $\matH$, we resort to the ergodicity argument to approximate the sample statistics of $\btheta^*$ [in \eqref{matrix_H}] to its expected value (which holds for a large number of players $M$). Thereby, $\matH$ can now be replaced by its expected value obtained from the probability distribution of $\btheta^*$, \ie
\begin{align*}
\matH &\approx \Ex_{\btheta^*}[\matH]\\
\numberthis \label{eq:H_approximation}
&=\ov{h} \matR
\end{align*}
with
\begin{align*}
\ov{h}
&= \Ex_{\btheta^*,\bx_k}[\mathcal{L}(\bx_k\T \btheta^* + \eta)]\\
&\approx \frac{\sqrt{\pi}}{2} \mcN(\eta;0,2v + 2)\\
\numberthis \label{mean-h_k}
&= \frac{1}{4} \frac{1}{\sqrt{v + 1}} \exp\left[\frac{-\eta^2}{4(v + 1)}\right]
\end{align*}
(for details, see \ref{Appendix.Expectation}). Next, substituting \eqref{covariance.matrix} and \eqref{eq:H_approximation} into \eqref{eq:weight-behavior}, and recalling the well-known property of the Elo algorithm which establishes that the sum of the skills does not change over time \cite[Ch.~5]{Langeville12_book} given the symmetrical nature of the ratings' update and fixed set of players, the mean behavior of each individual skill can be expressed as
\begin{align*}
% \label{Ex.tilde.theta.k.1}
% \Ex[\theta_{k+1,m}] &\approx \Ex[\theta_{k,m}] - \beta\ov{h} \Ex\{[\matR(\btheta_k-\btheta^*)]_m\}\\
\Ex[\theta_{k+1,m}] &\approx \Ex[\theta_{k,m}] - \frac{2 \beta \ov{h}}{M-1} \left( \Ex[\theta_{k,m}] - \theta^*_m - \frac{1}{M} \sum_{i=1}^{M}
\Ex[\theta_{k,i} - \theta^*_i] \right)\\
% &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\theta_{k,m}] + \frac{2 \beta \ov{h}}{M-1} \theta^*_m\\
\numberthis \label{eq:E[theta_k+1]}
&= \alpha_1 \Ex[\theta_{k,m}] + (1 - \alpha_1) \theta^*_m
\end{align*}
where
\begin{align} \label{eq:alpha_1}
\alpha_1 &= 1 - \frac{2 \beta \ov{h}}{M-1}
\end{align}
characterizes the convergence speed of the skills in the mean sense.

Therefore, since we assumed $\btheta_0 = \bzero$ in \eqref{eq:rating-sgd2}, \eqref{eq:E[theta_k+1]}  can be compactly written as 
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{eq:skill-behavior}
\Ex[\theta_{k,m}] &=  (1 - \alpha_1^k)\theta^*_m
\end{empheq}
which converges to $\btheta^*$ as $k$ increases if $|\alpha_1|<1$, \ie
\begin{align}
\label{lim.k.Ex.theta}
    \lim_{k\rightarrow\infty} \Ex[\theta_{k,m}] &=  \theta^*_m.
\end{align}
Based on \eqref{eq:skill-behavior}, the evolution of the skills can be predicted (as illustrated in Section~\ref{Sec:experimental_results}), converging to the ``true skills" at an exponential rate \cite[Theorem~2.2]{jabin2015}.

% \ls{I find the parenthesis around the statements "as shown in Sec. 5" confusing. Here you show the derivation, Sec. 5 is about the numerical examples. So the fact that something can be predicted is shown here and not in Sec. 5 which is rather used to show the example which are in agreement with out results. Maybe the statement "as illustrated in Sec. 5" would be better. }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mean-square deviation of the skills}\label{Sec:skills.variance}


% \sout{\cred{let's always use brackets around the expression we calculate the expectation of, maybe big brackets $\big[\cd[\cd]\cd\big]$ if the brackets are already inside.}}

Even when \eqref{lim.k.Ex.theta} is satisfied, it is still important to assess the uncertainty related to the estimate of skills, \ie the random fluctuations around the mean value. To this end, we define the \gls{msd} of the skills as
\begin{align}\label{eq:skills.variance0}
\ov{d}_k = \Ex[\tilde\btheta_k\T\tilde\btheta_k]
\end{align}
where
\begin{align}
\label{tilde.btheta}
\tilde\btheta_k &= \btheta_k - \btheta^*
\end{align}
represents the estimation error of the skills. Then, rewriting \eqref{eq:sgd-taylor.2} in terms of $\tilde\btheta_k$ as %[given by \eqref{tilde.btheta}] as
\begin{align}\label{eq:param-error}
\tilde\btheta_{k+1} &= 
(\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \bx_k
\end{align} 
determining the inner product $\tilde\btheta_k\T\tilde\btheta_k$, noting that $\bx_k\T\bx_k = 2$, and taking the expected value of both sides of the resulting expression, we get the following:
\begin{equation}
\label{eq:skills.variance1}
\begin{aligned}
\ov{d}_{k+1} &=  \ov{d}_k - 2\beta  \Ex[ h_k \tilde\btheta_k\T \bx_k\bx_k\T \tilde\btheta_k ] + 2\beta^2 \Ex[ h_k^2 \tilde\btheta_k\T \bx_k  \bx_k\T \tilde\btheta_k] \\
& + 2 \beta  \Ex[ g_k \bx_k\T \tilde\btheta_k] - 4\beta^2 \Ex[ g_k h_k \bx_k\T \tilde\btheta_k ] + 2\beta^2 \Ex[ g_k^2].
\end{aligned}
\end{equation}

Now, using the same approach as in \eqref{eq:H_approximation}, we approximate the second and third terms of the \gls{rhs} of \eqref{eq:skills.variance1} as
\begin{align}\label{eq:expected_value1}
\Ex[ h_k \tilde\btheta_k\T \bx_k\bx_k\T \tilde\btheta_k ] \approx \ov{h} \Ex[ \tilde\btheta_k\T \matR \tilde\btheta_k ]
\end{align}
and
\begin{align}\label{eq:expected_value2}
\Ex[ h_k^2 \tilde\btheta_k\T \bx_k\bx_k\T \tilde\btheta_k ] \approx \ov{h^2} \Ex[ \tilde\btheta_k\T \matR \tilde\btheta_k ]
\end{align}
in which $\ov{h}$ is defined in \eqref{mean-h_k},
%\cred{we have to decide if we use comma or the semi-colon to separate the variables in subscript of the expectation; I suggest comma, \ie $\Ex_{\btheta^*,\bx_k}[\cd]$}
\begin{align*}\label{mean-h_k^2}
\ov{h^2} &= \Ex_{\btheta^*,\bx_k}[\mcL^2(\bx_k\T \btheta^* + \eta)]\\
&\approx \frac{\sqrt{2\pi}}{16} \mcN(\eta;0,2v + 1)\\
&= \frac{1}{16} \sqrt{\frac{1}{2v + 1}} \exp{\left[\frac{-\eta^2}{2 (2v + 1)}\right]} \numberthis
\end{align*}
(for details, see \ref{Appendix.Expectation}), while
\begin{align*}
\Ex[ \tilde\btheta_k\T \matR \tilde\btheta_k ] &= \frac{2}{M-1} \Ex[ \tilde\btheta_k\T \tilde\btheta_k ] - \frac{2}{M(M-1)} \Ex[ \tilde\btheta_k\T \bone\bone\T \tilde\btheta_k ]\\
\label{eq:theta_R_theta}
&= \frac{2}{M-1} \ov{d}_k \numberthis
\end{align*}
since $\bone\T \tilde\btheta_k = 0$. Next, invoking the orthogonality principle \cite[Sec.~3.3]{book:Boroujeny}, it is possible to show that the fourth and fifth terms of the \gls{rhs} of \eqref{eq:skills.variance1} reduce to
\begin{align}
\Ex[ g_k h_k \bx_k\T \tilde\btheta_k ] &= 0
\end{align}
and
\begin{align} \label{eq:ortho-g_k}
\Ex[ g_k \bx_k\T \tilde\btheta_k] &= 0.
\end{align}
While, the last term of the \gls{rhs} of \eqref{eq:skills.variance1} is derived from \eqref{eq:gradient-optimal} as
\begin{align*}
\Ex[ g_k^2 ] &= \Ex_{\btheta^*,\bx_k,y_k}\{ [y_k - \sigma(\bx_k\T\btheta^* + \eta)]^2 \} \\
&= \Ex_{\btheta^*,\bx_k,y_k}[y_k^2 -2y_k\sigma(\bx_k\T\btheta^* + \eta) + \sigma^2(\bx_k\T\btheta^* + \eta) ] \\
% &= \Ex_{\btheta^*;\bx_k}[\sigma(\bx_k\T\theta^* + \eta) - 2\sigma^2(\bx_k\T\theta^* + \eta) + \sigma^2(\bx_k\T\theta^* + \eta)]\\
&= \Ex_{\btheta^*,\bx_k}\{ \sigma(\bx_k\T\btheta^* + \eta)[1 - \sigma(\bx_k\T\btheta^* + \eta)] \}\\
&= \Ex_{\btheta^*,\bx_k}[\mcL(\bx_k\T \btheta^* + \eta)]\\
&= \ov{h}. \numberthis \label{eq:expected_value_gk}
\end{align*}

Finally, substituting \eqref{eq:expected_value1}-\eqref{eq:expected_value_gk} into \eqref{eq:skills.variance1}, we obtain
\begin{align}\label{eq:skills.variance4}
\ov{d}_{k+1} &= \alpha_2\ov{d}_k + 2\beta^2 \ov{h}
\end{align}
where
\begin{align}\label{eq:alpha_2}
\alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})
\end{align}
represents the convergence speed in the mean-square sense. Alternatively, when $|\alpha_2| < 1$, \eqref{eq:skills.variance4} can be rewritten in a more convenient form as
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{eq:v_k-final}
\ov{d}_k  = \alpha_2^k (\ov{d}_0 - \ov{d}_{\infty}) + \ov{d}_{\infty}
\end{empheq}
where 
\begin{align} \label{eq:msd_0}
\ov{d}_0 &= M v
\end{align}
due to the initialization considered in \eqref{eq:rating-sgd2} and
\begin{align*}\label{eq:msd_inf}
\ov{d}_{\infty} &= \frac{2 \beta^2 \ov{h}}{1 - \alpha_2}\\
\numberthis
&= \frac{\beta \ov{h} (M-1)}{2(\ov{h} - \beta \ov{h^2})}
\end{align*}
comes from \eqref{eq:skills.variance4} by assuming that $d_\infty=d_{k+1}=d_k$. Therefore, from \eqref{eq:v_k-final}, the \gls{msd} can be predicted (as illustrated in Section~\ref{Sec:experimental_results}).


\subsection{Variance of the skills} \label{Sec:Variance.skills}

To have a better understanding of the statistics of skills, let us use the well-known bias-variance decomposition (see \cite[Sec.~4.4]{aldous2017}) to rewrite the \gls{msd} [defined in \eqref{eq:skills.variance0}] as
\begin{align*}
\ov{d}_k &= \Ex[(\tilde\btheta_k -\Ex[\tilde\btheta_k])\T (\tilde\btheta_k -\Ex[\tilde\btheta_k])] +  \Ex[\tilde\btheta_k\T] \Ex[\tilde\btheta_k]\\
&= \ov\omega_k + \ov{b}_k \numberthis \label{bias.variance.decomposition}
\end{align*}
where
\begin{align}
\label{skills.bias}
\ov{b}_k &= \alpha_1^{2k} \ov{d}_0
\end{align}
is the squared estimation bias obtained from \eqref{eq:skill-behavior}, and
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
% \ov\omega_k &= \ov{d}_k - \ov{b}_k\\
% \ov\omega_k = \alpha_2^k(\ov{d}_0 - \ov{d}_{\infty}) +\ov{d}_{\infty} - \alpha_1^{2k} \ov{d}_0 
\label{variance.skills}
\ov\omega_k =  (\alpha_2^k - \alpha_1^{2k}) \ov{d}_0 + (1-\alpha_2^k)\ov{d}_{\infty} 
\end{empheq}
is the total variance (\ie the sum of all variances) derived from \eqref{eq:v_k-final} and \eqref{skills.bias}. Note from \eqref{bias.variance.decomposition}-\eqref{variance.skills} that the bias-variance trade-off is actually a function of $k$. In particular, for $k=0$, the total variance is null (\ie $\ov\omega_0=0$) and the squared estimation bias is at its maximum (\ie $\ov{b}_0 = \ov{d}_0$). On the other hand, as $k$ increases, the squared estimation bias tends to zero (\ie $\ov{b}_\infty = 0$) and the total variance reaches its maximum (\ie $\ov\omega_\infty = \ov{d}_\infty$).

% by assuming that $\alpha_2\approx \alpha_1^2$ which holds for sufficiently small $\beta$
% \begin{align}
% \label{variance.skills.approximation}
% \ov\omega_k \approx (1-\alpha_2^k)\ov{d}_{\infty}
% \end{align}

% \begin{align}
% \ov\omega_k = (\alpha_2^k - \alpha_1^{2k}) \ov{d}_0 + (1-\alpha_2^k)\ov{d}_{\infty} \label{variance.skills}
% \end{align}


% allows us to clearly emphasize how the bias-variance trade-off is actually a function of $k$: for $k=0$ the variance is null, $\ov\omega_0=0$ but the squared bias is at the maximum $\ov{d}_0$. Increasing $k$, the bias goes to zero but the variance increases to the final value $\ov\omega_\infty = \ov{d}_\infty$.



% % \begin{align}
% % \label{bias.variance.decomposition}
% % \ov{d}_k &= \Ex[ \tilde\btheta_k\T\tilde\btheta_k ]
% % = \Var[\tilde\btheta_k] + \Ex[\tilde\btheta_k]\T \Ex[\tilde\btheta_k] \\
% % &= \ov\omega_k + b_k,
% % \end{align}

% \dz{
% \begin{align}
% \label{bias.variance.decomposition}
% \ov{d}_k &= \Ex[ \tilde\btheta_k\T \tilde\btheta_k ]\\
% &= \Tr\{\Var[\tilde\btheta_k]\} + \Ex[\tilde\btheta_k]\T \Ex[\tilde\btheta_k]\\
% &= \ov\omega_k + b_k,
% \end{align}
% where
% \begin{align}
% \label{skills.bias}
% b_k &= \Ex[\tilde\btheta_k]\T \Ex[\tilde\btheta_k]\\
% &= \alpha_1^{2k} \ov{d}_0
% \end{align}
% is the squared estimation bias obtained from \eqref{eq:skill-behavior}, and the estimate's total variance (\ie the sum of all variances) is given by
% \begin{align}
% \label{variance.sills}
% \ov\omega_k &= \Tr\{\Var[\tilde\btheta_k]\}\\
% &= \ov{d}_k - b_k\\
% \label{variance.sills.2}
% &=
% \alpha_2^k(\ov{d}_0 - \ov{d}_{\infty}) +\ov{d}_{\infty}
% - \alpha_1^{2k} \ov{d}_0 \\
% \label{variance.skills.approximation}
% &\approx
% (1-\alpha_2^k)\ov{d}_{\infty},
% \end{align}
% where \eqref{variance.sills.2} is obtained using \eqref{eq:v_k-final} together with \eqref{skills.bias}, and \eqref{variance.skills.approximation} assumes that $\alpha_2\approx \alpha_1^2$. The latter holds for sufficiently small $\beta$ and allows us to clearly emphasize how the bias-variance trade-off is actually a function of $k$: for $k=0$ the variance is null, $\ov\omega_0=0$ but the squared bias is at the maximum $\ov{d}_0$. Increasing $k$, the bias goes to zero but the variance increases to the final value $\ov\omega_\infty = \ov{d}_\infty$.
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mean behavior of the loss function}\label{Sec:loss.mean}

Since the loss function is our performance criterion, here we derive an expression characterizing its behavior in the mean sense. To this end, let us substitute \eqref{eq:gradient-optimal} and \eqref{eq:hessian-optimal2} into  \eqref{eq:cost-taylor}, take the expected value of both sides of the resulting expression, and recall \eqref{eq:ortho-g_k}, so that 
\begin{align*}
\ov\ell_k &= \Ex[\tilde\ell_k(\btheta_k)]\\
% &= \Ex[\ell_k(\btheta^*)] + \frac{1}{2} \Ex[\tilde\btheta_k\T \matH \tilde\btheta_k]\\
&= \Ex[\ell_k(\btheta^*)] + \frac{1}{2} \Ex[h_k \tilde\btheta_k\T \bx_k\bx_k\T \tilde\btheta_k].
\label{eq:loss-behavior0}\numberthis
\end{align*}
Next, using the ergodicity argument along with the derivations presented in \ref{Appendix.Expectation}, the first term of the \gls{rhs} of \eqref{eq:loss-behavior0} can be determined as
\begin{align*}\label{eq:l_min}
\ov\ell_{\rm min} &= \Ex_{\btheta^*,\bx_k,y_k}[\ell_k(\btheta^*)]\\
&= \Ex_{\btheta^*,\bx_k,y_k}\{-y_k \ln[\sigma(\bx_k\T \btheta^* + \eta)] - (1 - y_k) \ln[\sigma(-\bx_k\T \btheta^* + \eta)] \}\\
&= \Ex_{\btheta^*,\bx_k}\{ -\sigma(\bx_k\T \btheta^* + \eta)\ln[\sigma(\bx_k\T \btheta^* + \eta)] - \sigma(-\bx_k\T \btheta^* + \eta)\ln[\sigma(-\bx_k\T \btheta^* + \eta)] \}\\
&\approx 2\ln(2)\sqrt{2\ln(2)\pi}\ \mcN(\eta;0,2v + 4\ln(2))\\
&= \ln(2) \sqrt{\frac{2\ln(2)}{v + 2\ln(2)}} \exp{\left[\frac{-\eta^2}{4v + 8\ln(2)}\right]} \numberthis
\end{align*}
representing a lower bound on the mean of the loss function. In turn, the second term of the \gls{rhs} of \eqref{eq:loss-behavior0} can be derived from \eqref{eq:expected_value1} and \eqref{eq:theta_R_theta} as 
\begin{align}
\label{eq:l_ex} \nonumber
\ov\ell_{{\rm ex},k} &\approx \frac{\ov{h}}{2} \Ex[\tilde\btheta_k\T \matR \tilde\btheta_k]\\
&= \frac{\ov{h}}{M-1} \ov{d}_k
\end{align}
characterizing the mean excess-loss due to %the randomness in $\tilde\btheta_{k}$ caused by 
the \gls{sg} optimization algorithm, which is a linear function of $\ov{d}_k$. Therefore, using \eqref{eq:l_min} and \eqref{eq:l_ex}, the mean of the loss function can be predicted through
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{eq:loss-behavior}
\ov\ell_k &\approx \ov\ell_{\rm min} + \ov\ell_{{\rm ex},k}
\end{empheq}
(as we illustrate in Section~\ref{Sec:experimental_results}). 

==> old/Appendices.tex <==
\appendix
% \titleformat{\section}[block]{\bfseries}{\appendixname\\}{1em}{}
% \titleformat{\section}[block]{\bfseries}{\appendixname\\}{1em}{}
% \titleformat{\section}{\normalfont\bfseries}{}{0em}{}
% \titleformat{\chapter}{\normalfont\bfseries}{}{0em}{}

% \section{\normalfont\it Determination of \eqref{mean-h_k}, \eqref{mean-h_k^2}, and \eqref{eq:l_min}}\label{Appendix.Expectation}

\section{\normalfont\it Determination of \eqref{mean-h_k}, \eqref{mean-h_k^2}, and \eqref{eq:l_min}}\label{Appendix.Expectation}

We show how the Laplace approximation \cite[Ch.~5]{rdpeng-advstatcomp-online} can be applied to calculate the expected values in \eqref{mean-h_k}, \eqref{mean-h_k^2}, and \eqref{eq:l_min}], which involve a random variable of the form $f(z)$, with $f(\,\cdot\,)$ being a strictly positive, twice-differentiable, and absolutely integrable function, while $z$ is a Gaussian random variable with mean $\mu_z$ and variance $v_z$. Thereby, using the definition of expected value \cite[]{Therrien1992DRS}, we can write
\begin{align*}\label{log[f(z)]}
\Ex[f(z)] &= \int f(z) \mcN(z;\mu_z,v_z) \dd z\\
            &= \int \e^{\ln[f(z)]} \mcN(z;\mu_z,v_z) \dd z.\numberthis
\end{align*}
Next, expanding $\ln[f(z)]$ through Taylor series around $z=0$, \eqref{log[f(z)]} can be approximated to
\begin{align}\label{taylor_log[f(z)]}
\Ex[f(z)] &\approx\int \e^{\ln[f(0)] + [f'(0)/f(0)] z + \frac{1}{2}\{ f''(0)/f(0)-[f'(0)/f(0)]^2 \}z^2} \mcN(z;\mu_z,v_z) \dd z.
\end{align}
Then, assuming that $f(z)$ reaches its maximum at $z=0$ such that $f'(0) = 0$, \eqref{taylor_log[f(z)]} reduces to
\begin{align}\label{taylor_simplified}
\Ex[f(z)] &=f(0) \int \e^{\frac{1}{2} [f''(0)/f(0)] z^2} \mcN(z;\mu_z,v_z) \dd z.
\end{align}
Alternatively, since the exponential term resembles Gaussian \gls{pdf}, we can rewrite \eqref{taylor_simplified} as
\begin{align}\label{prod.Gaussian}
\Ex[f(z)] &=f(0) \sqrt{2\pi v_f}\int \mcN(z;0,v_f)\mcN(z;\mu_z,v_z) \dd z
\end{align}
in which
\begin{align}
v_f = -\frac{f(0)}{f''(0)}.
\end{align}
%\dz{Maybe comment on $z_k^*$ \eqref{z_k*} here:} 
Finally, recalling our assumption about the vector of true skills $\btheta^*$ (see Section~\ref{Sec:assumptions}) which implies that $\mu_z = \eta$ and $v_z=2v$, \eqref{prod.Gaussian} becomes
\begin{align*}
\Ex[f(z)] &\approx f(0)\sqrt{2\pi v_f} \mcN(0;\mu_z,v_z + v_f) \\
% &= f(0) \sqrt{\frac{v_f}{v_z + v_f}} \exp{\left[\frac{-\mu_z^2}{2 (v_z + v_f)}\right]}\\
&= f(0) \sqrt{\frac{v_f}{2v + v_f}} \exp{\left[\frac{-\eta^2}{2 (2v + v_f)}\right]}. \numberthis
\end{align*}
Note that some pre-calculated values of $v_f$ and $f(0)$ used here to calculate \eqref{mean-h_k}, \eqref{mean-h_k^2}, and \eqref{eq:l_min} are presented in Table \ref{tab:appendix.a} for ease of use.

\begin{table}[!ht]
\centering
\caption{Identities used in the derivations for different functions $f(z)$.}
\label{tab:appendix.a}
\medskip
\begin{tabular}{@{}ccc@{}}
\toprule
$f(z)$ & $v_f$ & $f(0)$\\ 
\midrule
$\mcL(z)$                                          & $2$         & $1/4$      \\
$\mcL^2(z)$                                        & $1$         & $1/16$     \\
$-\sigma(z)\ln[\sigma(z)] - \sigma(-z)\ln[\sigma(-z)]$ & $4\ln(2)$ & $\ln(2)$\\ \bottomrule
\end{tabular}
\end{table}


\section{\normalfont\it Determination of \eqref{eq:optimum_step}}\label{Appendix.Step}

% An optimum value for the step size $\beta$, considering a particular number of games $k$, can be determined to minimize \eqref{eq:v_k-final} [or, equivalently, the mean loss \eqref{eq:loss-behavior}]; specifically,
% \begin{equation}
% \beta_{{\rm o}, k} = \argmin_{\beta}\; \ov{d}_k.
% \end{equation}

%we need to solve the following optimization problem:

% Since a closed-form solution for \eqref{eq:optimum-beta} cannot be straightforwardly obtained for an arbitrary $k$, we derive here an approximate solution 

To derive an approximate solution for \eqref{eq:optimum-beta}, we resort to the Taylor series to expand \eqref{eq:v_k-final} around $\beta=0$, so that
\begin{align} \label{dk-taylor}
\ov{d}_k &\approx \ov{d}_k\Big|_{\beta=0} + \beta \left( \frac{\partial \ov{d}_k}{\partial \beta} \Big|_{\beta=0} \right) + \frac{1}{2} \beta^2 \left( \frac{\partial^2 \ov{d}_k}{\partial \beta^2} \Big|_{\beta=0} \right) 
\end{align}
in which
\begin{align} \label{dk-diff1}
\frac{\partial \ov{d}_k}{\partial \beta} \Big|_{\beta=0} &= -\frac{4 k \ov{h} M v}{M-1}
\end{align}
and
\begin{align} \label{dk-diff2}
    \frac{\partial^2 \ov{d}_k}{\partial \beta^2} \Big|_{\beta=0} = \frac{8 k \ov{h} M v}{M-1} \left[ \frac{2 \ov{h} (k - 1)}{M - 1} + \frac{\ov{h^2}}{\ov{h}} + \frac{1-1/M}{2 v} \right].
\end{align}
So, substituting \eqref{dk-diff1} and \eqref{dk-diff2} into \eqref{dk-taylor},  differentiating the resulting expression with respect to $\beta$, equating it to zero, and solving for $\beta$, one gets
\begin{align} \label{beta-taylor}
\beta_{\tr{o},k} &\approx \frac{1}{2} \left[ \frac{(1 - 1/M)}{2v} + \frac{\ov{h^2}}{\ov{h}} + \frac{2 \ov{h} (k - 1)}{M - 1} \right]^{-1}.
\end{align}
Next, in order to evaluate the accuracy of the approximate solution obtained, Fig.~\ref{fig:optimum_taylor} plots the results obtained from \eqref{beta-taylor} against those coming from the numerical solution of \eqref{eq:optimum-beta} as a function of $k$, considering different values of $v$ with $M=15$ and $\eta=0$. By doing so, we see that \eqref{beta-taylor} exhibits an important mismatch compared to the numerical results. Such a mismatch is more noticeable as $k$ increases, which leads us to infer that the contribution of the $k$-dependent term
\begin{align}\label{taylor-last-term}
    \frac{2 \ov{h} (k - 1)}{M - 1}
\end{align}
is not properly balanced. Moreover, for the special case of $k=1$, an analytical solution for \eqref{eq:optimum-beta} can be derived exactly as 
\begin{align} \label{beta-k=1}
\beta_{\tr{o},1} &= \frac{1}{2} \left[ \frac{(1 - 1/M)}{2v} + \frac{\ov{h^2}}{\ov{h}} \right]^{-1}
\end{align}
in which \eqref{taylor-last-term} does not appear (as expected); thereby, it reinforces the idea that the contribution of the term dependent on $k$ in \eqref{beta-taylor} must be revised. 
After an extensive analysis of different scenarios, we observed that $\ov{h}$ in \eqref{taylor-last-term} is too large and can be replaced by $\ov{h^2}$; as a result, a more accurate solution than \eqref{beta-taylor} to calculate the optimal step-size value follows as \eqref{eq:optimum_step}.



% investigating the impact of each term of \eqref{beta-taylor}, it is possible to infer that the contribution of 
% \begin{align}\label{taylor-last-term}
%     \frac{2 \ov{h} (k - 1)}{M - 1}
% \end{align}
% is not properly balanced.

% Next, investigating the impact of each term of \eqref{beta-taylor} on the solution, it is possible to infer that the contribution of 
% \begin{align}\label{taylor-last-term}
%     \frac{2 \ov{h} (k - 1)}{M - 1}
% \end{align}
% is not properly balanced.
% \cred{(Other values of $M$ and $\eta$ are not considered since it yields almost the same behavior.)}

% remove B label from figure numbering
\renewcommand{\thefigure}{\arabic{figure}}

\begin{figure}[t]
\centering
\includegraphics[scale=1]{figures/discussion/beta_appendix.pdf}
\caption{Optimal step-size value $\beta_{{\tr{o}}, k}$ obtained from the numerical solution of \eqref{eq:optimum-beta} (solid lines) and the approximate solution \eqref{beta-taylor} (dashed lines) as a function of the number of games $k$, considering different values of $v$ while $M = 15$ and $\eta = 0$. Curves for other values of $\eta$ are omitted since this variable does not affect \eqref{beta-taylor} significantly.
}
\label{fig:optimum_taylor}
\end{figure}



% \cred{
% %since we have to explain how we get here, appendix is the good place for that.
% Especially that there are some tricks used 
% [Taylor series for expanding \eqref{eq:v_k-final} at $\beta=0$, differentiate it with respect to $\beta$, and then solve the resulting expression for $\beta$; thereby, an approximate expression for the optimum step-size value considering a given number of games $k$ is obtained as]}

% \begin{align}
% \beta_{{\rm o},k} &\approx \frac{1}{2} \left[ \frac{(1 - 1/M)}{2v} + \frac{\ov{h^2}}{\ov{h}} + \frac{2 \ov{h^2} (k - 1)}{M - 1} \right]^{-1}.
% \end{align}



% Taylor series expansion of $f(a)$ at $a = a_0$:
% \begin{align}
% f(a) &\approx f(a_0) + f'(a_0) (a - a_0) + \frac{1}{2} f''(a_0) (a - a_0)^2
% \end{align}

% Solving $f'(a) = 0$:
% \begin{align}
% 0 &= f'(a_0) + f''(a_0) (a - a_0)\\
% a &= a_0 - \frac{f'(a_0)}{f''(a_0)}
% \end{align}


% \ov{d}_K''\Big|_{\beta=0} &= 16 K^2 M \ov{h}^2 v/(M - 1)^2 - 16 K M \ov{h}^2 v/(M - 1)^2 + 8 K M \ov{h^2} v/(M - 1) - 8 K \ov{h} (1/2 - M/2)/(M - 1)

% \begin{align}
% \frac{\partial \ov{d}_k}{\partial \beta} \Big|_{\beta=0} &= -\frac{4 k \ov{h} M v}{M-1} \\
% \frac{\partial^2 \ov{d}_k}{\partial \beta^2} \Big|_{\beta=0} &= \frac{8 k \ov{h} M v}{M-1} \left[ \frac{2 \ov{h} (k - 1)}{M - 1} + \frac{\ov{h^2}}{\ov{h}} + \frac{1-1/M}{2 v} \right]
% \end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{align}
% \ov{d}_K'(\beta) &= -\frac{8K\ov{h^2}}{M-1} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) (\ov{d}_0 - \ov{d}_{\infty})  \alpha_2^{K-1} + \frac{8 \beta^2 \ov{h}^2}{M-1} \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \end{align}


% \begin{align}
% \ov{d}_{k+1} &= \alpha_2\ov{d}_k + 2\beta^2 \ov{h}\\
% \ov{d}_k &= \alpha_2^k (\ov{d}_0 - \ov{d}_{\infty}) + \ov{d}_{\infty}\\
% \alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% \ov{d}_{\infty} &= \frac{2 \beta^2 \ov{h}}{1 - \alpha_2}\\
% \ov{d}_0 &= M v\\
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2 &= -\frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2})\\
% &= - \frac{1 - \alpha_2}{\beta} - \frac{4}{M-1} \beta \ov{h^2}\\
% &= \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)}\\
% &= -4\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right)
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2^K &= K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_{\infty} &= \frac{2 \ov{d}_{\infty}^2}{\beta^2 (M-1)}\\
% &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2}\\
% &= \frac{4 \lambda \beta^2 \ov{h}^2}{(1 - \alpha_2)^2}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_K &= \frac{\dd}{\dd\beta} [\alpha_2^K (\ov{d}_0 - \ov{d}_{\infty})] + \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + (1 - \alpha_2^K) \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2 + (1 - \alpha_2^K) \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= -4K\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) (\ov{d}_0 - \ov{d}_{\infty})  \alpha_2^{K-1} + 4 \lambda \beta^2 \ov{h}^2 \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% &= -4K\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) (\ov{d}_0 - \ov{d}_{\infty})  \alpha_2^{K-1} + 4 \lambda \beta^2 \ov{h}^2 \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Checking out the optimum step-size}

% % \ov{d}_{\infty} &= \frac{\beta \ov{h} (M-1)}{2(\ov{h} - \beta \ov{h^2})}\\
% \begin{align}
% \ov{d}_{k+1} &= \alpha_2\ov{d}_k + 2\beta^2 \ov{h}\\
% \ov{d}_k &= \alpha_2^k (\ov{d}_0 - \ov{d}_{\infty}) + \ov{d}_{\infty}\\
% \alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% \ov{d}_{\infty} &= \frac{2 \beta^2 \ov{h}}{1 - \alpha_2}\\
% \ov{d}_0 &= M v\\
% \end{align}

% \begin{align}
% \beta^2 - \beta \frac{\ov{h}}{\ov{h^2}} + \frac{(1 - \alpha) (M-1)}{4\ov{h^2}} = 0
% \end{align}

% \begin{align}
% \beta &= -\frac{\ov{h}}{2\ov{h^2}} \pm \frac{1}{2} \sqrt{\left( \frac{\ov{h}}{\ov{h^2}} \right)^2 - \frac{\ov{h}}{\ov{h^2}}\frac{(1 - \alpha) (M-1)}{\ov{h^2}} }\\
% \beta &= \frac{1}{2\ov{h^2}} \left[ -\ov{h} + \sqrt{ \ov{h}^2 - \ov{h} (1 - \alpha) (M-1) } \right] \\
% \beta &= \frac{\ov{h}}{2\ov{h^2}} \left[\sqrt{ 1 - \frac{(1 - \alpha) (M-1)}{\ov{h}} } - 1 \right] \\
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2 &= -\frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2})\\
% &= - \frac{1 - \alpha_2}{\beta} - \frac{4}{M-1} \beta \ov{h^2}\\
% &= \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)}
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2^K &= K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_{\infty} &= \frac{2 \ov{d}_{\infty}^2}{\beta^2 (M-1)}\\
% &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_{k+1} &= \frac{\dd}{\dd\beta}(\alpha_2 \ov{d}_k) + 4\beta \ov{h}\\
% \frac{\dd}{\dd\beta} \ov{d}_k &= \alpha_2^k (\ov{d}_0 - \ov{d}_{\infty}) + \ov{d}_{\infty}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_K &= \frac{\dd}{\dd\beta} [\alpha_2^K (\ov{d}_0 - \ov{d}_{\infty})] + \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + \alpha_2^K \frac{\dd}{\dd\beta} (\ov{d}_0 - \ov{d}_{\infty}) + \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + (1 - \alpha_2^K)\frac{\dd}{\dd\beta} \ov{d}_{\infty} \\
% &= (\ov{d}_0 - \ov{d}_{\infty}) K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2 + (1 - \alpha_2^K)\frac{\dd}{\dd\beta} \ov{d}_{\infty} \\
% &= \frac{\dd}{\dd\beta} \ov{d}_{\infty} + \alpha_2^{K-1} \left[ (\ov{d}_0 - \ov{d}_{\infty}) K \frac{\dd}{\dd\beta} \alpha_2 - \alpha_2 \frac{\dd}{\dd\beta} \ov{d}_{\infty} \right]\\
% % &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + \alpha_2^{K-1} \left[ (\ov{d}_0 - \ov{d}_{\infty}) K \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)} - \alpha_2 \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} \right]\\
% % &= (1-\alpha_2^K) \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + K\alpha_2^{K-1} (\ov{d}_0 - \ov{d}_{\infty}) \left( \frac{4\beta \ov{h^2}}{(M-1)} - \frac{1 - \alpha_2}{\beta} \right)\\
% &= (1-\alpha_2^K) \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + K\alpha_2^{K-1} \left( M v - \frac{2\beta^2\ov{h}}{1 - \alpha_2} \right) \left( \frac{4\beta \ov{h^2}}{(M-1)} - \frac{1 - \alpha_2}{\beta} \right)
% \end{align}


% \begin{align}
% 0 &= (1-\alpha_2^K) \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + K\alpha_2^{K-1} \left( M v - \frac{2\beta^2\ov{h}}{1 - \alpha_2} \right) \left( \frac{4\beta \ov{h^2}}{(M-1)} - \frac{1 - \alpha_2}{\beta} \right)\\
% 0 &= \frac{8 (1-\alpha_2^K) \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + \frac{K\alpha_2^{K-1}}{\beta(M-1)(1 - \alpha_2)} \left[ (1 - \alpha_2) M v - 2\beta^2\ov{h} \right] \left[ 4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1) \right]\\
% 0 &= \frac{8 (1-\alpha_2^K) \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + \frac{4\ov{h} K\alpha_2^{K-1}}{(M-1)(1 - \alpha_2)} \left[ (1 - \alpha_2) M v - 2\beta^2\ov{h} \right]\\
% 0 &= 8\beta^2 \ov{h}^2 \frac{(1-\alpha_2^K) }{(1 - \alpha_2)} + 4\ov{h} K\alpha_2^{K-1}\left[ (1 - \alpha_2) M v - 2\beta^2\ov{h} \right]\\
% \frac{8\beta^2 \ov{h}^2}{\alpha_2^{K-1}} &= 8\beta^2 \ov{h}^2 \alpha_2 - 4\ov{h}K (1 - \alpha_2) \left[ (1 - \alpha_2) M v - 2\beta^2\ov{h} \right]\\
% \frac{8\beta^2 \ov{h}^2}{\alpha_2^{K-1}} &= 8\beta^2 \ov{h}^2 \alpha_2 - 4\ov{h}K (1 - \alpha_2)^2 M v + 8\beta^2\ov{h}^2 K (1 - \alpha_2)\\
% \frac{8 \ov{h}^2}{\alpha_2^{K-1}} &= 8\ov{h}^2 K (1 - \alpha_2) + 8 \ov{h}^2 \alpha_2 - 4\ov{h}K (1 - \alpha_2)^2 M v \frac{1}{\beta^2}\\
% \frac{1}{\alpha_2^{K-1}} &= (K-1) (1 - \alpha_2) + 1 - K (1 - \alpha_2)^2 M v \frac{1}{2\beta^2\ov{h}}\\
% 2\beta^2\ov{h} &= [2\beta^2\ov{h} - (1 - \alpha_2) M v] K (1-\alpha_2) \alpha_2^{K-1}\\
% % 2\beta^2\ov{h} &= -\frac{KMv(1 - \alpha_2)^2 \alpha_2^{K-1}}{1 - K (1-\alpha_2) \alpha_2^{K-1}}\\
% \frac{1}{2\beta^2\ov{h}} &= \frac{1}{Mv} - \frac{1}{Mv K\alpha_2^{K-1}} \left[ \frac{M-1}{4\beta (\ov{h} - \beta \ov{h^2})} \right]^2\\
% \frac{Mv}{2\beta^2\ov{h}} &= 1 - \frac{1}{K\alpha_2^{K-1}} \left[ \frac{M-1}{4\beta (\ov{h} - \beta \ov{h^2})} \right]^2\\
% \frac{Mv}{2\ov{h}} &= \beta^2 - \frac{1}{K\alpha_2^{K-1}} \left[ \frac{M-1}{4(\ov{h} - \beta \ov{h^2})} \right]^2\\
% % \frac{Mv}{2\ov{h}} &= \left[\beta + \frac{1}{\sqrt{K} \alpha_2^{(K-1)/2}} \frac{M-1}{4(\ov{h} - \beta \ov{h^2})} \right] \left[\beta - \frac{1}{\sqrt{K} \alpha_2^{(K-1)/2}} \frac{M-1}{4(\ov{h} - \beta \ov{h^2})} \right]\\
% \frac{Mv}{2\ov{h}\beta^2} &= \left[1 + \frac{1}{\sqrt{K} \alpha_2^{(K-1)/2} (1-\alpha_2)} \right] \left[1 - \frac{1}{\sqrt{K} \alpha_2^{(K-1)/2} (1-\alpha_2)} \right]\\
% \frac{Mv}{2\ov{h}\beta^2} &= \frac{1}{K \alpha_2^{K-1}} \left[ K \alpha_2^{K-1} + \frac{\sqrt{K} \alpha_2^{(K-1)/2}}{1-\alpha_2} \right] \left[K \alpha_2^{K-1} - \frac{\sqrt{K} \alpha_2^{(K-1)/2}}{1-\alpha_2} \right]\\
% \end{align}


% \begin{align}
% 2\beta^2\ov{h} &= [2\beta^2\ov{h} - (1 - \alpha_2) M v] K (1-\alpha_2) \alpha_2^{K-1}\\
% 1 &= \frac{\ov{d}_\infty - \ov{d}_0}{\ov{d}_\infty} K (1-\alpha_2) \alpha_2^{K-1}\\
% \frac{\ov{d}_\infty}{K(\ov{d}_\infty - \ov{d}_0)} &= \alpha_2^{K-1} - \alpha_2^K\\
% \alpha_2 &\approx \left[ \frac{\ov{d}_\infty}{K(\ov{d}_\infty - \ov{d}_0)} \right]^{1/(K-1)}\\
% 1 - \frac{4}{M-1}\beta &\approx \left[ \frac{\ov{d}_\infty}{K(\ov{d}_\infty - \ov{d}_0)} \right]^{1/(K-1)}\\
% \end{align}

% \begin{align}
% v_z = 2\frac{Mv}{M-1}\\
% K_o = \frac{4K\ov{h}}{M-1}
% \end{align}

% \begin{align}
% 2\beta^2\ov{h} &= [2\beta^2\ov{h} - (1 - \alpha_2) M v] K (1-\alpha_2) \alpha_2^{K-1}\\
% \alpha_2^{K-1} &= \frac{\ov{d}_\infty}{K (\ov{d}_\infty - \ov{d}_0) (1-\alpha_2)}\\
% \alpha_2^{K-1} &\approx \frac{M-1}{4K\ov{h} (\beta - v_z)}\\
% \frac{1}{\alpha_2^{K-1}} &\approx K_o (\beta - v_z)\\
% \alpha_2 &\approx \left[ \frac{1}{K_o (\beta - v_z)} \right]^{1/(K-1)}\\
% 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2}) &\approx \left[ \frac{1}{K_o (\beta - v_z)} \right]^{1/(K-1)}\\
% \beta &\approx \frac{M-1}{4\ov{h^2}(\ov{h}/\ov{h^2} - \beta)} \left\{ 1 - \left[ \frac{1}{K_o (\beta - v_z)} \right]^{1/(K-1)} \right\}\\
% \end{align}


% \begin{align}
% 2\beta^2\ov{h} &= [2\beta^2\ov{h} - (1 - \alpha_2) M v] K (1-\alpha_2) \alpha_2^{K-1}\\
% \alpha_2^{K-1} &= \frac{\ov{d}_\infty}{K (\ov{d}_\infty - \ov{d}_0) (1-\alpha_2)}\\
% \alpha_2^{K-1} K (\ov{d}_\infty - \ov{d}_0) &\approx \ov{d}_\infty\\
% \alpha_2^{K-1} K (\beta (M-1)/2 - Mv) &\approx \beta (M-1)/2\\
% \end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section*{Checking out the optimum step-size}

% \begin{align}
% \ov{d}_{k+1} &= \alpha_2\ov{d}_k + 2\beta^2 \ov{h}\\
% \ov{d}_k &= \alpha_2^k (\ov{d}_0 - \ov{d}_{\infty}) + \ov{d}_{\infty}\\
% \alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% \ov{d}_{\infty} &= \frac{2 \beta^2 \ov{h}}{1 - \alpha_2}\\
% \ov{d}_0 &= M v\\
% \lambda &= \frac{2}{M-1}\\
% \alpha_2 &= 1 - 2 \lambda \ov{h^2} \beta \left( \frac{\ov{h}}{\ov{h^2}} - \beta \right)
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2 &= -\frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2})\\
% &= - \frac{1 - \alpha_2}{\beta} - \frac{4}{M-1} \beta \ov{h^2}\\
% &= \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)}\\
% &= -4\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right)
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2^K &= K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_{\infty} &= \frac{2 \ov{d}_{\infty}^2}{\beta^2 (M-1)}\\
% &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2}\\
% &= \frac{4 \lambda \beta^2 \ov{h}^2}{(1 - \alpha_2)^2}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{d}_K &= \frac{\dd}{\dd\beta} [\alpha_2^K (\ov{d}_0 - \ov{d}_{\infty})] + \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + (1 - \alpha_2^K) \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= (\ov{d}_0 - \ov{d}_{\infty}) K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2 + (1 - \alpha_2^K) \frac{\dd}{\dd\beta} \ov{d}_{\infty}\\
% &= -4K\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) (\ov{d}_0 - \ov{d}_{\infty})  \alpha_2^{K-1} + 4 \lambda \beta^2 \ov{h}^2 \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% &= -4K\lambda\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) (\ov{d}_0 - \ov{d}_{\infty})  \alpha_2^{K-1} + 4 \lambda \beta^2 \ov{h}^2 \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \end{align}


% \begin{align}
% % K\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) \ov{d}_0  \alpha_2^{K-1} &=  K\ov{h^2} \left( \frac{\ov{h}}{2\ov{h^2}} - \beta \right) \ov{d}_{\infty} \alpha_2^{K-1} + \beta^2 \ov{h}^2 \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \frac{\ov{d}_0}{2 \beta^2 \ov{h}}  \alpha_2^{K-1} &= \frac{\alpha_2^{K-1}}{1 - \alpha_2} + \frac{1}{K \left( 1 - 2 \frac{\ov{h^2}}{\ov{h}} \beta \right)}  \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \frac{\ov{d}_0}{2 \beta^2 \ov{h}}  \alpha_2^{K-1} &= \frac{1}{1 - \alpha_2} - \frac{1-\alpha_2^{K-1}}{1 - \alpha_2} + \frac{1}{K \left( 1 - 2 \frac{\ov{h^2}}{\ov{h}} \beta \right)}  \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \frac{\frac{\ov{d}_0}{2 \beta^2 \ov{h}}  \alpha_2^{K-1} - 1}{1 - \alpha_2} - \frac{\ov{d}_0}{2 \beta^2 \ov{h}} \frac{\alpha_2^K}{1 - \alpha_2} &= - \frac{1-\alpha_2^{K-1}}{1 - \alpha_2} + \frac{1}{K \left( 1 - 2 \frac{\ov{h^2}}{\ov{h}} \beta \right)}  \frac{(1 - \alpha_2^K)}{(1 - \alpha_2)^2} \\
% \end{align}



==> old/Common.Files/included_packages.tex <==
\usepackage{amsmath,amssymb,amscd,latexsym,dsfont,wasysym,bbm}
%\usepackage{txfonts}  %% transforms the fonts into Times-New-Roman style
\usepackage{float}
\usepackage{color}
\usepackage{graphicx,subfigure}
\usepackage{multirow,multicol} 
\usepackage{verbatim}
\usepackage{psfrag}
\usepackage{comment}
\usepackage{makeidx}
\usepackage[]{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
%\usepackage{cite}
\usepackage{cases}
%\usepackage{amsthm}
 \usepackage{setspace}
%\usepackage[table]{xcolor}
\usepackage{pgfplots} %%%% added by LS for the errata 7.sept.2015
%\usepackage{subdepth} %%% To fix the alignment of the subscripts. It helps, but it also makes {?BICM-ID.SumExp.m1} look horrible!

==> old/Common.Files/tikz.definitions.tex <==
% Define a few styles and constants

% Function block
\tikzstyle{rect_my} = [draw, rectangle, minimum width=2cm, text width=1.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{square_my} = [draw, rectangle, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{square_my_graph} = [draw, rectangle, minimum width=1.2cm, text width=1cm, fill=gray!15, 
  text centered,  minimum height=1.2cm]
\tikzstyle{circle_my} = [draw, circle, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=.9cm]
\tikzstyle{circle_my_graph} = [draw, circle, minimum width=1.1cm, text width=.8cm, fill=gray!15, 
  text centered]
\tikzstyle{cloud_my} = [draw, shape=cloud, minimum width=1cm, text width=0.8cm, fill=gray!15, 
  text centered,  minimum height=1cm]

% Point
\tikzstyle{point_my} = [draw=none, minimum width=0cm, text width=0cm, fill=none, 
  text centered,  minimum height=0cm]    
\tikzstyle{line_my} = [draw, -latex]    
% Boxes
\tikzstyle{box_my}=[draw, minimum size=2em, text width=4.5em, text centered]
\tikzstyle{bigbox_my}=[draw, inner sep=15pt]
\tikzstyle{arrow_my} = [thick,->,>=stealth]
\tikzstyle{noarrow_my} = [thick,-,=>stealth]

%%%
\newcommand{\jumpline}[2]{
\path(#1.east) --(#2.west)  coordinate[pos=0.4](mid);
\draw[-latex] (#1.east) -| (mid) |- (#2.west);
}

==> old/Discussion.tex <==
\section{Discussion}\label{Sec:Discussion}
%Here, some interesting insights coming from the model expressions are discussed, aiming to provide useful design guidelines about the behavior of the rating algorithm. Specifically, a discussion about the time constants related to the convergence of the algorithm is first presented. Next, some considerations about the mean loss are discussed, emphasizing the lower bound of the loss and the excess loss. Then, a condition on the step-size value is derived to ensure that the rating algorithm improves the skills' estimate over its initialization value, reducing the uncertainty of the solution as $k$ increases. Lastly, an approximate expression is obtained for computing the optimum step-size value given a certain number of games $k$.


Based on the model expressions derived so far (see Section~\ref{Sec:analysis}), some insight into the behavior of the rating algorithm (with respect to the number of games $k$, variance $v$, \gls{hfa} $\eta$, and step size $\beta$) are discussed below, in order to provide useful design guidelines.


%\sout{Specifically, we relate the variance $v$ (which characterizes the model) and the algorithm parameters (especially, $\beta$) to the practically relevant concepts such as the time constants and the values of the mean loss.}

% Aiming to make the mathematical development tractable, we first introduce assumptions and approximations used to derive mathematical expressions describing the behavior of the skills and of the loss function that are next used to obtain insights on the behavior of the algorithm providing at the same useful design guidelines.

%\subsection{Time constants and meaning of ``convergence''}\label{sec:time}
\subsection{Time constants}\label{sec:time}
For an intuitive interpretation of convergence, the concept of time constant associated with the exponential terms observed in \eqref{eq:skill-behavior} and \eqref{eq:v_k-final} can be used by rewriting the exponential term based on $\alpha_1$ in \eqref{eq:skill-behavior} as follows:
\begin{align}
\label{alpha.1.power.k}
\alpha_1^k &=\e^{-\frac{k}{\tau_1}}
\end{align}
%we have
%\begin{align*}
%\tau_1 &= -\frac{1}{\ln \alpha_1} \quad\\
%\numberthis  &\approx \frac{1}{1 - \alpha_1}
%\end{align*}
from which the convergence of skills $\btheta_{k}$ in the mean sense is characterized by the time constant $\tau_1 = -[\ln( \alpha_1)]^{-1}$. Thus, from \eqref{eq:alpha_1}, we have 
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{tau.1}
\tau_1 &\approx \frac{M-1}{2 \beta\ov{h}}.
\end{empheq}
Similarly, a time constant $\tau_2= -[\ln(\alpha_2)]^{-1}$ associated with the convergence of $\btheta_{k}$ in the mean-square sense [see \eqref{eq:v_k-final}] can be determined as %follows from
%\begin{align}
%\alpha_2^k &=\e^{-\frac{k}{\tau_2}}
%\tau_2 &= -\frac{1}{\ln \alpha_2}
%\end{align}
%as
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{tau.2}
\tau_2 &\approx \frac{M-1}{4 \beta(\ov{h} - \beta \ov{h^2})}.
\end{empheq}
Approximations used in \eqref{tau.1} and \eqref{tau.2} hold for values of $\alpha_1$ and $\alpha_2$ near 1.

% sufficiently small $\beta$. 

% values of $\alpha_1$ e $\alpha_2$ próximos de 1

%, which implies $\alpha_1 \approx 1$ and $\alpha_2 \approx 1$, respectively.
% \sout{rely on $\ln (1+a) \approx a$ valid for small $a$ and thus} 

% For small $\beta$ (which allows us to ignore the term $\beta\ov{h^2}$ in \eqref{tau.2}) we have $\tau_1 \approx 2\tau_2$. 

% \sout{We also note that, for large $\beta$, the term $\beta\ov{h^2}$ cannot be ignored in \eqref{tau.2} and the relationship $\tau_1\approx2\tau_2$ breaks. In fact, for a sufficiently large $\beta$,  $\btheta_k$ may converge in the mean, \ie $\alpha_1<1$ but the convergence of the \gls{msd} is not guaranteed, \ie $\alpha_2>1$. However, such extreme values of $\beta$ are of no interest.}


Fig.~\ref{fig:time_constant} shows how the time constants $\tau_1$ [given by \eqref{tau.1}] and $\tau_2$ [given by \eqref{tau.2}] related to the convergence speed of the rating algorithm in the mean and mean-square senses, respectively, as a function of the step-size value $\beta$, considering $M = 15$, $v=3$, and $\eta=0$. (Other values of $v$ are not considered since their impact on $\tau_1$ and $\tau_2$ is negligible.) Notice that these time constants are inversely proportional to the step size value; thus the convergence speed of the rating algorithm becomes slower as $\beta$ decreases and vice-versa. Furthermore, observe that the algorithm presents different convergence requirements in terms of $\tau_1$ (associated with the estimate of skills $\btheta_k$) and $\tau_2$ (related to the uncertainty of the skill estimates $\ov{d}_k$); in particular, $\ov{d}_k$ decays faster than the estimated skills $\btheta_k$ improve for small $\beta$, \ie $\tau_1 \approx 2 \tau_2$ since the term $\beta\ov{h^2}$ in \eqref{tau.2} can be ignored. Besides the aforementioned aspects, this figure gives us an idea that \eqref{tau.1} and \eqref{tau.2} may help in the selection of $\beta$ so that the algorithm reaches convergence within a pre-defined number of games.

\begin{figure}[t!]
\centering
\includegraphics[scale=1]{figures/discussion/time_constants.pdf}
\caption{Time constants related to the convergence of the rating algorithm in the mean $\tau_1$ [given by \eqref{tau.1}] and mean-square $\tau_2$ [given by \eqref{tau.2}] sense as a function of $\beta$, considering $M = 15$, $v=3$, and $\eta=0$.}
\label{fig:time_constant}
\end{figure}

% In addition, observe that the uncertainty of the skill estimates $\ov{d}_k$ (associated with $\tau_2$) reduces faster than the estimate of the skills $\btheta_k$ (related to $\tau_1$) improve;

% in particular, one verifies that $\tau_1 \approx 2 \tau_2$ for small $\beta$ since in this condition the term $\beta\ov{h^2}$ in \eqref{tau.2} can be ignored.
\subsection{Meaning of ``convergence''}\label{sec:convergence}

At this point, it may be useful to differentiate between the concept of convergence understood as a mathematical condition that guarantees that $\btheta_k$ tends to $\btheta^*$ as $k$ increases and the one used colloquially in the rating literature that loosely assumes that convergence to the optimum is reached after an arbitrary and pre-defined number of games.\footnote{As pointed out critically in \cite[Sec.~3]{aldous2017}, the statement ``ratings tend to converge on a team’s true strength relative to its competitors after about 30 matches" is accepted at face value both in the literature and applications \cite{eloratings.net}, \cite{fide}. Note that the number of games is commonly viewed in a per-team basis; so, for comparison purposes, it is important to use $2k/M$ as the number of games instead of $k$.} However, this colloquial meaning does not hold because convergence cannot be characterized in a deterministic sense; in other words, it is not possible to establish any deterministic guarantees to reach the optimum within a finite number of games $k$. Therefore, the convergence of the rating algorithm can only be assessed in %either [LS: both are possible so not "either or"]
asymptotic or probabilistic senses.

% However, this colloquial meaning  does not hold because  the convergence must be characterized both in asymptotic and probabilistic senses; as a consequence, it is not possible to establish any \cred{deterministic} guarantees on reaching the optimum within a finite number of games $k$.

Aiming to provide a practical guideline on the number of games required by the rating algorithm to reach convergence, we have to rely on some heuristics, such as
\begin{itemize}
\item The approximation error $|\Ex[\theta_{k,m}]-\theta^*_m|$ becomes sufficiently small compared to the initial one $|\theta_{0,m}-\theta^*_m|$, which defines convergence in the mean sense; or
\item $\ov{d}_k$ (or, equivalently, $\ov{\ell}_k$) is sufficiently small compared to $\ov{d}_0$ (or, equivalently, $\ov{\ell}_0$), which defines convergence in the mean-square sense.
\end{itemize}
%The ``sufficiently small'' value can be defined via the number of games $K_{\tr{c}}$ \cred{exceeding a multiple} of the time constants $\tau_1$ or $\tau_2$. 
The ``sufficiently small" value can be predefined by specifying the number of games to reach convergence $K_\tr{c}$ as a multiple of the time constants $\tau_1$ or $\tau_2$. For example, for $K_\tr{c}=3\tau_1$, the exponential curve \eqref{alpha.1.power.k} decays 95\% of its initial value, becoming sufficiently flat to declare convergence by eyeballing. As a result, for $k>K_\tr{c}$, the approximation error $|\Ex[\theta_{k,m}]-\theta^*_m|$ becomes smaller than $5\%$ of the initial value $|\theta_{0,m}-\theta^*_m|$; also, since $\tau_1 \approx 2\tau_2$  for sufficiently small $\beta$, convergence in the mean sense implies that $\ov{d}_k$ practically equals its final value $\ov{d}_\infty$. So, by analyzing $\tau_1$ and $\tau_2$ we can define the step size $\beta$ to achieve convergence within a predefined number of games $k$.

% Moreover, because , for any practical purposes, the \gls{msd} \eqref{eq:v_k-final} practically equals the final value $\ov{d}_\infty$.
% we are mostly concerned with the convergence of the mean which is slower than the convergence of the \gls{msd}/variance.

%\cred{\bf In my opinion, we should not discuss anything about per team convergence...it is just confusing the reader.}
%\cred{
%Finally, to address the literature claims on the number of games required for the team to ``reach the convergence'', we have to define the time constant on a per-team level. This is done by noting that the probability of any given team $m$ being scheduled is $\PR{i_k=m\vee j_k=m}=\frac{2}{M}$.\footnote{Under the uniform scheduling assumption, there are $2(M-1)$ pairs $(i_k, j_k)$ with $i_k=m$ or $j_k=m$, and the total number of pairs is $M(M-1)$} Thus, the individual time constant characterizing the convergence in the mean sense, has to be scaled down by the same number yielding
% \begin{align*}
% \tau_\tr{team} &= \frac{2\tau_1}{M}\\
% &= \frac{1-1/M}{\beta\ov{h}}. \numberthis
% \end{align*}
% Of course, the same scaling applied to $\tau_2$ but, as we said, we are mostly concerned with the convergence of the mean which is slower than the convergence of the \gls{msd}/variance.
% }





% Moreover, \eqref{tau.1} and \eqref{tau.2} allows adjusting $\beta$ such that the algorithm converges within a given number of games (\eg reaches $95\%$ of the final value in $3\tau_i$ games [REF]); for example, considering $\tau_i=90$ (implying convergence in at least 270 games), the step-size value may be chosen as $\beta_i$ for $i=1,2$ depending on the conflicting goals between excess loss and ??????


% \begin{align}
% \beta_2 \approx \frac{1}{2} \beta_1
% \end{align}



% Note that $\tau'_n = \frac{2}{M} \tau_n,\: n=1,2$ allows discussing in terms of individual teams.
% \begin{align}
% \tau_{n}' &= \frac{2}{M} \tau_n, \quad n=1,2
% \end{align}




% Moreover, based on \eqref{tau.1} and \eqref{tau.2}, it is possible to choose $\beta$ such that the algorithm reaches a proportion the final value of the estimate and its uncertainty 

% $\Ex[\btheta_k]$ and $\ov{d}_k$

% \dz{30 games? maybe, but depends on the scenario ($v$). Also, optimum step size changes with $K$.}

% depending on $v$, one observes that 

% \dz{Trade-off between the convergences in the mean ($\tau_1$) and mean-square sense ($\tau_2$).}


% tau = [1, 2, 3, 4, 5] 
% % of convergence = [0.63212056, 0.86466472, 0.95021293, 0.98168436, 0.99326205]

% See: \url{https://en.wikipedia.org/wiki/Time_constant}

% \begin{align*}
% \ov{d}_{\infty} \approx 2 \beta^2 \ov{h} \tau_2
% \end{align*}




% \ls{This is my idea of how to present the results and (hopefully) avoid confusion:
% \begin{enumerate}
%     \item The argument axis = $K$, \ie the number of games.
%     \item For each $K$ we find the step $\beta$ which guarantees that we converge at $K$, \ie $3\tau=K$ (of course, here we can have the discussion which $\tau$ to choose). This will also depend on the variance which is the plot's parameter.
%     \item We show the horizontal lines which are the limits guaranteeing the improvement over initialization. Or optimum $\beta$ for $K=1$, or even the optimal $\beta$ for any $K$ tout court.
%     \item Then we will see that for large $v$ the step which guarantee the improvement will also help us to converge in 30 games. For smaller $v$ we will see that we need more games to converge and improve.
% \end{enumerate}
% I still feel the trade-off convergence-- excess-loss is not clearly emphasized. Maybe another figure showing the excess-loss as a function of $K$ (for $\beta$ which guarantees the convergence)? 
% }

\subsection{On the mean loss}\label{sec:loss}

% Based on \eqref{eq:loss-behavior}, one verifies that the mean loss achieved by the algorithm is composed of two (non-negative) terms, namely, $\ov\ell_{\tr{min}}$ (which is mainly affected by the variance $v$) and $\ov\ell_{{\rm ex},k}$ (which mostly depends on the choice of the step size $\beta$). So, we discuss in the following the impact of these variables on the performance/behavior of the rating algorithm.

Based on \eqref{eq:loss-behavior}, it can be verified that the mean loss $\ov\ell_{k}$ achieved by the algorithm is made up of a sum of two (non-negative) terms, namely $\ov\ell_{\tr{min}}$ [given by \eqref{eq:l_min}] and $\ov\ell_{{\rm ex},k}$ [given by \eqref{eq:l_ex}] which depend on $v$, $\eta$, $M$, $k$, and $\beta$. Particularly, $\ov\ell_{\tr{min}}$ depends only on the application/operating scenario considered (mainly through $v$), \ie it is not affected by the choice of step size $\beta$, \gls{hfa} $\eta$, number of teams $M$, and number of games $k$. In turn, $\beta$ and $k$ play important roles on the excess-loss $\ov\ell_{{\rm ex},k}$, increasing somehow the value of $\ov\ell_{k}$ achieved by the rating algorithm. So, it becomes helpful to clarify the impact of these variables on the performance of the rating algorithm.

%To illustrate the role ,
\figref{fig:loss_min} plots the lower-bound of the loss $\ov\ell_\tr{min}$ [given by \eqref{eq:l_min}] as a function of the variance $v$, considering different values of $\eta$ and $M=15$. This figure emphasizes that the performance of the algorithm degrades as $v$ decreases due to the high uncertainty of the results; this also leads to larger values of $\ov\ell_\tr{min}$. On the other hand, when $v$ increases, the difference between the skills of the players may be large and the results of the games between these players are more easily predicted; hence $\ov\ell_\tr{min}$ becomes smaller. Also, note that the impact of the \gls{hfa} parameter $\eta$ on $\ov\ell_\tr{min}$ is less significant as $v$ increases, since $\eta$ in \eqref{eq:l_min} can be ignored when the differences between skills are large.

In order to characterize the meaning of small and large $v$ (high and low uncertainty), let us approximate the curves in \figref{fig:loss_min} by using two asymptotes, one of them valid when $v\rightarrow 0$ and the other for $v\rightarrow\infty$. Thereby, we can determine a boundary/threshold $v_\tr{th}$ from the intersection of these two asymptotes [arising from \eqref{eq:l_min}], \ie
\begin{align}
    \ov{\ell}_\tr{min}\Big|_{v=0} &= \ov{\ell}_\tr{min}\Big|_{v\gg 2\ln(2)}
    %\\
    %\ln2 &= \frac{\ln2\sqrt{2\ln2}}{\sqrt{v_\tr{th}}}\\
\end{align}
which results in
\begin{align*}
    v_\tr{th} &= 2\ln(2)\\
              &\approx 1.4.\numberthis
\end{align*}
So, this value $v_\tr{th}$ establishes a boundary that separates small and large $v$.

% which is thus a variance threshold separating the high- and low- variance scenarios.

% Specifically, we can consider \eqref{eq:l_min} with $v=0$ as an approximation valid when $v\rightarrow 0$ and $v\gg 2\ln(2)$ as an approximation valid when $v\rightarrow\infty$.

%The quasi-linear behaviour of the curves in \figref{fig:loss_min} for extreme values of $v$ may be exploited to separate the high- and low-variance scenarios: 
% we  use \eqref{eq:l_min} for $v=0$ (yielding the approximation valid when $v\rightarrow 0$), and for $v\gg 2\ln(2)$ (approximation valid when $v\rightarrow\infty$).  Assuming $\eta=0$ and using \eqref{eq:l_min} we obtain the intersection of both lines at $v=v_\tr{th}$ as
% \begin{align}
%     \ov{\ell}_\tr{min}|_{v=0} &= \ov{\ell}_\tr{min}|_{v\gg 2\ln 2}\\
%     \ln2 &= \frac{\ln2\sqrt{2\ln2}}{\sqrt{v_\tr{th}}}\\
%     v_\tr{th} &= 2\ln 2 \approx 1.4
% \end{align}
% which is thus a variance threshold separating the high- and low- variance scenarios.

% \begin{align}
% \ln(2) \exp{\left[\frac{-\eta^2}{8\ln(2)}\right]} &= \ln(2) \sqrt{\frac{2\ln(2)}{v_\tr{th}}}\\
% v_\tr{th} &= 2\ln(2) \exp{\left[\frac{\eta^2}{4\ln(2)}\right]}
% \end{align}

\begin{figure}[t]
\centering
\includegraphics[scale=1]{figures/discussion/loss_min.pdf}
\caption{Lower bound of the loss $\ov\ell_{\tr{min}}$ [given by \eqref{eq:l_min}] as a function of variance $v$, considering different values of $\eta$ and $M=15$. Asymptotes are shown using dark-dashed lines.}
\label{fig:loss_min}
\end{figure}


%To assess the impact of , 
\figref{fig:loss_ex} plots the mean excess-loss $\ov\ell_{{\rm ex},k}$ [given by \eqref{eq:l_ex}] as a function of $\beta$, considering different number of games $k$ while $\eta = 0$, $v = 3$, and $M = 15$. This figure ratifies the impact of $\beta$ and $k$ on the excess loss attained by the rating algorithm. Specifically, for a large number of games ($k\to\infty$), the excess loss exhibits a monotonically increasing characteristic with respect to $\beta$, \ie large $\beta$ yields higher values of $\ov\ell_{\tr{ex},k}$. On the other hand, for finite $k$ (\eg 50, 100, or 200 games), a unimodal characteristic (\ie unique minimum) is observed in the mean excess-loss\footnote{The loss $\ov\ell_k$ [given by \eqref{eq:loss-behavior}] will also exhibit the same convex characteristic.} due to the bias-variance trade-off (see Section~\ref{Sec:Variance.skills}); so, there is an optimum step-size value $\beta_{\tr{o}, k}$ which leads to the minimum attainable value of $\ov\ell_{\tr{ex},k}$ for a given number of games $k$ (as discussed later in Section~\ref{sec:optimum_step}). This characteristic is due to the fact that the rating algorithm is not capable of converging within $k$ games for small values of $\beta$; as a consequence, $\ov\ell_{\tr{ex},k}$ may be higher than the one achieved with intermediate values of $\beta$. Therefore, since $k$ is finite, in general, choosing an appropriate value for $\beta$ becomes important. 


% We can observe here the trade-off between the bias and the variance we already discussed in \secref{Sec:Variance.skills}. In particular,
% \begin{itemize}
%     \item For small $\beta$ and finite $k$, the excess loss is practically equal to $\ell_{\tr{ex},0}\approx \ov{h} v=\frac{vM}{4\sqrt{v+1}(M-1)}$, which is obtained plugging \eqref{mean-h_k} and \eqref{eq:msd_0} into \eqref{eq:l_ex}; here it is equal to $\ell_{\tr{ex},0}\approx 0.4$. This value is entirely caused by the initialization bias.
%     \item Increasing $k$ to infinity, we obtain $\ell_{\tr{ex},\infty}\approx \frac{\beta}{8\sqrt{v+1}}$.
% \end{itemize}


\begin{figure}[t]
\centering
\includegraphics[scale=1]{figures/discussion/steady_state.pdf}
\caption{%\cred{I would show the grid}
Excess loss [given by \eqref{eq:l_ex}] as a function of the step-size value $\beta$, considering different number of games $k$ while $\eta = 0$, $v = 3$, and $M = 15$.}
\label{fig:loss_ex}
\end{figure}



\subsection{Improvement over initialization}
A condition on the step-size $\beta$ is now derived to ensure that the uncertainty about the estimated skills $\btheta_k$ (characterized by $\ov{d}_k$) is reduced over its initial value as $k$ increases, \ie
\begin{align}\label{ineq:improvement_msd}
\ov{d}_k &< \ov{d}_0.
\end{align}
To this end, substituting \eqref{eq:v_k-final} into \eqref{ineq:improvement_msd}, we have the following:
\begin{align}
\label{ineq:improvement_msd3}
(1 - \alpha_2^k) (\ov{d}_0 - \ov{d}_{\infty}) &> 0.
\end{align}
Then, since $|\alpha_2| < 1$ implies that $(1-\alpha_2^k)$ is positive, 
% which holds if $|\alpha_2| < 1$ and reduces to
\eqref{ineq:improvement_msd3} reduces to\footnote{
Note that \eqref{ineq:improvement_msd4} can be reinterpreted in terms of the bias-variance trade-off as $\ov\omega_\infty < \ov{b}_0$; so improvement occurs when the maximum variance $\ov\omega_\infty$ is smaller than the initial squared bias $\ov{b}_0$.}
\begin{align}
\label{ineq:improvement_msd4}
\ov{d}_\infty &< \ov{d}_0.
\end{align}
Next, using \eqref{eq:msd_0} and \eqref{eq:msd_inf} in \eqref{ineq:improvement_msd4}, we get
\begin{align}
\frac{\beta \ov{h} (M-1)}{2(\ov{h} - \beta \ov{h^2})} &< M v
\end{align}
and solving the resulting expression for $\beta$, leads to
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{ineq:improvement.condition}
% 0 < \beta < \frac{2 v \ov{h}}{(1-1/M) \ov{h} + 2 v \ov{h^2}} \approx \frac{1 }{1/(2 v) + \ov{h^2}/\ov{h}},
% 0 < \beta < \frac{1}{(1-1/M)/(2 v) + \ov{h^2}/\ov{h}}.
0 < \beta < \left[ \frac{(1 - 1/M)}{2v} + \frac{\ov{h^2}}{\ov{h}} \right]^{-1}.
\end{empheq}
Note that, assuming $M$ large, \eqref{ineq:improvement.condition} can be asymptotically approximated as
\begin{align}
% 0 < \beta < \frac{1}{1/(2v) + \ov{h^2}/\ov{h}}
0 < \beta < \left( \frac{1}{2v} + \frac{\ov{h^2}}{\ov{h}} \right)^{-1}
\end{align}
and, given that $\ov{h^2}/\ov{h}$ is limited to $[\sqrt{2}/8, 1/4]$ such that it can be ignored for small $v$, %(given that $\ov{h}/\ov{h^2}$ is limited to $[4, 4\sqrt{2}]$),
we have\footnote{In practice, $\beta$ is typically chosen smaller than \eqref{eq:improvement_over_small_v}. For example, \gls{fifa} \cite{fifa_ranking} uses $\beta\in[0.02,0.23]$ in football rankings and \gls{fide} \cite{fide} considers $\beta\in[0.06,0.23]$ in chess rankings. Note that these values have been obtained by scaling the step-size value $\beta'$ provided by either \gls{fifa} or \gls{fide} through $\beta = \beta'/s'$, with $s'$ defined in \eqref{scale-ln10}.}
\begin{align}\label{eq:improvement_over_small_v}
0 < \beta < 2v.
%\ls{0 < \beta < \frac{2v}{1+v/2}}
\end{align}
%\ls{which, for small values of $v$ may be expressed as $0 < \beta < 2v$.}

% FIFA: [0.01918821 0.23025851]
% FIDE: [0.05756463 0.23025851]

\figref{fig:improvement_over} plots the upper bound on the  step-size value $\beta$ given in \eqref{ineq:improvement.condition} as a function of $v$, considering $M = 15$ and $\eta = 0$. Other values of $M$ and $\eta$ have not been used, as they do not significantly affect \eqref{ineq:improvement.condition}. Notice that the upper bound on $\beta$ is lower as $v$ decreases, exhibiting an almost linear dependence on $v$; hence, \eqref{eq:improvement_over_small_v} holds as a rule of thumb. %for the upper bound on $\beta$
%Notice that \eqref{ineq:improvement.condition} is almost linear on $v$ (\ie the upper bound is lower as $v$ decreases) and thus \eqref{eq:improvement_over_small_v} holds as a rule of thumb for the upper bound on $\beta$.
Nevertheless, we emphasize that such a bound may be too loose and merely guarantees the improvement over initialization; therefore, in practice, it may be preferable to choose a smaller $\beta$ [than \eqref{eq:improvement_over_small_v}] especially when the number of games $k$ is limited.

% \ls{
% % Although \eqref{ineq:improvement.condition} establishes the upper bound on the step-size value $\beta$, we emphasize that such a bound may be too loose and merely guarantees the improvement over the initialization. 
% For a limited number of games $k$, it may be preferable to pick a smaller $\beta$ whose optimal value, as we have already seen in \figref{fig:loss_ex}, also depends on $k$.
% }

%the choice of $\beta$ should still take into account the number of games $k$ (as discussed later in \secref{sec:optimum_step}); for instance, if $\beta$ is too small, the rating algorithm may not be capable of reaching convergence within a given number of games $K$ (as already shown in Sections~\ref{sec:time}~and~\ref{sec:loss}).

\begin{figure}[t!]
\centering
\includegraphics[scale=1]{figures/discussion/improvement_over.pdf}\\
\caption{Condition on $\beta$ for improvement over initialization [given by \eqref{ineq:improvement.condition}] as a function of $v$, considering $M = 15$ and $\eta = 0$.}
%Curves for other values of $M$ and $\eta$ are omitted since these variables do not affect \eqref{ineq:improvement.condition} significantly.
\label{fig:improvement_over}
\end{figure}

\subsection{Optimum step-size value}\label{sec:optimum_step}

\begin{figure}[t]
\centering
\includegraphics[scale=1]{figures/discussion/optimal_beta.pdf}\\
\caption{Optimum step-size value $\beta_{{\tr{o}},k}$ obtained from the numerical solution of \eqref{eq:optimum-beta} (solid lines) and the approximate solution \eqref{eq:optimum_step} (dashed lines) as a function of the number of games $k$, considering different values of $v$ while $M = 15$ and $\eta = 0$. Curves for other values of $\eta$ are omitted since this variable does not significantly affect \eqref{eq:optimum_step}.}
\label{fig:optimal_beta}
\end{figure}

An optimum value for step-size $\beta$, considering a particular number of games $k$, can be determined to minimize \eqref{eq:v_k-final} [or, equivalently, the mean loss \eqref{eq:loss-behavior}]; specifically, we need to find a solution for the following optimization problem:
\begin{equation}\label{eq:optimum-beta}
\beta_{{\rm o}, k} = \argmin_{\beta}\; \ov{d}_k.
\end{equation}
Since a closed-form solution for \eqref{eq:optimum-beta} cannot be straightforwardly obtained for an arbitrary $k$, we resort to approximations (shown in \ref{Appendix.Step}) to obtain
\begin{align}\label{eq:optimum_step}
\beta_{\tr{o},k} &\approx \frac{1}{2} \left[ \frac{(1 - 1/M)}{2v} + \frac{\ov{h^2}}{\ov{h}} + \frac{2 \ov{h^2} (k - 1)}{M - 1} \right]^{-1}.
\end{align}

% Note that, when the number of games $k$ is small, \eqref{eq:optimum_step} reduces approximately to half of the upper bound given in \eqref{ineq:improvement.condition}, which for small $v$ becomes
% \begin{align}
% \beta_{\tr{o},1}\approx v;
% \end{align}
% this is also a good rule of thumb for choosing $\beta$ at the beginning of tournaments.

\figref{fig:optimal_beta} plots the optimal step-size value $\beta_{\tr{o},k}$ as a function of the number of games $k$, for  different values of $v$ while $M=15$ and $\eta=0$. We consider both the numerical solution of \eqref{eq:optimum-beta} and the approximate solution \eqref{eq:optimum_step}, and observe that 
\begin{itemize}
\item The results calculated from \eqref{eq:optimum_step} match very well with those determined from the numerical solution of \eqref{eq:optimum-beta} regardless of $v$ and $k$, thus confirming the practicality of the approximate solution we obtained.

\item The optimal step size $\beta_{\tr{o},k}$ exhibits a decreasing characteristic with respect to the number of games $k$, \ie larger step sizes are needed to improve the convergence of the rating algorithm when $k$ is small. 

\item %\ls{Considering the league seasons where the teams play each of the other teams at home and away so the total number of games is approximately $M^2$, }
The impact of $v$ on the choice of the step-size value is more significant than the number of games $k$; in particular, for small $v$, $k$ can be neglected, and we can use $\beta_{\tr{o},k}\approx v$.
%\cred{I'm not sure it is true. Is it because we set only show $k\approx 210$ games?  if we use the formulas for $\ov{h^2}$ and set $k=M^2$, what happens? it seems there will be an interplay between $v$ and $M$.}
\end{itemize}
\noindent
Therefore, the choice of the step-size value $\beta$ should be made carefully depending on the competition scenario.

%if the value of $\beta$ is too low, a team’s rating will not change quickly enough when it improves its performance, while if the value of $\beta$ is too high, the rating will be unreliable, changing too much from one match to another.

==> old/Experimental.tex <==
%\section{Experimental results}\label{Sec:experimental_results}
\section{Application on real-world data}\label{Sec:experimental_results}
%\ls{Aiming to assess the accuracy of the analysis and the relevance of the model proposed in \secref{Sec:analysis}, the results produced by the algorithm are now compared to the analytical expressions we obtained.} %those obtained by running the rating algorithm [given in \eqref{eq:rating-sgd2}] on the empsirical data.} to those obtained by using the analytical the behavior described by the model expressions. 

To assess the accuracy of the expressions derived from our analysis, the results produced by running the rating algorithm [given in \eqref{eq:rating-sgd2}] are compared to the behavior described through the proposed model\footnote{The code used in the experiments is available at \url{https://github.com/dangpzanco/elo-rating}.}. To this end, we use real-world data from the Italian professional volleyball league (SuperLega), spanning 10 seasons from 2009/10 to 2018/19, whose results are available on FlashScore's website \cite{flashscore.ca}. In particular, we consider only the regular season games and neglect the playoffs at the end of each season; by doing so, we guarantee that all teams play the same number of games against each other, and, hence, modeling the scheduling as uniform is appropriate (\ie the regular season is a home-away, round-robin tournament). Note that the aim is to verify whether our analysis characterizes well the behavior of the rating algorithm for a known operating scenario, thus ratifying the insights discussed from our analysis.

%\cred{This part will go or stay depending how we decide to deal with the cross-validation}

The \gls{hfa} parameter $\eta$ (used in the rating algorithm) and the variance of the skills $v$ (required in the stochastic model) are assumed known a priori in each season so that $\ov{h}$ [see \eqref{mean-h_k}], $\ov{h^2}$ [see \eqref{mean-h_k^2}], and $\ov\ell_{\rm min}$ [see \eqref{eq:l_min}] can be properly computed to validate the analysis. Specifically, $\eta$ may be treated as a parameter along with $\btheta$ in \eqref{ML.optimization} and, hence, both of them can be estimated by using any popular machine-learning approach \cite{goodfellow-deeplearning}, yielding thus $\hat\eta$ and $\hat\btheta$; once $\hat\btheta$ is obtained, we can determine $\hat{v}$ directly from its (unbiased) sample variance, since the scheduling is uniform\footnote{In a more general scenario, $v$ should be determined as half the sample variance of $z_k^*$ instead.}. Note that we have used here the \gls{sg} optimization method with a very-small step size and a large number of epochs.

%, such that the uncertainty (random fluctuations) around $\btheta_k$ becomes negligible \ls{[if we say that we calculate $\hat\btheta$ then it means that we solve \eqref{ML.optimization}. Therefore, we do not need to talk about uncertainty of the numerical procedure we decided to apply.]}.

%\dz{such that the excess loss $\ov\ell_{\tr{ex},k}$ is negligible in comparison to the lower-bound of the loss $\ov\ell_\tr{min}$}.


% In turn, an estimate of $v$ is determined from the sample variance of the true skills vector $\btheta^*$ which is also obtained by solving \eqref{ML.optimization} via batch gradient descent \cite[Sec.~8.1]{goodfellow-deeplearning}, \ie 

% (\eg \cite{scikit-learn})

% Although the true skills vector $\btheta^*$ is not readily available, it is required in the derived model expressions describing the behavior of the rating algorithm. In this sense, $\btheta^*$ is determined here, for each season, by solving the optimization problem \eqref{ML.optimization} via batch gradient descent with a small \dz{learning rate} ($\beta = 0.001$) and a large number of iterations (10000 iterations). 

% To find the hyper-parameters, $\hat{v}$ and $\hat{\eta}$ that provide the best explanation for the observed data, we will use the \gls{loo} cross-validation; it is  an unambiguous methodology also implemented in popular most machine learning packages \cred{\cite{Scikit}}.

% Alternatively, it might be assumed that each season is characterized by its own hyper-parameters $\hat{v}^{(t)}$ and $\hat{\eta}^{(t)}$.

% In this sense, $\eta$ is estimated here, based on \cite{Szczecinski20}, as
% \begin{align}
% % \eta &= \sigma^{-1}(\PR{Y_k=1})\\
% % \eta &\approx \sigma^{-1}\left( \frac{1}{K} \sum_{k=1}^{K} y_k \right)
% \eta &\approx \ln\left[ \frac{\displaystyle\sum_{k=1}^{K} y_k}{\displaystyle\sum_{k=1}^{K} (1 - y_k) }  \right]
% \end{align}
% which characterizes a ratio between the probabilities of winning and losing at home. 

% The variance of the skills $v$, and  the \gls{hfa} $\eta$ may be treated as hyper-parameters of the model and we may find them by a conventional machine-learning approach. 
% Namely, assuming that the skills are drawn from a Gaussian distribution amounts to 
% transforming the \gls{ml} problem \eqref{ML.optimization} into the \gls{map} estimation, \ie finding the mode of the posterior distribution via the following optimization
% \begin{align}
% \label{map.optimization}
%     \hat\btheta^{*,(t)}
%     &=
%     \argmin_{\btheta}
%     \sum_{k=1}^{K^{(t)}} \ell_k^{(t)}(\btheta) + \frac{1}{2v}\|\btheta\|^2,
% \end{align}
% where the term $\frac{1}{2v}\|\btheta\|^2 $ represents the log-domain Gaussian prior and the index $^{(t)}$ refers to the data in the $t$-th season, $t=1,\ld, T$ with $T=10$ seasons. In fact, we may see \eqref{map.optimization} as a regularization method used already before, \eg in \cite{Gramacy13}, \cite{Szczecinski22b}. 

% Note that the variance $v$ plays the role of the regularization parameter, $\eta$ enters the optimization via the likelihoods $\ell^{(t)}_k(\btheta)$ per \eqref{eq:loss_k}, and the solution $\hat\btheta^{*,(t)}$ is an estimate of the hypothetical exact skills $\btheta^{*,(t)}$ generated in the season $t$.\footnote{Due to the regularization, the solution of \eqref{map.optimization} is not the same as the \gls{ml} solution \eqref{ML.optimization}.}

% \cred{I suppose that, showing the evolution of the skills $\btheta_k$, or the \gls{msd}, we may have a mismatch between the theoretical curves and the experimental ones. I remember from our discussion that you were concerned with this. However, I note that we do not have any theoretical result saying that $\btheta_k$ converges to $\hat\btheta$, we rather say that $\btheta_k$ converges to $\btheta^*$. And we have no particular reason to say that $\btheta^*\approx\hat\btheta$ rather than using the estimate from \eqref{map.optimization}, \ie $\btheta^*\approx\hat\btheta^{*}$.}


% Note that, in \eqref{map.optimization} we assumed that the skills of the teams in all observed seasons are drawn from the distribution characterized by the same hyper-parameters $v$ and $\eta$.



% However, in our view, the advantage of the former approach is that, by using the same parameters we considered them as proper to the competition we analyze.

% As we can see in \tabref{tab:summary}, using the same $\hat{v}=XXX$ and $\hat{\eta}=YYY$, we provide a well-defined method to ``average'' the hyper-parameters $\hat{v}^{(t)}$ and $\hat{\eta}^{(t)}$, which, although vary across the seasons, are rather similar.


% \ls{We emphasize that \eqref{map.optimization} is solely used to obtain the hyper-parameters of $v$ and $\eta$. On the other hand, for the illustration purpose we will also obtain the parameters $\hat\btheta^{(t)}$ via \eqref{ML.optimization} we solved via a batch gradient descent \cite[Sec.~8.1]{goodfellow-deeplearning}).}


A summary of \mbox{SuperLega}'s data is presented in \tabref{tab:summary}, highlighting the number of teams $M$ and games $K$ along with the estimated values of the \gls{hfa} parameter $\eta$ and the variance of skills $v$. Notice that $M$ varies (within the range of 12 to 15); as a consequence, $K$ changes (from 132 to 210 games) depending on the considered season. In addition to these aspects, one can observe that the estimated values of $\eta$ and $v$ do not change significantly; in practice, these values could be estimated from the results of previous tournaments.


\begin{table}[t!]
\centering
\caption{Summary of the SuperLega's dataset.}
\label{tab:summary}
\medskip
\begin{tabular}{@{}ccccc@{}}
\toprule
Season    & $M$ & $K$ &  $\hat\eta$  &   $\hat{v}$    \\ \midrule
% 2009 & 15 & 210 & 0.662625 & 2.738321 \\
% 2010 & 14 & 182 & 0.321430 & 1.576293 \\
% 2011 & 14 & 182 & 0.348231 & 1.222075 \\
% 2012 & 12 & 132 & 0.402100 & 1.916473 \\
% 2013 & 12 & 132 & 0.551887 & 1.307860 \\
% 2014 & 13 & 156 & 0.469551 & 2.932582 \\
% 2015 & 12 & 132 & 0.055876 & 2.364083 \\
% 2016 & 14 & 182 & 0.771591 & 2.373615 \\
% 2017 & 14 & 182 & 0.223695 & 3.023535 \\
% 2018 & 14 & 182 & 0.485662 & 3.683417 \\ 
2009 & 15 & 210 & 0.66 & 2.7 \\
2010 & 14 & 182 & 0.32 & 1.6 \\
2011 & 14 & 182 & 0.35 & 1.2 \\
2012 & 12 & 132 & 0.40 & 1.9 \\
2013 & 12 & 132 & 0.55 & 1.3 \\
2014 & 13 & 156 & 0.47 & 2.9 \\
2015 & 12 & 132 & 0.06 & 2.4 \\
2016 & 14 & 182 & 0.77 & 2.4 \\
2017 & 14 & 182 & 0.22 & 3.0 \\
2018 & 14 & 182 & 0.49 & 3.7 \\ 
\bottomrule
\end{tabular}
\end{table}


% Season    & $M$ & $K$ &  $\eta$  &   $v$    \\ \midrule
% 2009/10   & 15  & 210 & 0.346276 & 2.461513 \\
% 2010/11   & 14  & 182 & 0.220671 & 1.546726 \\
% 2011/12   & 14  & 182 & 0.242946 & 1.193692 \\
% 2012/13   & 12  & 132 & 0.243622 & 1.847960 \\
% 2013/14   & 12  & 132 & 0.367725 & 1.229153 \\
% 2014/15   & 13  & 156 & 0.231802 & 2.768929 \\
% 2015/16   & 12  & 132 & 0.030305 & 2.362341 \\
% 2016/17   & 14  & 182 & 0.423814 & 2.071665 \\
% 2017/18   & 14  & 182 & 0.110001 & 2.983370 \\
% 2018/19   & 14  & 182 & 0.220671 & 3.458560 \\ \bottomrule


\subsection{Example 1}

% [0.03, 0.87, 2.49]

This example aims i) to assess the ability of the proposed model to characterize the behavior of the rating algorithm; and ii) to show how $\beta$ affects the \gls{msd} of the skills \eqref{eq:v_k-final} and the mean loss function \eqref{eq:loss-behavior}. To this end, different step-size values are used, namely: $\beta=0.1$ (within the range suggested by \cite{fifa_ranking,fide}), $\beta=0.87$ [obtained by averaging the optimum step-size value \eqref{eq:optimum_step} with $k=K/4$ for all seasons], and $\beta=2.49$ [determined by averaging the condition to improve over initialization \eqref{ineq:improvement.condition} for all seasons]. Note that the rating algorithm is run for each season and the mean behavior is computed (over the seasons) by truncating the number of games to the shortest season ($K=132$).

\figref{fig:exp_metrics} presents the evolution of the \gls{msd} of the skills and the mean loss function, considering $\beta=0.1$ [Figs.~\ref{fig:exp_metrics}(a)~and~(b)], $\beta=0.87$ [Figs.~\ref{fig:exp_metrics}(c)~and~(d)], and $\beta=2.49$ [Figs.~\ref{fig:exp_metrics}(e)~and~(f)]. Notice from these figures that the proposed model describes very well the behavior of the rating algorithm in the transient- and steady-state phases, irrespective of the considered step-size values. In addition to this aspect, from Figs.~\ref{fig:exp_metrics}(a)~and~(b), one can observe that the rating algorithm is not capable of reaching convergence until the end of the season for small values of $\beta$ (as suggested by \cite{fifa_ranking,fide}). In turn, when $\beta$ is adjusted according to the optimal step-size value [given by \eqref{eq:optimum_step}] assuming $k$ equal to a quarter of the season (\ie $k=K/4$ games), it can be verified that the convergence speed of the rating algorithm is significantly improved [as shown in Figs.~\ref{fig:exp_metrics}(c)~and~(d)]; in this condition, the algorithm reaches the optimal solution within $K$ games. Lastly, if we increase $\beta$ to the threshold derived as improvement over initialization [defined by \eqref{ineq:improvement.condition}], little to no improvement is observed as $k$ increases [as depicted in Figs.~\ref{fig:exp_metrics}(e)~and~(f)]. Therefore, we verify that the convergence of the rating algorithm is affected by the choice of $\beta$, ratifying the relevance of \eqref{eq:optimum_step}.



\begin{figure}[t]
\centering
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/msd_beta0.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/loss_beta0.pdf}}\\
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/msd_beta1.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/loss_beta1.pdf}}\\
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/msd_beta2.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/metrics/loss_beta2.pdf}}\\
\caption{Example 1. Evolution of the \gls{msd} of the skills (left) and the mean loss function (right) obtained from simulation results (gray-solid lines) and proposed model (dark-dashed lines), considering (a)~and~(b)~$\beta = 0.1$, (c)~and~(d)~$\beta = 0.87$, and (e)~and~(f) $\beta = 2.49$. %\dz{another line with $K = 3\tau$}
}
\label{fig:exp_metrics}
\end{figure}


\subsection{Example 2}
In this example, the main goals are i) to assess the accuracy of the model expressions derived characterizing the \gls{msd} \eqref{eq:v_k-final} and the mean loss  \eqref{eq:loss-behavior} when $k$ increases to the end of the season; ii) to investigate the impact of step-size $\beta$ on the \gls{msd} and loss; and iii) to verify the practical applicability of the design guidelines provided about the choice of $\beta$ (as discussed in Section~\ref{Sec:Discussion}). To this end, we consider different values for the step-size, \ie $\beta\in(0.01, 4)$. Note that the rating algorithm is run for each season and the mean behavior is computed (over the seasons) by truncating the number of games to the shortest season ($K=132$) and averaging the last 10 samples of the variable of interest, in order to provide a better visualization of the experimental results. 


% We evaluate the behaviour near the largest possible number of games across seasons $k=\min_{t}{K^{(t)}}=132$ and the estimates of the loss $\ov{\ell}_k$ and the \gls{msd} $\ov{d}_k$ obtained by averaging 
% \begin{align}
%     \ov{\ell}_{k} 
%     \approx &
%     \frac{1}{LT}\sum_{t=1}^T\sum_{n=k-L+1}^k \ell_n^{(t)}\\
%     \ov{d}_k 
%     \approx &
%     \frac{1}{LT}\sum_{t=1}^T\sum_{n=k-L+1}^k d_n^{(t)},
% \end{align}
% where $d_k=\tilde{\btheta}_k\T\tilde\btheta_k$ is the squared deviation, and the averaging window size is $L=10$.

\figref{fig:exp-steady} depicts the results obtained for the \gls{msd} [\figref{fig:exp-steady}(a)] and mean loss [\figref{fig:exp-steady}(b)] as a function of $\beta$. Based on these figures, one can draw the following conclusions: First, the proposed model describes very well the behavior of the rating algorithm (when approaching the end of the season) over a wide range step-size values $\beta$.  Second, step-size values exceeding ``improvement over initialization'' [given  by \eqref{ineq:improvement.condition}] imply a high uncertainty of the skill estimates and predictions (\gls{msd} and loss, respectively); therefore, such values of $\beta$ should not be used. Third, adjusting $\beta$ according to the optimal step-size value [given by \eqref{eq:optimum_step}] allows achieving a value of \gls{msd} and loss very close to their minimum within a certain number of games $k$. Therefore, the design guidelines provided in Section~\ref{Sec:Discussion} also hold on empirical data and should be taken into account in practice.



% Fourth, for a relatively small number of games (as occurs in the professional sport leagues), $\beta$ needs to be properly adjusted [\eg using \eqref{eq:optimum_step}] in such a way that the rating algorithm converges before reaching the end of the season.



% The \gls{msd} is shown in  \figref{fig:exp-steady}(a) while the mean loss function, in \figref{fig:exp-steady}(b) and the main conclusions are
% \begin{itemize}
% \item The results predicted through the proposed model match very well with the behavior of the rating algorithm for a large range of considered step-size $\beta$.    
% \item Design guidelines discussed in \secref{Sec:Discussion} are confirmed on empirical data. Namely:
%     \begin{itemize}
%     \item Step-size values exceeding ``improvement over initialization'' \eqref{ineq:improvement.condition} imply very high uncertainty on the skills and predictions; hence, such values of $\beta$ are not useful in practice [see, e.g., Figs.~\ref{fig:exp_metrics}(e)~and~(f)]
%     \item Adjusting $\beta$ according to the optimum step-size value given by \eqref{eq:optimum_step} allows achieving a value of \gls{msd} and loss very close to their minimum.    
%     \end{itemize}
% \end{itemize}

% Quite obviously, for a relatively small number of games, a scenario which materializes in the professional sport leagues, $\beta$ needs to be properly adjusted [\eg using \eqref{eq:optimum_step}] in such a way that the rating algorithm converges before reaching the end of the season.

\begin{figure}[t]
\centering
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/steady/steady_state-msd.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/steady/steady_state-loss.pdf}}\\
\caption{Example 2. Values of (a) \gls{msd} and (b) mean loss achieved by the rating algorithm as $k$ approaches $K$ obtained from simulation results (gray-solid lines) and proposed model (dark-dashed lines), considering different step-size values $\beta$. Vertical lines indicate the upper bound of the improvement over initialization condition \eqref{ineq:improvement.condition} (dark-solid line) and the optimum step-size value \eqref{eq:optimum-beta} for $k=K$ (dark dash-dotted line).}
\label{fig:exp-steady}
\end{figure}


%\newpage


\subsection{Example 3}
% 1.26914615, 0.9611244 , 1.23993294, 1.50551097
Our goal here is to show that the derived stochastic model explains well the evolution of the estimate of the skills $\btheta_k$ [through \eqref{eq:skill-behavior}] and \gls{msd} of the skills [given in \eqref{eq:v_k-final}]. Also, we aim to verify the impact of the data from different seasons on the ability of the derived model to describe the behavior of the rating algorithm.
%Here, we aim i) to assess the accuracy of the proposed model characterizing the evolution of the skills [given in \eqref{eq:skill-behavior}] and the \gls{msd} of the skills [given in \eqref{eq:v_k-final}]; and ii) to verify the impact of the data of different seasons on the rating algorithm and proposed model. To this end, 
Specifically, for the sake of visualization, the algorithm is evaluated using data from seasons 2009/10, 2010/11, 2015/16, and 2018/2019, and we use the optimum step-size value computed [from \eqref{eq:optimum_step}] at $k=K/4$ for each season (for the sake of simplicity). %\cred{I use the notation $k_\tr{t}$ to denote the ``target'' $k$, for which we optimize the step size. Otherwise it may be confusing.} 
Note that, instead of analyzing the averages over the seasons, we compare the results of a single run of the algorithm (which is a realization of a random process) to its mean behavior described from the model.
%while $\eta$, $v$, and $M$ are given in Table~\ref{tab:summary}] for each of these seasons as 0.88, 0.71, 0.93, and 1.06, respectively. Note that a single run of the rating algorithm for each season is now compared with results predicted through the proposed model.

% 0.88395081 0.7092163  0.93009523 1.06002658

% \cred{and iii) to discuss about the convergence of the skills based on the derived time constant \eqref{tau.1} (see Section~\ref{sec:time}).}

% \dz{Change the description (new figures):}

\figref{fig:exp_seasons} presents the evolution of skills (for four selected teams) \dz{(Comment 14)} and their \gls{msd} obtained by running the rating algorithm and through the derived model. Specifically, results for seasons 2009/10 [Fig.~\ref{fig:exp_seasons}(a)~and~(b)], 2015/16 [Fig.~\ref{fig:exp_seasons}(c)~and~(d)], 2017/18 [Fig.~\ref{fig:exp_seasons}(e)~ and~(f)], and 2018/19 [Fig.~\ref{fig:exp_seasons}(f)~and~(g)] are shown. Notice that the evolution of the skills obtained by running the algorithm have a staircase-like form\footnote{When averaging over different realizations of the scheduling, the staircase form would be replaced by the exponential form of the mean of skills $\Ex[\theta_m]$.} due to a particular realization of the scheduling, \ie the skills remain constant when the team is not playing.
%In addition, it is important to remark that the evolution of the skills exhibits a piecewise constant nature due to the game schedules, \ie the skills remain constant when the corresponding teams are not playing against any other. Moreover, these figures confirm that the choice of the step-size value based on \eqref{eq:optimum_step} with $k=K/4$ yields a very good convergence characteristic for the rating algorithm.
% establish [based on \eqref{tau.1}] the transient and steady-state phases of the rating algorithm for each season (see the vertical lines in Fig.~\ref{fig:exp_seasons}). Notice that the teams skills clearly evolve until reaching the specified number of games while exhibit an ``almost" constant characteristic after such number of games. Hence, we infer also that \eqref{tau.1} characterizes very well the number of games required for the rating algorithm to achieve convergence. 
Observe also that, while the estimates $\btheta_k$ are random (owing to random outcome and scheduling of games), the analytical expressions proposed for the mean of skills $\Ex[\btheta_k]$ as well as their \gls{msd} become a practical proxy for $\btheta_k$ and $\ov{d}_k$ regardless of the considered season. Therefore, we conclude that the proposed model characterizes well the behavior of the rating algorithm, which validates the applicability of the design guidelines discussed so far (given in Section~\ref{Sec:Discussion}).


% Color order: blue, orange, green, red
% 2009 3*tau = 124 ['Pineto' 'Taranto' 'Monza' 'Trentino']
% 2010 3*tau = 130 ['Forli' 'Piacenza' 'Monza' 'Trentino']
% 2015 3*tau = 98 ['Piacenza' 'Ravenna' 'Verona' 'Lube Civitanova']
% 2018 3*tau = 110 ['BCC-NEP Castellana' 'Ravenna' 'Verona' 'Lube Civitanova']

% \dz{Make the same figures with \gls{msd}.}


% \begin{figure}[t!]
% \centering
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/skills-season2009.pdf}}
% \quad
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/skills-season2010.pdf}}\\
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/skills-season2015.pdf}}
% \quad
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/skills-season2018.pdf}}
% \caption{Example 3. Evolution of the skills (left) and \gls{msd} (right) obtained from simulation results (solid lines) and proposed model (dashed lines), considering season (a) 2009/2010, (b) 2010/2011, (c) 2015/2016, and (d)~2018/2019. Vertical lines indicate the theoretical number of games [given by \eqref{tau.1}] required to achieve $95\%$ of its final value.%, which yields (a) 124 games, (b) 130 games, (c) 98 games, and (d) 110 games.
% \dz{Put custom ticks showing the last game index; include time constant as a vertical line, ticks}}
% \label{fig:exp_seasons}
% \end{figure}


\begin{figure}[hb!]
\centering
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/skills-season2009.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/msd/msd-season2009.pdf}}\\
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/skills-season2015.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/msd/msd-season2015.pdf}}\\
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/skills-season2017.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/msd/msd-season2017.pdf}}\\
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/skills-season2018.pdf}}
\quad
\subfloat[]{\includegraphics[width=0.48\textwidth]{figures/experiments/seasons/msd/msd-season2018.pdf}}
\caption{Evolution of the skills for a subset of 4 teams (left) and \gls{msd} of the skills (right) obtained from simulation results (solid lines) and proposed model (dashed lines), considering season (a)~and~(b) 2009/10, (c)~and~(d) 2015/16, (e)~and~(f) 2017/18, and (f)~and~(g) 2018/19.}
% the 2009/10 season ($K=210$, left side of the figure) and the 2015/16 season ($K=132$, right side). We use $\hat\beta$ obtained by solving $3\tau_1=K$, see \eqref{tau.1} (a) and (b); for $2\hat\beta$ (c) and (d), and for $0.5\hat\beta$ (e) and (f).
\label{fig:exp_seasons}
\end{figure}



% \begin{figure}[t!]
% \centering
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/loss/loss-season2009.pdf}}
% \quad
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/loss/loss-season2010.pdf}}\\
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/loss/loss-season2015.pdf}}
% \quad
% \subfloat[]{\includegraphics[width=0.48\textwidth]{figures/exp_seasons/loss/loss-season2018.pdf}}
% \caption{Example 3. Evolution of the loss obtained from simulation results (solid lines) and proposed model (dashed lines), considering season (a) 2009/2010, (b) 2010/2011, (c) 2015/2016, and (d)~2018/2019. Vertical lines indicate the theoretical number of games [given by \eqref{tau.1}] required to achieve $95\%$ of its final value.%, which yields (a) 124 games, (b) 130 games, (c) 98 games, and (d) 110 games.
% \dz{Put custom ticks showing the last game index; include time constant as a vertical line, ticks}}
% \label{fig:exp_seasons}
% \end{figure}


==> old/Introduction.tex <==
\section{Introduction}

Over the recent decades, different ranking/rating algorithms have been devised and used in tournaments/competitions (sports and games) to assign numbers to teams (or players in the case of individual sports) \cite{stefani2011}. The rating consists of assigning a numerical value to a competitor based on empirical observations (of the game outcomes), while the ranking is obtained by sorting the rating values \cite{stefani2011}; so, a ``stronger" team has a large rating and is ranked before the weaker team \cite{barrow2013}. Hence, the rating, which reflects the skills/abilities/strength of each team compared to the others (see the extensive surveys in \cite{stefani2011,barrow2013,lasek2021,Csato2021}), can be used to obtain quick information on the state of a tournament, to assess the strength of teams, to decide on seeding/pairing (defining game schedules with more ``interesting'' matches) or promotion/relegation (between high- and low-level leagues) \cite{lasek2021}, as well as to provide support for both bookmakers and gamblers \cite{hvattum2010,wolf2020}. As a consequence of practical applicability, the development and refinement of rating\footnote{The problem of rating falls into the topic of ``paired comparison'' modeling in the field of statistics \cite{BradleyTerry52,Glickman93_thesis,leitner2010}.} systems have become an important and active research field (as properly summarized, \eg through \cite{vaughanwilliams2010} and \cite{mchale2019} and references therein).

From a statistical perspective, the rating consists of inferring unknown parameters (skills) from the observed outcomes (game results) via a formal mathematical model of skills-outcomes (see \cite[Ch.~4]{dobson2011} for details on goal- or result-based models, and \cite[Appendix]{stekler2010} for a sport-by-sport discussion). In this sense, the Elo algorithm (or Elo rating system), devised in the 1960s \dz{by the Hungarian-American physics professor Arpad Elo (???)} to rate chess players \cite{Elo78_Book}, is arguably the most well-known and widely used, mainly due to its simplicity and intuitive interpretation \cite{lasek2021}. This algorithm assumes that each team has a ``single'' parameter governing its performance (\ie ``its true strength'') and then the goal is to provide an estimate of such a parameter (\ie ``a rating"); to this end, the algorithm increases the skills of a particular team when the score of the game is larger than the expected/predicted one and vice versa \cite{Elo78_Book}, thus updating (after each match) the rating of the teams depending on the game outcomes \cite{barrow2013,ryall2010}. Therefore, the self-correcting characteristic of the algorithm allows it to (intrinsically) track the skills of the teams over time \cite{glickman1995}.

The Elo algorithm has become a reference and has been adopted for rating in chess by \gls{fide} \cite{fide}, or, in association football (soccer), for ranking of the national Women's teams in 2003 \cite{fifa_rating_W} and Men's teams in 2018 \cite{fifa_ranking} by \gls{fifa}, among others \cite{play-pokemon,Silver14,carbone2016,FiveThirtyEight}. I was also used for simulation of sports tournaments \cite{Chater2021,Csato2022,Csato2023}. Extensions and variations of the (original) Elo algorithm have also been derived and applied to various other sports, as discussed, among others, in \cite{Glickman1999,Herbrich06,leitner2010,ryall2010,lasek2013,dorsey2019,kovalchik2020,wolf2020,Szczecinski20,lasek2021,wheatcroft2021,Szczecinski22}. \dz{(Comment 5 here) For example, }. Despite the widespread use of the Elo algorithm, the discussions presented so far in the literature have generally been based on empirical studies. This is especially true with respect to the choice of the step-size value (which is the only hyperparameter of the algorithm) that differs significantly from one application to another (\eg see \cite[Table~10]{stefani2011} and \cite[Sec.~3]{lasek2013}). In fact, to the best of our knowledge, a theoretical analysis of the convergence of the Elo algorithm has only been discussed in \cite{jabin2015}, which demonstrates that the estimates of skills converge to their ``true strengths" at an exponential rate in a round-robin (all-meet-all) tournament \cite[Theorem~2.2]{jabin2015}. \dz{(Comment 4) xxxx.} However, as pointed out critically by \cite{kovalchik2020}, further theoretical studies of the Elo algorithm, as well as its extensions and variations, would still be valuable. 

In this context, the present research work aims to obtain a stochastic model for characterizing the Elo algorithm, considering round-robin tournaments; particularly, aiming to gain more insights into the algorithm and avoid resorting to extensive numerical simulations, our approach relies on using mathematical tools from the area of adaptive filters. In summary, we aim to address the following aspects:
\begin{itemize}
\item To provide a comprehensive mathematical framework to analyze the Elo algorithm applied in a round-robin tournament;

\item To obtain analytical expressions characterizing the evolution of skills (along with other important performance metrics) throughout a tournament;

\item To investigate the impact of the hyperparameters on the performance of the algorithm, aiming to obtain useful insights and design guidelines; and

\item To compare the analytical results with those obtained through the algorithm using real-world data (from the Italian SuperLega, Volleyball League) illustrating the applicability of the theoretical findings.
\end{itemize}

The remainder of this paper is organized as follows. Section~\ref{Sec:Model} revisits some fundamental concepts related to the rating model and the Elo algorithm. Section~\ref{Sec:analysis} presents the proposed stochastic analysis for the Elo algorithm. Section~\ref{Sec:Discussion} discusses some interesting insights and design guidelines obtained from the analysis. Section~\ref{Sec:experimental_results} presents experimental results based on data extracted from the Italian league of volleyball. Lastly, conclusions and suggestions for future research works are summarized in Section~\ref{Sec:Conclusions}.

The mathematical notation adopted in this paper follows the standard practice of using lower-case boldface letters for vectors, upper-case boldface letters for matrices, and italic letters for scalar quantities. Superscript $\mf{T}$ stands for the transpose operator, $\Ex(\,\cdot\,)$ denotes the expected value operator which (unless otherwise stated explicitly) is calculated with respect to all random variables appearing inside parenthesis/brackets, while $[\mathbf{A}]_{m,n}$ represents the scalar $m,n$-entry of matrix $\mathbf{A}$. Still, when dealing with probabilities, we abused the notation to write simply $\PR{a|b}$ instead of $\PR{A=a|b}$ with $A$ denoting the random variable itself and $a$ its realization conditioned on $b$.

==> old/Model.tex <==
% \section{Model and simplifications}\label{Sec:Model}

\section{Problem statement}\label{Sec:Model}

Here, we first introduce the rating model along with some fundamental concepts, and then present a recursive algorithm that is used to solve the rating problem.

\subsection{Rating model}
Let us consider $M$ teams (with index $m=1,\ld, M$) playing against each other in a round-robin tournament/competition (see \citep{Szymanski2003,scarf2006,Scarf2009,Lasek2018,Csato2021} for detailed discussions on tournament design) with games indexed through $k=1,\ld,K$, where $K$ is the total number of games observed in a given period of time (\eg the number of games in a season). In each game $k$, opponents are scheduled by an external mechanism that assigns ``home'' and ``away'' indices ($i_k$ and $j_k$, respectively) to the teams. The distinction between home and away teams is particularly useful in tournaments in which \gls{hfa}\footnote{\dz{(Comment 6)}} is present, \ie when playing at home increases the probability of winning (for details, see \cite[Sec.~2]{ryall2010}). The results of the games are denoted as $y_k \in \{0,1\}$ with $y_k = 1$ when the home team wins and $y_k = 0$ otherwise.


In the rating problem, we are interested in finding the skills of the teams $\btheta = [\theta_1,\ld,\theta_M]\T$ that make it possible to directly compare the abilities of the $M$ teams. Statistical inference of skills $\btheta$ from observed outcomes $y_k$ requires a model that relates both quantities. To this end, we adopt the popular Bradley---Terry model \cite{BradleyTerry52}
\begin{align}\label{Pr.y.1}
\PR{y_k = 1|\btheta} &= \sigma(z_k/s + \eta)
\end{align}
which relies on the difference between the skills of the playing teams
\begin{align*}
z_k &= \theta_{i_k} - \theta_{j_k}\\
    &= \bx_k\T \btheta \numberthis \label{z_k}
\end{align*}
%It is convenient to express \eqref{z.k.initial} as
% \begin{align*}\label{z_k}
% \numberthis    
% z_k &= \bx_k\T \btheta
% \end{align*}
with the scheduling vector $\bx_k=[x_{k,1}\;\ldots\; x_{k,M}]\T$ defined as
\begin{align} \label{eq:schedule_vector}
x_{k,m} =
\begin{cases}
1,&  m = i_k \\
-1,& m = j_k \\
0,&  \text{otherwise}
\end{cases}
\end{align}
%Note in \eqref{Pr.y.1} that
while
\begin{align}\label{logit}
\sigma(z) = \frac{1}{1+\e^{-z}}
\end{align}
is the logistic function and $\eta$ plays the role of the \gls{hfa} parameter (capturing the increased probability of the home-team winning).

% ; also, the choice of the exponent base in \eqref{logit} is equivalent to a change in the scaling factor

Note that $s > 0$ in \eqref{Pr.y.1} and the exponent base in \eqref{logit} are arbitrary scaling factors used to stretch/accommodate the value of the skills to a desirable range, \eg
\begin{align*}
\sigma(z/s) &= \frac{1}{1+\e^{-z/s}}\\
&= \frac{1}{1+10^{-z/s'}}\numberthis \label{logit10}
\end{align*}
where
\begin{align}
\label{scale-ln10}
s' &= s\ln(10).
% &\approx 2.3 s. \numberthis \label{scale-ln10}
\end{align}
Therefore, \eqref{logit10} links the logistic function \eqref{logit} to the base-10 function commonly used in the Elo rating, ratifying that the change of scale can be seen as a change of the base of the exponent (as also noted in \cite{leitner2010}); henceforth, for the sake of simplicity, we consider $s = 1$.


\subsection{Rating problem and algorithm}\label{Sec:rating.problem}

Taking into account the total number of games $K$, as well as assuming that the home-field advantage $\eta$ and the scheduling vectors $\bx_k$ are known, the problem at hand is to estimate the skills $\btheta$ from the game outcomes $y_k$. To solve this problem, which can be interpreted as a logistic regression problem \cite[Ch.~4.4]{Hastie_book}, we can resort to the \gls{ml} principle to write
\begin{align}\label{ML.optimization}
\hat\btheta = \argmin_{\btheta}\; \sum_{k=1}^{K} \ell_k(\btheta)
\end{align}
with the negative log-likelihood function (also known as loss function) given by
\begin{align}\label{eq:loss_k}
\nonumber
\ell_k(\btheta) &= -\ln[\PR{y_k | \btheta}]\\
&= -y_k \ln[\sigma(\bx_k\T\btheta+\eta)] - (1 - y_k) \ln[1 - \sigma(\bx_k\T\btheta+\eta)].
\end{align}
A solution for \eqref{ML.optimization} can be found recursively through the \gls{sg} optimization method (as described in \cite{lasek2021}), \ie
\begin{align}
%\label{eq:rating-sgd}
\nonumber
\btheta_{k+1} &= \btheta_{k} - \beta \nabla \ell_k(\btheta_k) \\
\label{eq:rating-sgd2}
&= \btheta_{k} + \beta [y_k - \sigma(\bx_k\T \btheta_k+\eta)] \bx_k
\end{align}
with $\beta > 0$ denoting the step-size parameter and $\btheta_0$ being conveniently initialized as an $M$-dimensional vector of zeros. Note that \eqref{eq:rating-sgd2} describes how the ratings are updated after each game $k$ and represents exactly the Elo algorithm described in \cite{Elo78_Book}. 
\dz{An illustrative example would be useful to highlight how the rantings are updated in practice.}


\begin{itemize}
\item $M = 5$
\item $\btheta = [0.5, 0.1, -0.4, 0.3, 0]\T$
\item $i_k = 1$, $j_k = 4$
\item $\eta = 0.1$
\end{itemize}

\begin{align*}
\bx_k &= [1, 0, 0, -1, 0]\T\\
\bx_k\T \btheta &= 0.5 - 0.3 = 0.2\\
\PR{y_k = 1| \btheta} &= \sigma(0.2 + 0.1) \approx 57.4\%
\end{align*}



% \cred{
% So, for given initial condition $\btheta_0$ and an appropriate choice of $\beta$, the estimate of the skills $\btheta_k$ [obtained from the Elo algorithm \eqref{eq:rating-sgd2}] will ``converge" to $\hat\btheta$ as $k$ increases.
% One of its properties is that the sum of the skills remains constant \cite[Ch.~5]{Langeville12_book}, \ie
% \begin{align}
% \label{Sum.skills.const.}
%     \sum_{m=1}^M\theta_{k,m} = c
% \end{align}
% and while any initialization can be used, it is convenient to use the all-zero one, $\btheta_0=\bzero$, which together with \eqref{Sum.skills.const.} yields
% \begin{align}
% \label{Sum.skills.zero}
%     \bone\T\btheta_k=\sum_{m=1}^M\theta_{k,m} =0.
% \end{align}
% }

%************************************************************************************


==> old/_unused.tex <==
\newpage
\section*{Checking out $z_k$}

\begin{align}
z_{k+1} &= \bx_{k+1}\T \tilde\btheta_{k+1}\\
&= \bx_{k+1}\T (\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \bx_{k+1}\T \bx_k\\
&\neq \bx_k\T (\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \bx_k\T \bx_k\\
&= \bx_k\T \tilde\btheta_k - \beta h_k \bx_k\T \bx_k\bx_k\T \tilde\btheta_k + \beta g_k \bx_k\T \bx_k\\
&= (1 - 2 \beta h_k) z_k + 2 \beta g_k
\end{align}


This is ``suspicious \gls{sg}'':
\begin{align} \label{eq:suspicious-sgd}
z_{k+1} &\approx z_k - \beta \nabla_{z_k} \tilde\ell(z_k)\\
&= (1 - \beta h_k) z_k + \beta g_k
\end{align}

if \eqref{eq:suspicious-sgd} holds\footnote{It does not, but maybe approximately it does.}, then
\begin{align}
\Ex[z_{k+1}] &= (1 - \beta \ov{h}) \Ex[z_k]
\end{align}

This is true:
\begin{align}
E[\tilde\ell_k(\btheta_k)] &= E[\tilde\ell_k(\btheta^*)] + \frac{1}{2} E[h_k z_k^2]\\
&= E[\tilde\ell_k(\btheta^*)] + \frac{1}{2} \ov{h} E[z_k^2]\\
&= \tilde\ell_{\rm min} + \tilde\ell_{{\rm ex},k}
\end{align}

This depends on \eqref{eq:suspicious-sgd}
\begin{align}
\Ex[z_{k+1}^2] &= (1 + \beta^2 \Ex[h_k^2] + 2 \beta \Ex[h_k]) \Ex[z_k^2] + \beta^2 \Ex[g_k^2] + 2 \beta \Ex[(1 - \beta h_k) z_k g_k]\\
&= [1 - \beta (2 \ov{h} - \beta \ov{h^2})] \Ex[z_k^2] + \beta^2 \ov{h}
\end{align}

This result is the same we got on the ``single player problem'', where the factor of 2 appeared only on $\ov{h}$:
\begin{align}
\Ex[z_{k+1}^2] &= [1 - \beta (2 \ov{h} - \beta \ov{h^2})] \Ex[z_k^2] + \beta^2 \ov{h}
\end{align}

Then:
\begin{align}
\Ex[z_{\infty}^2] &= \frac{\beta \ov{h}}{2 \ov{h} - \beta \ov{h^2}}\\
\Ex[z_0^2] &= \Ex[(\theta^*_m - \theta^*_n)^2] = 2v\\
\ov{\ell}_{\infty} &= \frac{\beta \ov{h}^2}{4 \ov{h} - 2 \beta \ov{h^2}}\\
\ov{\ell}_0 &= v \ov{h}\\
\alpha &= [1 - \beta (2 \ov{h} - \beta \ov{h^2})]^k\\
% \ov{\ell}_k &= [1 - \beta (2 \ov{h} - \beta \ov{h^2})]^k (\ov{\ell}_0 - \ov{\ell}_{\infty}) + \ov{\ell}_{\infty}
\end{align}

\section*{Checking out $z_k$ (with size $(M - 1)$)}

\begin{align}
\matA = [\bone | -\matI_{M-1}] =
\begin{bmatrix}
1 & -1 & 0 & \hdots & 0 & 0\\
1 & 0 & -1 & \hdots & 0 & 0\\
\vdots & \vdots & \vdots & \ddots & \vdots & \vdots\\
1 & 0 & 0 & \hdots & -1 & 0\\
1 & 0 & 0 & \hdots & 0 & -1\\
% \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots\\
\end{bmatrix}
\end{align}

\begin{align}
\bz_{k+1} &= \matA \tilde\btheta_{k+1}\\
&= \matA (\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \matA \bx_k\\
&= \matA\tilde\btheta_k - \beta h_k \matA \bx_k\bx_k\T \tilde\btheta_k + \beta g_k \matA \bx_k
\end{align}



\newpage


The excess loss is calculated as
\begin{align}
\label{eq:L_ex}
\tilde\ell_{{\rm ex},k} 
&= \frac{1}{2} \Tr\{\Ex[\tilde\btheta_k\T \matH     \tilde\btheta_k]\}
= \frac{1}{2} \Ex\{\Tr[\tilde\btheta_k \tilde\btheta_k\T\matH]\}\\
% &= \frac{1}{2} \ov{h}\Tr\{\Ex[\tilde\btheta_k \tilde\btheta_k\T]     \matR\}\\
\label{eq:L_ex2}
% &\approx \frac{1}{2} \ov{h}\Ex\{\Tr[\tilde\btheta_k \tilde\btheta_k\T\matR]\}
&\approx \frac{1}{2} \ov{h}\Ex\{\Tr[\tilde\btheta_k \tilde\btheta_k\T\matR]\}
\end{align}
where the approximation is needed to obtain \eqref{eq:L_ex2} from   \eqref{eq:H_approximation}. Using the approximate \gls{sg} recursion \eqref{eq:param-error}, we can express \eqref{eq:L_ex2} as
\begin{align}
\label{tilde.L.ex.k+1}
    \tilde\ell_{{\rm ex},k+1} 
    &\approx
    \frac{1}{2}\ov{h} \Ex\Big[\Tr[(\tilde\btheta_k - \beta h_k \bx_k \bx_k\T \tilde\btheta_k + \beta g_k \bx_k)(\tilde\btheta_k - \beta h_k \bx_k \bx_k\T \tilde\btheta_k + \beta g_k \bx_k)\T \matR]\Big] \\
\label{tilde.L.ex.k+1.2}
    &=
    \tilde\ell_{{\rm ex},k} - \frac{4\ov{h}\beta}{M - 1}\tilde\ell_{{\rm ex},k} + \beta^2 \frac{1}{2}\ov{h} \Ex\Big[\Tr[h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\Big] + \frac{2\ov{h}^2 \beta^2}{M - 1}\\
\label{tilde.L.ex.k+1.3}
    &=
    \left[ 1 - \frac{4}{M - 1}\beta(\ov{h} - \beta\ov{h^2}) \right] \tilde\ell_{{\rm ex},k} + \frac{2\ov{h}^2 \beta^2}{M - 1},
\end{align}
where, to pass from \eqref{tilde.L.ex.k+1} to \eqref{tilde.L.ex.k+1.2} and then to \eqref{tilde.L.ex.k+1.3} we use simple algebraic steps detailed in the \ref{Appendix.B} which also shows that
\begin{align}\label{mean-h_k^2}
\ov{h^2} &= \Ex_{\btheta^*;\bx_k}[\mcL^2(\bx_k\T \btheta^*; 0, 1)]\\
% \frac{1}{16} \sqrt{\frac{1}{2v + 1}}.
&\approx \frac{1}{16} \mcN(0;\eta,2v + 1) \sqrt{2\pi}\\
&= \frac{1}{16} \sqrt{\frac{1}{2v + 1}} \exp{\left[\frac{-\eta^2}{2 (2v + 1)}\right]}.
\end{align}

% Determining the outer product $\tilde\btheta_{k+1} \tilde\btheta_{k+1}\T$ from \eqref{eq:param-error}, taking the expected value on both sides of the resulting expression, and considering \eqref{eq:L_ex2}, one has
% \begin{align}\label{eq:correlation-weight1}
% \tilde\ell_{{\rm ex},k+1} 
% \approx&\ \frac{1}{2}\ov{h} \Ex\{\Tr[\tilde\btheta_{k+1} \tilde\btheta_{k+1}\T\matR]\}\\
% =&
% \ \frac{1}{2}\ov{h} \Ex\{\Tr[(\tilde\btheta_k - \beta h_k \bx_k \bx_k\T \tilde\btheta_k + \beta g_k \bx_k)(\tilde\btheta_k - \beta h_k \bx_k \bx_k\T \tilde\btheta_k + \beta g_k \bx_k)\T \matR]\} \\
% =&\ \frac{1}{2}\ov{h} \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \matR]\} \\
% &- \frac{1}{2}\ov{h} \beta \Ex\{\Tr[h_k \tilde\btheta_k\tilde\btheta_k\T \bx_k\bx_k\T \matR]\} - \frac{1}{2}\ov{h} \beta \Ex\{\Tr[h_k \bx_k\bx_k\T \tilde\btheta_k\tilde\btheta_k\T \matR]\} \\
% &+ \frac{1}{2}\ov{h} \beta \Ex\{\Tr[g_k\bx_k \tilde\btheta_k\T (\bI - \beta h_k \bx_k \bx_k\T) \matR]\} \\
% &+ \frac{1}{2}\ov{h} \beta \Ex\{\Tr[g_k (\bI - \beta h_k \bx_k \bx_k\T) \tilde\btheta_k \bx_k\T \matR]\}\\
% &+ \frac{1}{2}\ov{h} \beta^2 \Ex\{\Tr[ h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\} + \frac{1}{2}\ov{h} \beta^2 \Ex\{\Tr[g_k^2 \bx_k\bx_k\T \matR]\}
% \\
% % =&\ \frac{1}{2}\ov{h} \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \matR]\} - \ov{h} \beta \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \ov{h} \matR \matR]\} + \beta^2 \frac{1}{2}\ov{h} \Ex\{\Tr[h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\} + \frac{1}{2}\ov{h} \beta^2 \Ex\{\Tr[\ov{h} \matR \matR]\}\\
% % =&\ \frac{1}{2}\ov{h} \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \matR]\} - \frac{4\ov{h}\beta}{M - 1} \frac{1}{2}\ov{h}  \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \matR]\} + \beta^2 \frac{1}{2}\ov{h} \Ex\{\Tr[h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\} + \frac{2\ov{h}^2 \beta^2}{M - 1}\\
% =&\ \tilde\ell_{{\rm ex},k} - \frac{4\ov{h}\beta}{M - 1}\tilde\ell_{{\rm ex},k} + \beta^2 \frac{1}{2}\ov{h} \Ex\{\Tr[h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\} + \frac{2\ov{h}^2 \beta^2}{M - 1}
% % \\\matG_{k+1} =&\ \matG_k - \beta\ov{h} (\matG_k \matR + \matR \matG_k) + \beta^2 \ov{h^2} \Ex[\bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T] + \beta^2\ov{h} \matR
% \end{align}

% \ls{it looks less messy (I mean with $\tilde\ell_{\tr{ex},k}$). Does it make sense to introduce $\matH_k=\bx_k h_k \bx_k\T$ already in \eqref{eq:cost-taylor}? Just to not trail all the redundant notation $\bx_k h_k \bx_k\T$.}

% where we used the results given in \ref{Appendix.A} to simplify
% \begin{align}
% \Ex\{\Tr[h_k \tilde\btheta_k\tilde\btheta_k\T \bx_k\bx_k\T \matR]\} = \Ex\{\Tr[h_k \bx_k\bx_k\T \tilde\btheta_k\tilde\btheta_k\T \matR]\} = \ov{h} \frac{2}{M - 1} \Ex\{\Tr[\tilde\btheta_k\tilde\btheta_k\T \matR]\}
% \end{align}
% and
% \begin{align}\label{eq:correlation-weight2}
% \Ex[g_k^2 \bx_k\bx_k\T] 
% &= \Ex_{\bx_k;y_k}\{[y_k - \sigma(\bx_k\T \btheta^*+\eta)]^2 \bx_k\bx_k\T\}\\
% &= \Ex_{\bx_k}\{[\Ex_{y_k|\bx_k}[y_k^2] + \sigma^2(\bx_k\T \btheta^*+\eta) - 2 \Ex_{y_k|\bx_k}[y_k] \sigma(\bx_k\T \btheta^*+\eta)] \bx_k\bx_k\T\}\\
% &= \Ex_{\bx_k}\{\mcL(\bx_k\T \btheta^*+\eta) \bx_k\bx_k\T\}\\
% &\approx \ov{h} \matR.
% \end{align}
% and
% \begin{align}\label{eq:h_k^2}
% \ov{h^2} &= \Ex[h_k^2]\\
% &= \Ex_{\btheta^*}[\mathcal{L}^2(\theta^*_m - \theta^*_n; 0, 1)],\quad \forall m \neq n\\
% &\approx \sqrt{2\pi}\mcL^2(0; 0, 1) \mcN(0;0,2v + 1) \\
% &= \frac{1}{16} \sqrt{\frac{1}{2v + 1}}
% \end{align}
% obtained following the methodology discussed in \ref{Appendix.B}. Note in \eqref{eq:correlation-weight1} that $\Ex\{\Tr[h_k^2 \bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T \matR]\}$ does not have a closed-form solution for the general case.

% % \cred{Note in \eqref{eq:correlation-weight1} that $\Ex[\bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T]$ does not have a closed-form solution for the general case.} 


% % To proceed further with the model development, we focus now on the determination of \eqref{eq:L_ex} instead of \eqref{eq:correlation-weight1}. To this end, post-multiplying both sides of \eqref{eq:H_k} by $\matR$ and taking the trace of the resulting expression, we get
% % \begin{equation}\label{eq:TrHR}
% % \begin{aligned}
% % \Tr[\matG_{k+1}\matR]
% % &=
% % \Tr[\matG_k\matR] - \beta\ov{h} \Tr[\matG_k \matR\matR + \matR \matG_k\matR]\\ &+ \beta^2 \ov{h^2} \Tr\{\Ex[\bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T]\matR\} + \beta^2\ov{h} \Tr[\matR\matR].
% % \end{aligned}
% % \end{equation}
% % Then, considering the results given in Appendix A to simplify
% % \begin{equation}
% % 	\Tr[\matR\matR] = \frac{4}{M-1}
% % \end{equation}

% and
% \begin{align}
% \label{final.step.is.here}
% \Tr\{\Ex[\bx_k \bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T]\matR\}
% &= 
% \Ex\{\Tr[\bx_k\T \tilde\btheta_k \tilde\btheta_k\T \bx_k \bx_k\T\matR\bx_k]\}\\
% &\approx\Tr[\matG_k\matR ]\Ex[\bx_k\T\matR\bx_k]\\
% &=\frac{2}{M-1}\Tr[\matG_k\matR ]\Ex\left[\bx_k\T\left(\bI - 		\frac{1}{M}\bone\bone\T\right)\bx_k\right]\\
% &=\frac{2}{M-1}\Tr[\matG_k\matR ]\Ex[\bx_k\T\bx_k]\\
% &=\frac{4}{M-1}\Tr[\matG_k\matR ]
% \end{align}

The initial excess loss, $\tilde\ell_{\tr{ex},0}$ is obtained knowing that the skills are initialized with $\btheta_0 = \bzero$,
\begin{align}
\tilde\ell_{{\rm ex},0} 
&= \frac{1}{2}\ov{h} \Ex\Big[\Tr[\tilde\btheta_0 \tilde\btheta_0\T\matR]\Big] =
\frac{1}{2}\ov{h}\Tr[\btheta^*  \matR(\btheta^*)\T]\\
%&= \frac{1}{2}\ov{h}\Tr[(\btheta^*)\T\btheta^* \matR]\\
%&= \frac{1}{2}\ov{h} \frac{2}{M-1} \left[ \Tr[(\btheta^*)\T\btheta^*] - \frac{1}{M}(\btheta^*\bone)^2 \right]\\
%&= \frac{1}{2}\ov{h} \frac{2}{M-1} \left[ \|\btheta^*\|^2 - \frac{1}{M}(\btheta^*\bone)^2 \right]\\
&= \frac{\ov{h}}{M-1} \|\btheta^*\|^2\\
%&= \frac{\ov{h}}{2}\frac{\|\btheta^*\|^2}{M - 1}\\
&\approx v\ov{h}.
\end{align}

We can now rewrite \eqref{tilde.L.ex.k+1.3} to make clear distinction between  the transient and steady-state phases in the convergence
\begin{align}\label{eq:TrHR_alpha}
\tilde\ell_{{\rm ex},k} = \alpha^k(\tilde\ell_{{\rm ex},0} - \tilde\ell_{{\rm ex},\infty}) + \tilde\ell_{{\rm ex},\infty}
% \Tr[\matG_k\matR] = \alpha^k\{\Tr[\matG_0\matR] - \Tr[\matG_{\infty}\matR]\} + \Tr[\matG_{\infty}\matR]
\end{align}
where
\begin{align}
\alpha &= 1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2}),\\
%\tilde\ell_{{\rm ex},0} 
%&= \frac{1}{2}\ov{h} \Ex\{\Tr[\tilde\btheta_0 \tilde\btheta_0\T\matR]\} = \ov{h} v,\\
\tilde\ell_{{\rm ex},\infty} &= \frac{(\ov{h})^2 \beta}{2(\ov{h} - \beta \ov{h^2})}
\end{align}




%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence conditions}
\ls{The derivations from this subsection should go to \secref{Sec:Discussion}}

Note\footnote{Is this paragraph useful?} that we can characterize the transient behavior of \eqref{eq:TrHR_alpha} by obtaining the time constant from the following equation
\begin{equation}
	\alpha^k = \e^{-\frac{k}{\tau}},
\end{equation}
and the time constant is given by
\begin{equation}
	\tau \approx \frac{M-1}{4 \beta(\ov{h} - \beta \ov{h^2})}
\end{equation}
when $(1 - \alpha) \ll 1$.

% \alpha = 1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})
From \eqref{eq:TrHR_alpha}, the stability condition of the linearized algorithm is guaranteed when $|\alpha| < 1$, thus the learning rate $\beta$ must satisfy the inequality
\begin{align}\label{ineq:convergence_condition1}
0 < \beta &< \frac{\ov{h}}{\ov{h^2}}\\
0 < \beta &< 4 \sqrt{\frac{2v + 1}{v + 1}} \exp\left[\frac{\eta^2}{4(v + 1)(2v + 1)}\right].
\end{align}
% \ov{h} = \frac{1}{4} \sqrt{\frac{1}{v + 1}} \exp\left[\frac{-\eta^2}{4(v + 1)}\right]
% \ov{h^2} = \frac{1}{16} \sqrt{\frac{1}{2v + 1}} \exp\left[\frac{-\eta^2}{2(2v + 1)}\right]

% The stability condition is sufficient for convergence, but it does not guarantee a decrease in steady-state excess loss when compared to the initial loss.
% a reduction of the steady-state excess loss when compared to the initial loss.

% That is, although the ratings converge to a solution, its variance can be larger than the true ratings.

The stability condition is sufficient for convergence, but it does not guarantee a reduction in steady-state excess loss over its initial value. Furthermore, if we restrict $\beta$ by ensuring that
\begin{align}
% \tilde\ell_{{\rm ex},\infty} < \tilde\ell_{{\rm ex},0},
\ov{v}_{\infty} < \ov{v}_0,
\end{align}
we obtain an ``improvement condition''\footnote{Should we name it so it's easier to reference?} for the learning rate, which is given by the inequality
\begin{align}\label{ineq:convergence_condition2}
% \frac{\beta\ov{h}}{\ov{h} - \beta \ov{h^2}} &< 2v\\
\beta &< \frac{2 v \ov{h}}{(1-1/M) \ov{h} + 2 v \ov{h^2}}\\
% \beta &< \frac{2v \ov{h}}{\ov{h} + 2v \ov{h^2}}\\
% &< \frac{2v}{1 + 2v \frac{\ov{h^2}}{\ov{h}}}\\
\frac{1}{\beta} &> \frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}\\
\frac{1}{\beta} &> \dz{ \frac{1}{2v} + \frac{\ov{h^2}}{\ov{h}} }\\
&> \frac{1}{2v} + \frac{1}{4} \sqrt{\frac{v + 1}{2v + 1}} \exp\left[\frac{-\eta^2}{4(2v + 1)(v + 1)}\right]\\
&> \frac{1}{4v} \left\{2 + v \sqrt{\frac{v + 1}{2v + 1}} \exp\left[\frac{-\eta^2}{4(2v + 1)(v + 1)}\right] \right\}\\
\beta &< \frac{4v}{2 + v \sqrt{\frac{v + 1}{2v + 1}} \exp\left[\frac{-\eta^2}{4(2v + 1)(v + 1)}\right]}\\
&< \frac{4v (2v + 1)}{4(2v + 1) + v \sqrt{(v + 1)(2v + 1)} \exp\left[\frac{-\eta^2}{4(2v + 1)(v + 1)}\right]}
% \beta &< 4v \sqrt{\frac{2v + 1}{v^3 + v^2 + 8v + 4}} \text{, \dz{this is for $\eta = 0$}}
\end{align}
% h_1 = \frac{1}{4} \sqrt{\frac{1}{v + 1}}
% h_2 = \frac{1}{16} \sqrt{\frac{1}{2v + 1}}

\dz{We can also interpret this as the harmonic sum of the sample variance (of the skills differences $z_k$) and the stability condition:
\begin{align}
\frac{1}{\beta} &> \frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}\\
&> \frac{1}{(2v)/(1-1/M)} + \frac{1}{\frac{\ov{h}}{\ov{h^2}}}\\
&> \frac{1}{\ov{v}_z} + \frac{1}{\frac{\ov{h}}{\ov{h^2}}}\\
\beta &> \frac{1}{\frac{1}{\ov{v}_z} + \frac{\ov{h^2}}{\ov{h}}}
\end{align}
}

Also note that when $v \to \infty$, this second condition tends to the stability limit
\begin{align}
\lim_{v \to \infty} \frac{2v \ov{h}}{\ov{h} + 2v \ov{h^2}} &= \lim_{v \to \infty} \frac{\ov{h}}{\ov{h^2}} = 4\sqrt{2},
% &= \frac{\ov{h}}{\ov{h^2}}.
\end{align}
% and when $v$ is sufficiently small
and when $2v \ov{h^2} \ll \ov{h}$, \ie for sufficiently small $v$,
\begin{align}
\frac{2v \ov{h}}{\ov{h} + 2v \ov{h^2}} \approx 2v.
\end{align}



% For values of $K > 1$, there are no analytical solutions to the problem.

% We notice\footnote{I think it needs another condition to prove that it's true} that $\beta_{{\rm opt}, K} \leq \beta_{{\rm opt}, K-1}$ since, when the optimal learning rate is used, the excess loss is monotonically decreasing with respect to $K$, that is 
% \begin{equation}
% 	\min_{\beta} \tilde{L}_{{\rm ex}, K} \, \leq \, \min_{\beta} \tilde{L}_{{\rm ex}, K-1}.
% \end{equation}

% $\beta_{{\rm opt}, K} \leq \beta_{{\rm opt}, K-1}$.

% By induction, we can show that $\beta_{{\rm opt}, K} \leq \beta_{{\rm opt}, 1}$ and we stablish a more restrictive limit of the learning rate by solving \eqref{eq:optimization_etaloss} for $K = 1$, given by

% Although it is not possible to analytically express the solution of \eqref{eq:optimization_etaloss} for most $K$,

Alternatively, we can find the optimal learning rate $\beta$ which minimizes the skills variance for a particular number of games $K$. That is, solving the univariate optimization problem
\begin{equation}\label{eq:optimization_etaloss}
\beta_{{\rm opt}, K} = \argmin_{\beta} \ov{v}_K.
\end{equation}

An analytical solution of \eqref{eq:optimization_etaloss} is not easily obtained for a generic $K$, but, as shown in \ref{Appendix.C}, by restricting to $K = 1$ the optimal step is given by
\begin{equation} \label{eq:optimal-beta1}
\beta_{{\rm opt}, 1} = \frac{v \ov{h}}{2v\ov{h^2} + \ov{h}},
\end{equation}
which is a half of the ``improvement condition'' shown in \eqref{ineq:convergence_condition2}.

We notice that, when an optimal learning rate is used, the excess loss is monotonically decreasing with respect to the number of games $K$, that is
\begin{equation}
\min_{\beta} \ov{v}_K \, \leq \, \min_{\beta} \ov{v}_{K-1},
\end{equation}
and it follows that
\begin{equation}
	\beta_{{\rm opt}, K} \, \leq \, \beta_{{\rm opt}, K-1}.
\end{equation}

Finally, we establish $\beta_{{\rm opt}, 1}$ as the most restrictive condition of the learning rate, since
\begin{equation}
	\beta_{{\rm opt}, K} \, \leq \, \beta_{{\rm opt}, 1}, \quad \forall K \in \mathbb{N}^*.
\end{equation}

% more restrictive condition of the learning rate

% Finally, we can use $\beta_{{\rm opt}, 1}$ as a learning rate value suggestion 

% \begin{equation}
% \begin{aligned}
% 	\Tr[\bH_{K}\matR] &< \Tr[\bH_0\matR]\\
% 	\alpha^K\{\Tr[\bH_0\matR] - \Tr[\bH_{\infty}\matR]\} + \Tr[\bH_{\infty}\matR] &< \Tr[\bH_0\matR]\\
% 	\alpha^K\{\Tr[\bH_0\matR] - \Tr[\bH_{\infty}\matR]\} &< \Tr[\bH_0\matR] - \Tr[\bH_{\infty}\matR]\\
% 	\alpha^K &< 1\\
% 	\alpha &< 1\\
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% 	\Tr[\bH_{K}\matR] &< \Tr[\bH_0\matR]\\
% 	\alpha^K\{\Tr[\bH_0\matR] - \Tr[\bH_{\infty}\matR]\} + \Tr[\bH_{\infty}\matR] &< \Tr[\bH_0\matR]\\
% 	\Tr[\bH_{\infty}\matR] - \alpha^K \Tr[\bH_{\infty}\matR]&< \Tr[\bH_0\matR] - \alpha^K \Tr[\bH_0\matR]\\
% 	(1 - \alpha^K) \Tr[\bH_{\infty}\matR]&< (1 - \alpha^K) \Tr[\bH_0\matR]\\
% 	\Tr[\bH_{\infty}\matR]&< \Tr[\bH_0\matR]\\
% \end{aligned}
% \end{equation}


% \begin{equation}
% \begin{aligned}
% 	\frac{\dd \tilde{L}_{{\rm ex}, 1}}{\dd \beta} &= 0\\
% 	\frac{\dd}{\dd \beta} \Tr[\bH_{1}\matR] &= 0\\
% 	\frac{\dd}{\dd \beta} \left[2v \alpha + (1 - \alpha) \frac{\beta\ov{h}}{\ov{h} - \beta \ov{h^2}}\right] &= 0\\
% 	\frac{\dd}{\dd \beta} \left[2v - 2v \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2}) + \frac{4}{M-1} \beta^2 \ov{h} \right] &= 0\\
% 	\frac{\dd}{\dd \beta} \left[- 2v\ov{h} \beta + (2v\ov{h^2} + \ov{h})\beta^2 \right] &= 0\\
% 	- v\ov{h} + (2v\ov{h^2} + \ov{h})\beta &= 0\\
% 	\beta &= \frac{v \ov{h}}{2v\ov{h^2} + \ov{h}}
% \end{aligned}
% \end{equation}


% \begin{equation}
% \begin{aligned}
% 	% \beta &= \frac{v \ov{h}}{2v\ov{h^2} + \ov{h}}\\
% 	% \ov{h} &= \frac{1}{4} \sqrt{\frac{1}{v + 1}}\\
% 	% \ov{h^2} &= \frac{1}{16} \sqrt{\frac{1}{2v + 1}}\\
% 	% \alpha &= 1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})\\
% 	\frac{\dd \tau}{\dd \beta} &= 0\\
% 	\frac{\dd }{\dd \beta} \left(-\frac{1}{\ln(\alpha)}\right) &= 0\\
% 	-\frac{1}{\alpha \ln^2(\alpha)} \frac{\dd \alpha}{\dd \beta} &= 0\\
% 	\frac{\dd \alpha}{\dd \beta} &= 0\\
% 	\frac{\dd}{\dd \beta} [1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})] &= 0\\
% 	\frac{\dd}{\dd \beta} [\beta\ov{h} - \beta^2 \ov{h^2}] &= 0\\
% 	\ov{h} - 2\beta \ov{h^2} &= 0\\
% 	\beta &= \frac{\ov{h}}{2\ov{h^2}}\\
% \end{aligned}
% \end{equation}


% \begin{equation}
% \begin{aligned}
% \beta_{\rm opt} &= \argmin_{\beta} \tilde{L}_{{\rm ex}, K} \\
% % &= \argmin_{\beta} \alpha^K\{\Tr[\bH_0\matR] - \Tr[\bH_{\infty}\matR]\}\\
% % &= \argmin_{\beta} \left[1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})\right]^K \frac{2v\ov{h} - \beta (2v \ov{h^2} + \ov{h})}{\ov{h} - \beta \ov{h^2}}\\
% \end{aligned}
% \end{equation}


% v * c_1 * (M - 1) / (4*v * c_1**2 *(K-1) + (M - 1) * (c_1 + 2*v * c_2))

% \begin{equation}
% \begin{aligned}
% \beta_{\rm opt} &\approx \frac{v \ov{h}}{4v\ov{h}^2(K-1)/(M - 1) + \ov{h} + 2v \ov{h^2}} \\
% \end{aligned}
% \end{equation}



% When do we have an optimal convergence time and a steady state loss smaller than the initial loss?
% \begin{equation}
% \begin{aligned}
% 	% \beta &= \frac{v \ov{h}}{2v\ov{h^2} + \ov{h}}\\
% 	% \ov{h} &= \frac{1}{4} \sqrt{\frac{1}{v + 1}}\\
% 	% \ov{h^2} &= \frac{1}{16} \sqrt{\frac{1}{2v + 1}}\\
% 	% \alpha &= 1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})\\
% 	\frac{\ov{h}}{2\ov{h^2}} &< \frac{2v \ov{h}}{2v\ov{h^2} + \ov{h}}\\
% 	2v\ov{h^2} + \ov{h} &< 4v \ov{h^2}\\
% 	\ov{h} &< 2v \ov{h^2}\\
% 	\frac{\ov{h}}{\ov{h^2}} &< v\\
% 	4 \sqrt{\frac{2v + 1}{v + 1}} &< v\\
% 	16 (2v + 1) &< v^2(v+1)\\
% 	0 &< v^3 + v^2 - 32v - 16\\
% 	v &> 5.43255
% \end{aligned}
% \end{equation}


% \begin{equation}
% 	\Tr[\bH_K\matR] = 2v\left[1-\frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})\right]^K + \left\{1 - \left[1-\frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2})\right]^K\right\} \frac{\beta\ov{h}}{\ov{h} - \beta \ov{h^2}}
% \end{equation}

% \begin{equation}
% 	\frac{d \Tr[\bH_K\matR]}{d \beta} = 0
% \end{equation}

% Finally,




\ls{DANIEL: is this the same one we already evoked after \eqref{eq:g_kx_k}?}
\dz{yes, if $A$ is a random variable, independent of $y_k$, then:
\begin{align}
\Ex[g_k A] = \Ex[g_k] \Ex[A] = 0 \Ex[A] = 0
\end{align}
}
\ls{Yes, but this comes from the independence principle... If I recall correctly, the orthogonality principles is related to the optimization of the mean squared error.}
\dz{Let me see, paraphrasing \cite[Sec.~3.3]{book:Boroujeny}:
Primary result: the \textit{optimal prediction error} ($g_k$) is uncorrelated with the \textit{input samples} ($\bx_k$). Secondary result: The \textit{optimal prediction} ($\sigma(\bx_k\T \btheta^*)$) and the \textit{optimal prediction error} ($g_k$) are orthogonal.
\begin{align*}
g_k = \sigma(\bx_k\T \btheta^*) - y_k
\end{align*}
}


\dz{Should we define a new matrix for the 2nd order approximation on \eqref{eq:skills.variance2}? I don't think it helps much, but it's consistent with the derivation of the mean behavior.
\begin{align}
\Ex\Big[ h_k^2 \tilde\btheta_k\T \bx_k \bx_k\T \tilde\btheta_k \Big] &= \Ex\Big[ \tilde\btheta_k\T \matH_2 \tilde\btheta_k \Big]\\
\matH_2 &= \Ex[h_k^2 \bx_k \bx_k\T]\\
&\approx \Ex[h_k^2] \matR = \ov{h^2} \matR
\end{align}
}


\newpage
\section{\normalfont\it Determination of \eqref{eq:optimal-beta1}}\label{Appendix.C}



We want to determine the adaptation step $\beta$ which minimizes the total variance of skills $\ov{v}_K$ for $K = 1$ game.
\begin{equation}
\begin{aligned}
\frac{\dd \ov{v}_1}{\dd \beta} &= 0\\
\frac{\dd}{\dd \beta} \left[ \alpha_2 (\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty \right] &= 0\\
\frac{\dd}{\dd \beta} \left[ \alpha_2 (\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty - v_0 \right] &= 0\\
\frac{\dd}{\dd \beta} \left[ (1 - \alpha_2) (\ov{v}_\infty - \ov{v}_0) \right] &= 0\\
\frac{\dd}{\dd \beta} \left[ \ov{h} (M-1) \beta^2 - 2 Mv\ov{h} \beta + 2 Mv \ov{h^2} \beta^2 \right] &= 0\\
\ov{h} (M-1) \beta - Mv\ov{h} + 2 Mv \ov{h^2} \beta  &= 0\\
\beta_{\rm opt, 1} &= \frac{v \ov{h}}{\ov{h} (1-1/M) + 2 v \ov{h^2}}
\end{aligned}
\end{equation}
which is a half of the ``improvement condition'' shown in \eqref{ineq:convergence_condition2}.

% Cheatsheet:
% \begin{align}
% \alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% \ov{v}_0 &= M v\\
% \ov{v}_{\infty} &= \frac{\beta \ov{h} (M-1)}{2(\ov{h} - \beta \ov{h^2})}\\
% (1 - \alpha_2)\ov{v}_{\infty} &= 2 \beta^2 \ov{h}\\
% (1 - \alpha_2)\ov{v}_0 &= \frac{4 Mv}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% (1 - \alpha_2)\ov{v}_{\infty} - (1 - \alpha_2)\ov{v}_{0} &= 2 \beta^2 \ov{h} - \frac{4 Mv}{M-1} (\ov{h} \beta - \ov{h^2} \beta^2)
% \end{align}

% An analytical solution of \eqref{eq:optimization_etaloss} is not easily obtained for a generic $K$, but by restricting to $K = 1$ the optimal step is given by
% \begin{equation}
% \begin{aligned}
% \frac{\dd \tilde{L}_{{\rm ex}, 1}}{\dd \beta} &= 0\\
% % \frac{\dd}{\dd \beta} \Tr[\bH_{1}\bR] &= 0\\
% \frac{\dd}{\dd \beta} \left[\alpha \left(2v - \frac{\beta\ov{h}_1}{\ov{h}_1 - \beta \ov{h}_2}\right) + \frac{\beta\ov{h}_1}{\ov{h}_1 - \beta \ov{h}_2}\right] &= 0\\
% \frac{\dd}{\dd \beta} \left[2v \alpha + (1 - \alpha) \frac{\beta\ov{h}_1}{\ov{h}_1 - \beta \ov{h}_2}\right] &= 0\\
% \frac{\dd}{\dd \beta} \left[2v - 2v \frac{4}{M-1} \beta(\ov{h}_1 - \beta \ov{h}_2) + \frac{4}{M-1} \beta^2 \ov{h}_1 \right] &= 0\\
% \frac{\dd}{\dd \beta} \left[- 2v\ov{h}_1 \beta + (2v\ov{h}_2 + \ov{h}_1)\beta^2 \right] &= 0\\
% - v\ov{h}_1 + (2v\ov{h}_2 + \ov{h}_1)\beta &= 0\\
% \beta_{{\rm opt}, 1} &= \frac{v \ov{h}_1}{2v\ov{h}_2 + \ov{h}_1},
% \end{aligned}
% \end{equation}



% \begin{equation}
% \begin{aligned}
% \frac{\dd \ov{v}_1}{\dd \beta} &= 0\\
% \frac{\dd}{\dd \beta} \left[ \alpha (\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ \ov{v}_0 + \ov{v}_\infty - \alpha \ov{v}_\infty \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ \alpha \ov{v}_0 + (1 - \alpha) \ov{v}_\infty \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ -(1 - \alpha) \ov{v}_0 + (1 - \alpha) \ov{v}_\infty \right] &= 0\\
% \frac{\dd}{\dd \beta} \left[ \alpha (\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty - v_0 \right] &= 0\\
% \frac{\dd}{\dd \beta} \left[ (1 - \alpha) (\ov{v}_\infty - \ov{v}_0) \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ \beta^2 \ov{h} (M-1)/2 - \beta (\ov{h} - \beta \ov{h^2}) M v \right] &= 0\\
% \frac{\dd}{\dd \beta} \left[ \beta^2 \ov{h} (M-1) - 2M v \beta \ov{h} + 2M v\beta^2 \ov{h^2}  \right] &= 0\\
% \beta \ov{h} (M-1) - M v \ov{h} + 2M v\beta \ov{h^2} &= 0\\
% % \beta &= \frac{M v \ov{h}}{\ov{h} (M-1) + 2M v \ov{h^2}}\\
% \beta_{\rm opt, 1} &= \frac{v \ov{h}}{\ov{h} (1-1/M) + 2 v \ov{h^2}}
% \end{aligned}
% \end{equation}

% \begin{align}
%     \ov{v}_{k+1}
%     &=\alpha\alpha^{k}(\ov{v}_0-\ov{v}_{\infty}) +\ov{v}_{\infty}\\
%     &=\alpha(\ov{v}_k-v_{\infty}) +\ov{v}_{\infty}\\
% \end{align}

% and
% \begin{align}
%     \ov{v}_{k+1} &< \ov{v}_k\\
%     \alpha(\ov{v}_k-v_{\infty}) +\ov{v}_{\infty} &< \ov{v}_k\\
%     v_{\infty} &< \ov{v}_k\\
%     (\alpha-1)(\ov{v}_k-v_{\infty})&<0
% \end{align}


% \begin{align}
% % \ov{v}_{k+1} &= \min_{\beta_k} \alpha(\ov{v}_k-v_{\infty}) +\ov{v}_{\infty}\\
% \frac{\dd}{\dd \beta} \ov{v}_{k+1} &= \frac{\dd}{\dd \beta} [\alpha \ov{v}_k + v_{\infty} - v_{\infty} \alpha]\\
% &= \alpha \frac{\dd}{\dd \beta} \ov{v}_k + \ov{v}_k \frac{\dd}{\dd \beta}\alpha + \frac{\dd}{\dd \beta}[v_{\infty} (1-\alpha)]\\
% &= \alpha \frac{\dd}{\dd \beta} \ov{v}_k - \ov{v}_k \frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2}) + 4 \beta \ov{h}\\
% &= -\ov{v}_k \frac{4}{M-1} (\ov{h} - 2 \beta_{\tr{opt},k} \ov{h^2}) + 4 \beta_{\tr{opt},k} \ov{h}
% \end{align}

% \begin{align}
% \beta_{\tr{opt},k} &> [\alpha^k (\ov{v}_0-\ov{v}_{\infty}) +\ov{v}_{\infty}] \frac{1}{M-1} \left( 1 - 2 \beta_{\tr{opt},k} \frac{\ov{h^2}}{\ov{h}} \right)\\
% \ov{v}_k &< \frac{(M-1)\beta_{\tr{opt},k}\ov{h}}{\ov{h} - 2 \beta_{\tr{opt},k} \ov{h^2}}
% \end{align}


% \begin{align}
% \ov{v}_k &< (M-1)\beta_{\tr{opt},k}\\
% \beta_{\tr{opt},k} &> [\alpha^k (\ov{v}_0-\ov{v}_{\infty}) +\ov{v}_{\infty}] \frac{1}{M-1}\\
% \beta_{\tr{opt},k} &> [\left(1 - \frac{4}{M-1} \right)^k (\ov{v}_0-\ov{v}_{\infty}) +\ov{v}_{\infty}] \frac{1}{M-1}\\
% \end{align}

% \begin{align}
% \ov{v}_k &= \alpha_2^k (\ov{v}_0 - \ov{v}_{\infty}) + \ov{v}_{\infty}
% \end{align}
% where



% \begin{align}
% \frac{\dd \ov{v}_\infty}{\dd \beta} &= (M - 1) \frac{\dd}{\dd \beta} \frac{\beta \ov{h}}{2(\ov{h} - \beta \ov{h^2})}\\
% &= (M - 1) \frac{\ov{h}^2}{2(\ov{h} - \beta \ov{h^2})^2}\\
% \frac{\dd \alpha}{\dd \beta} &= -\frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2})
% \end{align}


\dz{This is why we don't solve the quadratic equation, it gives 2 results of negative $\beta$:
\begin{align*}
|\alpha_2| &< 1\\
-1 < 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2}) &< 1\\
2 > \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2}) &> 0\\
\beta^2 - \beta \frac{\ov{h}}{\ov{h^2}} + \frac{1}{2(M-1)\ov{h^2}} &> 0\\
% \beta &= \frac{-b \pm \sqrt{b^2 - 4ac}}{2a} \\
\beta &= -\frac{\ov{h}}{2\ov{h^2}} \pm \frac{1}{2} \sqrt{\frac{\ov{h}^2}{\ov{h^2}^2} - \frac{2}{(M-1)\ov{h^2}}} \\
\beta &= \frac{1}{2\ov{h^2}} \left[ -\ov{h} + \sqrt{\ov{h}^2 - \frac{2\ov{h^2}}{M-1}} \right] < \frac{1}{2\ov{h^2}} \left[ -\ov{h} + \sqrt{\ov{h}^2} \right] = 0
\end{align*}
}


Simplify:

Furthermore, we assume that $\btheta^*$ is obtained from a Gaussian distribution with zero-mean and a variance $v$. Again, this assumption is well rooted in observations already made in the literature: there are many average teams (with skills $\theta^*_m$ close to zero), and a small number of teams with very high skills, as well as a small number of poorly performing teams. In fact, the Gaussian prior on the teams' skills is often used when solving the regularized rating problems, \eg \cite{Gramacy13}. This is just a convenient assumption which allows us to simplify the development and the interpretation of the results.

\cred{I did not understand the connection between the information given in the previous paragraphs with the discussion presented below this point...}

First of all, we will be able to use the ergodicity argument and approximate the sample statistics with the average, \ie
\begin{align}
\label{ergodicity.argument}
    \frac{1}{M}\sum_{m=1}^M f(\theta^*_m) = \Ex_{\theta^*}[f(\theta^*)].
\end{align}
which should hold very well for sufficiently large $M$. In particular, we may then assume that
\begin{align}\label{ergodicity.variance}
    \frac{1}{M}\sum_{m=1}^M (\theta^*_m)^2 & \approx v.
\end{align}


Second, using the Gaussian model of $\btheta^*$ allows us to treat $v$ as a sole parameter which summarizes all the effects due to particular form of $\btheta^*$. 

In particular, large $v$ means that the difference $z_k=\theta^*_{i_k}-\theta^*_{j_k}$ is likely to be large, and then the game result $y_k$ (generated randomly per \eqref{Pr.y.1}) will be quasi-deterministic, \ie $\PR{y_k=1|z_k}\approx 1$ or $\PR{y_k=1|z_k}\approx 0$. On the other hand, for small $v$, we are likely to encounter small $z_k\approx 0$ which means that $\PR{y_k=1|z_k}\approx\frac{1}{2}$, \ie the uncertainty of the results conditioned on the skills is high. In other words, $v$ controls the uncertainty of the outcomes $y_k$. 

Consider, for example the same professional league, where the teams are expected to perform similarly. A significant uncertainty in the game results, is then modeled by small $v$. On the other hand, the international teams have large disparities in the quality of the players so the games between the strongest and the weakest teams are usually quite easy to predict and we would use a large variance $v$ to model this effect. 

Thus, by changing $v$ we refer to different contexts in which the rating algorithm may be used.

\cred{O.K. The discussion seems interesting; however, I think it is important to create a connection between the ideas within this section.}



\dz{We can also interpret this as the harmonic sum of the sample variance (of the skills differences $z_k$) and the stability condition:
\begin{align}
\frac{1}{\beta} &> \frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}\\
&> \frac{1}{(2v)/(1-1/M)} + \frac{1}{\frac{\ov{h}}{\ov{h^2}}}\\
&> \frac{1}{\ov{v}_z} + \frac{1}{\frac{\ov{h}}{\ov{h^2}}}\\
\beta &< \frac{1}{\frac{1}{\ov{v}_z} + \frac{\ov{h^2}}{\ov{h}}}
\end{align}
}


which may be shown as follows:
\begin{align}
|\alpha_1| < 1 &\implies \beta < \frac{M-1}{\ov{h}}\\
|\alpha_2| < 1 &\implies \beta < \frac{\ov{h}}{\ov{h^2}}\\
\frac{\ov{h}}{\ov{h^2}} &\leq \frac{M-1}{\ov{h}}\\
4 \sqrt{\frac{2v + 1}{v + 1}} \exp\left[\frac{\eta^2}{4(v + 1)(2v + 1)}\right] &\leq 4(M - 1) \sqrt{v + 1} \exp\left[\frac{\eta^2}{4(v + 1)}\right]\\
\frac{\sqrt{2v + 1}}{v+1} \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] &\leq M - 1\\
\frac{\sqrt{2v + 1}}{v+1} \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] &\leq \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] \leq 1 \leq M - 1
\end{align}
which is true because $v$ is positive and $M \geq 2$.



\begin{align}
% \ov{v}_{\infty} &< \ov{v}_0,
% \ov{v}_{k} &< \ov{v}_{k-1}\\
% \alpha_2^k(\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty &< \alpha_2^{k-1}(\ov{v}_0 - \ov{v}_\infty) + \ov{v}_\infty\\
% \alpha_2(\ov{v}_0 - \ov{v}_\infty) &< (\ov{v}_0 - \ov{v}_\infty)\\
% (1 - \alpha_2)(\ov{v}_0 - \ov{v}_\infty) &> 0\\
\ov{v}_{\infty} &< \ov{v}_0,
\end{align}
which is satisfied if 
\begin{align}\label{ineq:convergence_condition2}
% \beta &< \frac{2 v \ov{h}}{(1-1/M) \ov{h} + 2 v \ov{h^2}}\\
% \frac{1}{\beta} &> \frac{M-1}{2v M} + \frac{\ov{h^2}}{\ov{h}}\\
% \frac{1}{\beta} &> \frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}\\
% \frac{1}{\beta} &> \frac{M-1}{2\ov{v}_0} + \frac{\ov{h^2}}{\ov{h}}\\
% \frac{1}{\beta} &> \dz{ \frac{1}{2v} + \frac{\ov{h^2}}{\ov{h}} }\\
% \beta &< \frac{4v}{2 + v \sqrt{\frac{v + 1}{2v + 1}} \exp\left[\frac{-\eta^2}{4(2v + 1)(v + 1)}\right]}\\
% \beta &< 4v \sqrt{\frac{2v + 1}{v^3 + v^2 + 8v + 4}} \text{, \dz{this is for $\eta = 0$}}
\beta &< \frac{2 v \ov{h}}{(1-1/M) \ov{h} + 2 v \ov{h^2}}
\end{align}


\begin{align}
\Ex[\tilde\btheta_{k+1}] &= \Ex[\tilde\btheta_{k}] + \beta \Ex\{ [y_k - \sigma(\bx_k\T \btheta_k+\eta)] \bx_k \}\\
&= \Ex[\tilde\btheta_{k}] + \beta \Ex\{ [\sigma(\bx_k\T \btheta^*+\eta) - \sigma(\bx_k\T \btheta_k+\eta)] \bx_k \}\\
&= \Ex[\tilde\btheta_{k}] - \beta \Ex\{ [\sigma(\tilde{z}_k + z_k^* + \eta) - \sigma(z_k^* + \eta)] \bx_k \}\\
&\approx \Ex[\tilde\btheta_{k}] - \beta \Ex[\mcL(z_k^* + \eta) \tilde{z}_k \bx_k]\\
&= \Ex[\tilde\btheta_{k}] - 2\beta \Ex[\mcL(\bx_k\T \btheta^* + \eta) \tilde\btheta_k]\\
&= \Ex[\tilde\btheta_{k}] - 2\beta \ov{h} \Ex[\tilde\btheta_k]
\end{align}



%\dz{Very similar to our derivation, but they use the inverse of the Fisher matrix (not possible, since it's singular in our case): \url{https://en.wikipedia.org/wiki/Scoring_algorithm}}
% where
% \begin{align}
% \label{eq:optimal-error}
% 	g_k = y_k - \sigma(\bx_k\T \btheta^*+\eta)
% \end{align}
% is the prediction error for the optimal skills.
%Finally, subtracting $\btheta^*$ from both sides of \eqref{eq:sgd-taylor.2},  we obtain
%\begin{align}\label{eq:param-error}
%\tilde\btheta_{k+1} &= 
%(\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \bx_k 
%\end{align}
%which also satisfies the constant-sum condition \eqref{constant.sum}, \ie 
%\begin{align}
%\label{constant.sum.tilde}
%\bone\T\tilde\btheta_k &=\bone\T\tilde\btheta_0\\
%&=0.
%\end{align}


\dz{Alternative definition:
\begin{align}
[\matH]_{m,n} & = 
% \Ex_{\bx_k}[\mcL(\bx_k\T\btheta^*+\eta)x_{k,m} x_{k,n}]\\
% &=
\frac{1}{M(M-1)} 
\begin{cases}
-2\mcL(\eta) + \displaystyle\sum_{l=1}^M \mcL(\theta^*_{m}-\theta^*_{l}+\eta)+\mcL(\theta^*_{l}-\theta^*_{m}+\eta), & m = n \\
\displaystyle -\mcL(\theta^*_{m}-\theta^*_{n}+\eta) -\mcL(\theta^*_{n}-\theta^*_{m}+\eta),\quad  &\text{otherwise}.
\end{cases}
\end{align}
}




%We also observe that for $-1 < \alpha_1 <0$, the mean converges to the optimal solution $\btheta^*$ in an oscillatory fashion, while for $0< \alpha_1 <1$, the mean converges smoothly (without oscillations). The fastest convergence (in one step) is ensured when $\alpha_1\approx 0$, \ie $\ov{h}\beta\approx (M-1)/2$. While we may accelerate the convergence with appropriately chosen $\beta$, the ``one-step convergence'' is a result of the analytical approximations and is unlikely to be practical.


%\dz{It doesn't oscillate in practice (see \url{https://i.imgur.com/p8HsiEX.png}, $v=5$, $\beta=0.6 (M - 1) / \ov{h} \approx 80$, $\alpha_1 \approx -0.8$). This is an artifact of using the Taylor series approximation to linearize the skill-update equation. The approximation \gls{sg} actually does oscillate, but we are not talking about it. Oh! Another thing, this ``first order'' condition is less restrictive than the one we obtain from the variance/loss:
%\begin{align}
%\beta_{\rm max} &\geq \frac{\ov{h}}{\ov{h^2}}\\
%\lim_{v\to\infty} \frac{M-1}{\ov{h}} = \infty &> 4\sqrt{2} = %\lim_{v\to\infty} \frac{\ov{h}}{\ov{h^2}}\\
%\lim_{v \to 0} \frac{M-1}{\ov{h}} = 4(M-1) &\geq 4 = \lim_{v \to 0} \frac{\ov{h}}{\ov{h^2}}
%\end{align}
%}
%\ls{I see the figure on the web. But I'm not sure it is the proof of no-oscillations... :) I suppose this is the average of the true SG. My remark on the oscillations is true for the analytical prediction... so you would say, that the analytical prediction is not good when $\alpha_1<0$?} \dz{Yes, the analytical predictions get worse and worse as $\beta$ increases. They work well for practical values of $\beta$, smaller than 4, for example. Say $\alpha_1 < 0$, then $\beta > (M-1)/(2\ov{h}) \geq \ov{h}/\ov{h^2}$. $\ov{h} \in [1/4, 0]$, $\ov{h}/\ov{h^2} \in [4, 4\sqrt{2}]$}

%\ls{I see... we do not use in practice $\beta$ as large...}


% To illustrate this point we show in \figref{fig:fisher_matrix_skills} the  expected skills $\Ex[\theta_{k,m}]$ obtained  using a) the simplified formula \eqref{eq:skill-behavior2} (dotted line), b) the approximation \eqref{eq:weight-behavior} (dashed line), and c) the simulations (solid lines), \ie randomly generating $\bx_k$ and $y_k$,  applying the \gls{sg} algorithm \eqref{eq:rating-sgd2}, and averaging the simulation results. We use $\beta=0.1$, $\eta=0.5$, and $\btheta^*=\sqrt{v}\btheta_{\tr{o}}$ with
% \begin{align*}
%     \btheta_\tr{o}=[-1.82, -1.06, -0.84, -0.29,  0.03,  0.06, 0.37, 0.75, 1.16, 1.64]\T,
% \end{align*}
% which satisfies $\bone\T\btheta_{\tr{o}}=0$ and $\frac{1}{M}\|\btheta_{\tr{o}}\|^2=1$. 
% The low-variance case, $v=1$ is shown in \figref{fig:fisher_matrix_skills}a and, the high-variance case, $v=5$ in \figref{fig:fisher_matrix_skills}b.

% % v=1
% % alpha_1: 0.9961924922630578
% % 1 - alpha_1: 0.0038075077369421617

% % v = 5
% % alpha_1: 0.9977554567984103
% % 1 - alpha_1: 0.0022445432015897326

% Since the same adaptation step $\beta$ is used in the examples, the convergence rate, depending on $\beta\ov{h}$ will vary. In fact, for $v=1$ we have $(1-\alpha_1) \approx 3.81 \times 10^{-3}$, while for $v=5$ we calculate $(1-\alpha_1) \approx 2.24 \times 10^{-3}$. This explains why the convergence appears slower in \figref{fig:fisher_matrix_skills}b. More importantly, we see that, despite two-step approximations, \eqref{eq:skill-behavior2} is close to the actual mean and its advantage over \eqref{eq:weight-behavior} is particularly clear for larger $v$.

% We refer to the initial parts of the curves as the \emph{transients} and the last part, as the \emph{steady-state}. Quite obviously, the differences between the approximations appear more clearly in the transient part of the curves.

% \begin{figure}[t!]
% \centering
% \subfloat[]{\includegraphics[scale=1]{figures/fisher_matrix_skills.pdf}}%
% \qquad
% \subfloat[]{\includegraphics[scale=1]{figures/fisher_matrix_skills(high_v).pdf}}%
% \caption{Mean behavior of the skills: obtained by simulations (solid lines), predicted from \eqref{eq:weight-behavior} (dashed lines), and calculated via the approximation \eqref{eq:skill-behavior2} (dotted lines); $M = 10$, $\beta = 0.1$, $\eta = 0.5$, and (a) $v = 1$, (b) $v = 5$}%
% \label{fig:fisher_matrix_skills}%
% \end{figure}


\dz{\begin{align}
\Ex[\matH']_{m,n} &= \frac{2\ov{h}}{M(M-1)}\\
\Ex[\matH'] &= \frac{2\ov{h}}{M(M-1)} \bone\bone\T
\end{align}
\begin{align}
\Ex[\matH] &= \Ex[\tr{diag}(\matH' \bone)] - \Ex[\matH']\\
&= \tr{diag}\{\Ex[\matH'] \bone\} - \Ex[\matH']\\
&= \frac{2\ov{h}}{M(M-1)} \tr{diag}\{\bone\bone\T\bone\} - \frac{2\ov{h}}{M(M-1)} \bone\bone\T\\
&= \frac{2\ov{h}}{M-1} \bI - \frac{2\ov{h}}{M(M-1)} \bone\bone\T\\
&= \frac{2\ov{h}}{M-1} \left(\bI - \frac{1}{M}\bone\bone\T\right)\\
&= \ov{h}\matR
\end{align}}



% \begin{align}
% % \ov{v}_k &= \alpha_2^k (\ov{v}_0 - \ov{v}_{\infty}) + \ov{v}_{\infty}\\
% \ov{v}_{?} &= \ov{v}_{\infty} +  (\ov{v}_0 - \ov{v}_{\infty}) \frac{1}{K-N} \sum_{k=K-N+1}^{K} \alpha_2^k\\
% &= \ov{v}_{\infty} +  (\ov{v}_0 - \ov{v}_{\infty}) \frac{\alpha_2^{K+1}}{K-N} \frac{\alpha_2^{-N} - 1}{1 - \alpha_2} \\
% &= \ov{v}_{\infty} +  (\ov{v}_0 - \ov{v}_{\infty}) \frac{\alpha_2^{K-N+1}}{K-N} \frac{1 - \alpha_2^N}{1-\alpha_2}\\
% \end{align}



% \begin{align}
% \ov{v}_{k+1} &= \alpha_2\ov{v}_k + 2\beta^2 \ov{h}
% \end{align}

% \begin{align}
% \ov{v}_{k+1} - \ov{v}_k &= \alpha_2 (\ov{v}_k - \ov{v}_{k-1})\\
% &= \alpha_2^k (1 - \alpha_2) (\ov{v}_\infty - \ov{v}_0)\\
% % &= (\alpha_2 - 1) \alpha_2^k (\ov{v}_0 - \ov{v}_\infty) + (\alpha_2 - 1) \ov{v}_\infty + 2\beta^2 \ov{h}
% \end{align}

\begin{align}
\Ex[(\bx_k\T \tilde\btheta_k)^2] &= \Ex[\tilde\btheta_k\T \bx_k \bx_k\T \tilde\btheta_k]\\
&= \frac{2}{M-1} \ov{v}_k
\end{align}

\begin{align}
\Ex\{[\nabla\ell(\btheta_k)/\bx_k]^2\} &\approx \Ex\{[\nabla\tilde\ell(\btheta_k)]^2\}\\
% &= \Ex[(h_k \bx_k\bx_k\T \tilde\btheta_k - g_k \bx_k)^2]\\
% &= \frac{2}{M-1} \ov{h^2} \ov{v}_k + 2 \ov{h}
&= \Ex[(h_k \bx_k\T \tilde\btheta_k - g_k)^2]\\
&= \frac{2}{M-1} \ov{h^2} \ov{v}_k + \ov{h}
\end{align}

\begin{align}
\Ex[\bx_k\T \tilde\btheta_k \nabla\ell(\btheta_k)/\bx_k] &= \Ex[\bx_k\T \tilde\btheta_k (h_k \bx_k\T \tilde\btheta_k - g_k)]\\
&= \Ex[h_k (\bx_k\T \tilde\btheta_k)^2 - g_k \bx_k\T \tilde\btheta_k]\\
&= \Ex[h_k (\bx_k\T \tilde\btheta_k)^2]\\
&= \frac{2}{M-1} \ov{h}
\end{align}

\begin{align}
\beta_{o, k} &= \frac{1}{2} \frac{\Ex[\bx_k\T \tilde\btheta_k \nabla\ell(\btheta_k)]}{\Ex\{[\nabla\ell(\btheta_k)]^2\}}\\
&= \frac{\ov{v}_k}{\ov{h}}
\end{align}


\begin{align}
\beta_{o, k} &= \frac{1}{2} \frac{\Ex[(\bx_k\T \tilde\btheta_k)^2]}{\Ex\{[\nabla\ell(\btheta_k)]^2\}}\\
&\approx \frac{\ov{v}_k}{2 \ov{h^2} \ov{v}_k + (M-1) \ov{h}}
\end{align}

\begin{align}
\beta &= \frac{\ov{v}_k}{2 \ov{h^2} \ov{v}_k + (M-1) \ov{h}}\\
\ov{v}_k &= 2\beta \ov{h^2} \ov{v}_k + \beta (M-1) \ov{h}\\
&= \frac{\beta (M-1) \ov{h}}{1 - 2\beta \ov{h^2}}
\end{align}

\begin{align}
\alpha_2^k (\ov{v}_0 - \ov{v}_{\infty}) + \ov{v}_{\infty} &= \frac{2\beta (M-1) \ov{h}}{1 - 2\beta \ov{h^2}}
\end{align}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Checking out the optimum step-size}

% % \ov{v}_{\infty} &= \frac{\beta \ov{h} (M-1)}{2(\ov{h} - \beta \ov{h^2})}\\
% \begin{align}
% \ov{v}_{k+1} &= \alpha_2\ov{v}_k + 2\beta^2 \ov{h}\\
% \ov{v}_k &= \alpha_2^k (\ov{v}_0 - \ov{v}_{\infty}) + \ov{v}_{\infty}\\
% \alpha_2 &= 1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2})\\
% \ov{v}_{\infty} &= \frac{2 \beta^2 \ov{h}}{1 - \alpha_2}\\
% \ov{v}_0 &= M v
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2 &= -\frac{4}{M-1} (\ov{h} - 2 \beta \ov{h^2})\\
% &= - \frac{1 - \alpha_2}{\beta} - \frac{4}{M-1} \beta \ov{h^2}\\
% &= \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)}
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \alpha_2^K &= K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2
% \end{align}

% \begin{align}
% \frac{\dd}{\dd\beta} \ov{v}_{\infty} &= \frac{2 \ov{v}_{\infty}^2}{\beta^2 (M-1)}\\
% &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{v}_{k+1} &= \frac{\dd}{\dd\beta}(\alpha_2 \ov{v}_k) + 4\beta \ov{h}\\
% \frac{\dd}{\dd\beta} \ov{v}_k &= \alpha_2^k (\ov{v}_0 - \ov{v}_{\infty}) + \ov{v}_{\infty}
% \end{align}


% \begin{align}
% \frac{\dd}{\dd\beta} \ov{v}_K &= \frac{\dd}{\dd\beta} [\alpha_2^K (\ov{v}_0 - \ov{v}_{\infty})] + \frac{\dd}{\dd\beta} \ov{v}_{\infty}\\
% &= (\ov{v}_0 - \ov{v}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + \alpha_2^K \frac{\dd}{\dd\beta} (\ov{v}_0 - \ov{v}_{\infty}) + \frac{\dd}{\dd\beta} \ov{v}_{\infty}\\
% &= (\ov{v}_0 - \ov{v}_{\infty}) \frac{\dd}{\dd\beta} \alpha_2^K + (1 - \alpha_2^K)\frac{\dd}{\dd\beta} \ov{v}_{\infty} \\
% &= (\ov{v}_0 - \ov{v}_{\infty}) K \alpha_2^{K-1} \frac{\dd}{\dd\beta} \alpha_2 + (1 - \alpha_2^K)\frac{\dd}{\dd\beta} \ov{v}_{\infty} \\
% &= \frac{\dd}{\dd\beta} \ov{v}_{\infty} + \alpha_2^{K-1} \left[ (\ov{v}_0 - \ov{v}_{\infty}) K \frac{\dd}{\dd\beta} \alpha_2 - \alpha_2 \frac{\dd}{\dd\beta} \ov{v}_{\infty} \right]\\
% % &= \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + \alpha_2^{K-1} \left[ (\ov{v}_0 - \ov{v}_{\infty}) K \frac{4\beta^2 \ov{h^2} - (1 - \alpha_2)(M-1)}{\beta(M-1)} - \alpha_2 \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} \right]\\
% % &= (1-\alpha_2^K) \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + K\alpha_2^{K-1} (\ov{v}_0 - \ov{v}_{\infty}) \left( \frac{4\beta \ov{h^2}}{(M-1)} - \frac{1 - \alpha_2}{\beta} \right)\\
% &= (1-\alpha_2^K) \frac{8 \beta^2 \ov{h}^2}{(M-1)(1 - \alpha_2)^2} + K\alpha_2^{K-1} \left( M v - \frac{2\beta^2\ov{h}}{1 - \alpha_2} \right) \left( \frac{4\beta \ov{h^2}}{(M-1)} - \frac{1 - \alpha_2}{\beta} \right)
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{\cred{Stability conditions} in the mean and mean-square sense}

Based on \eqref{eq:skill-behavior} and \eqref{eq:v_k-final}, \cred{stability conditions} on $\beta$ can be derived to ensure the convergence of the mean of $\btheta_k$ towards $\btheta^*$ as well as the convergence of the MSE of the skills $\ov{v}_k$ to a bounded value. In particular, from \eqref{eq:skill-behavior}, one verifies that the convergence in the mean sense is guaranteed when $|\alpha_1| < 1$. Such a condition is satisfied by choosing $\beta$ within the following range:
\begin{align}
\label{beta.condition.mean}
0 &< \beta < \frac{M - 1}{\ov{h}}
\end{align}
which can also be expressed using \eqref{mean-h_k} as
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{beta.ov.h.condition}
0 &< \beta < 4(M-1)\sqrt{v+1} \exp\left[\frac{\eta^2}{4(v + 1)}\right].
\end{empheq}
In turn, the convergence in the mean-square sense is guaranteed in \eqref{eq:v_k-final} when 
$|\alpha_2| < 1$. This condition leads then to the following inequality on $\beta$:
\begin{align}
0 < \beta &< \frac{\ov{h}}{\ov{h^2}}
\end{align}
which, considering \eqref{mean-h_k} and \eqref{mean-h_k^2}, can alternatively be expressed as
\begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
\label{beta.ov.h.condition2}
0 < \beta &< 4 \sqrt{\frac{2v + 1}{v + 1}} \exp\left[\frac{\eta^2}{4(2v + 1)(v + 1)}\right].
\end{empheq}
Note that \eqref{beta.ov.h.condition2} imposes a more stringent condition on $\beta$ than the one given by \eqref{beta.ov.h.condition}; as a consequence, ensuring convergence in the mean-square sense is a sufficient condition for convergence in the mean sense, \ie $|\alpha_2| < 1$ implies $|\alpha_1| < 1$.

Therefore, $\beta$ must be chosen within the stability range established in \eqref{beta.ov.h.condition2}; however, in practice\footnote{For example, \gls{fifa} \cite{fifa_ranking} uses $\beta\in(0.003,0.04)$ and \gls{fide} \cite{fide} uses $\beta\in(0.01,0.04)$, respectively, in football and chess rankings, which are obtained by scaling the step-size value $\beta'$ provided (by either \gls{fifa} or \gls{fide}) through $\beta = \beta'/s'$ with $s'$ defined in \eqref{scale-ln10}.}, $\beta$ is chosen much smaller than the stability upper-bound we found [see, in Fig.~\ref{fig:stability_limit}, \eqref{beta.ov.h.condition2} as a function of $v$ and $\eta$].


\begin{figure}[h!]
\centering
\includegraphics[scale=1]{figures/stability_limit2.pdf}
\caption{Stability condition \eqref{beta.ov.h.condition2} as a function of $v$ for different values of $\eta$.}%
\label{fig:stability_limit}%
\end{figure}

\cred{\figref{fig:stability_limit} plots the stability conditions \eqref{beta.ov.h.condition} and \eqref{beta.ov.h.condition2} as a function of $v$ for $M = 100$ and different values of $\eta$. -- Which insights could we draw out from \figref{fig:stability_limit}? }



which may be shown as follows:
\begin{align}
|\alpha_1| < 1 &\implies \beta < \frac{M-1}{\ov{h}}\\
|\alpha_2| < 1 &\implies \beta < \frac{\ov{h}}{\ov{h^2}}\\
\frac{\ov{h}}{\ov{h^2}} &\leq \frac{M-1}{\ov{h}}\\
4 \sqrt{\frac{2v + 1}{v + 1}} \exp\left[\frac{\eta^2}{4(v + 1)(2v + 1)}\right] &\leq 4(M - 1) \sqrt{v + 1} \exp\left[\frac{\eta^2}{4(v + 1)}\right]\\
\frac{\sqrt{2v + 1}}{v+1} \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] &\leq M - 1\\
\frac{\sqrt{2v + 1}}{v+1} \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] &\leq \exp\left[ \frac{-v\eta^2}{2(v + 1)(2v + 1)}\right] \leq 1 \leq M - 1
\end{align}
which is true because $v$ is positive and $M \geq 2$.

% \ov{h} = \frac{1}{4} \sqrt{\frac{1}{v + 1}} \exp\left[\frac{-\eta^2}{4(v + 1)}\right]
% \ov{h^2} = \frac{1}{16} \sqrt{\frac{1}{2v + 1}} \exp\left[\frac{-\eta^2}{2(2v + 1)}\right]

% \begin{align}
% \alpha_2 &\leq \alpha_1\\
% \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2}) &\geq \frac{2\beta\ov{h}}{M-1}\\
% 2 (\ov{h} - \beta \ov{h^2}) &\geq \ov{h}\\
% \beta &\leq \frac{1}{2} \frac{\ov{h}}{\ov{h^2}}
% \end{align}


\newpage

\begin{align}
2\beta^2 \ov{h} &< \frac{4Mv}{M-1} \beta (\ov{h} - \beta\ov{h^2})\\
\beta &< \frac{2Mv}{M-1} (1 - \beta\ov{h^2}/\ov{h})\\
\frac{1}{\beta} &> \frac{1-1/M}{2v} \frac{1}{1 - \beta\ov{h^2}/\ov{h}}\\
\frac{1}{\beta} &> \frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}\\
\beta &< \frac{1}{\frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}}
\end{align}
\begin{align}
\ov{d}_0 &> \ov{d}_{\infty}\\
Mv &> \frac{2\beta^2 \ov{h}}{1 - \alpha_2}\\
Mv (1 - \alpha_2) &> 2\beta^2 \ov{h}\\
\frac{4Mv}{M-1} \beta (\ov{h} - \beta\ov{h^2}) &> 2\beta^2 \ov{h}\\
\frac{2Mv}{M-1} (1 - \beta\ov{h^2}/\ov{h}) &> \beta\\
\frac{1-1/M}{2v} \frac{1}{1 - \beta\ov{h^2}/\ov{h}} &< \frac{1}{\beta}\\
\frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}} &< \frac{1}{\beta}\\
\frac{1}{\frac{1-1/M}{2v} + \frac{\ov{h^2}}{\ov{h}}} &> \beta\\
\end{align}
\begin{align}
\alpha_2^k &< 1\\
\alpha_2 &< 1\\
1 - \frac{4}{M-1} \beta (\ov{h} - \beta \ov{h^2}) &< 1\\
\beta (\ov{h} - \beta \ov{h^2}) &> 0\\
\end{align}



% \section*{Checking out Feynman's Technique of Integration (I did something wrong)}

% \url{https://www.youtube.com/watch?v=YO38MCdj-GM}

% \begin{align}
% I(s) &= \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% &= [\sigma(z/s) \mcN(z;\mu_z,v_z)] \Big|_{z=-\infty}^{z=\infty} - \int \mcL(z) \mcN'(z;\mu_z,v_z) \dd z\\
% &= - \int \mcL(z/s) \mcN'(z;\mu_z,v_z) \dd z
% \end{align}

% \begin{align}
% \frac{\dd}{\dd z} \mcL(z/s) &= \mcL'(z/s) = -\frac{1}{s^2} \mcL(z/s) (2 \sigma(z/s) - 1)\\
% \frac{\dd}{\dd s} \mcL(z/s) &= \frac{1}{s} \mcL(z/s) \left[ \frac{z}{s} (2 \sigma(z/s) - 1) - 1 \right]\\
% &= \frac{1}{s^2} \mcL(z/s) (2 \sigma(z/s) - 1) z - \frac{1}{s} \mcL(z/s)\\
% &= - z \mcL'(z/s) - \frac{1}{s} \mcL(z/s)
% \end{align}


% \begin{align}
% \frac{\dd }{\dd s} I(s) &= 
% \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% &= -\int z \mcL'(z/s) \mcN(z;\mu_z,v_z) \dd z - \frac{1}{s} \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% &= -I_2(s) - \frac{1}{s} I(s)\\
% \end{align}

% \begin{align}
% I_2(s) &= \int \mcL'(z/s) z\mcN(z;\mu_z,v_z) \dd z\\
% &= [\mcL(z/s) z\mcN(z;\mu_z,v_z)] \Big|_{z=-\infty}^{z=\infty}\\
% &- \int \mcL(z/s) [z \mcN'(z;\mu_z,v_z) + \mcN(z;\mu_z,v_z)] \dd z\\
% &= - \int \mcL(z/s) z \mcN'(z;\mu_z,v_z) \dd z - \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% &= - \int \mcL(z/s) z \mcN'(z;\mu_z,v_z) \dd z - I(s)\\
% &= - I(s)
% \end{align}

% \begin{align}
% \frac{\dd }{\dd s} I(s) &= \frac{s-1}{s} I(s)\\
% \int \frac{\dd I(s)}{I(s)} &= \int 1 - \frac{1}{s} \dd s\\
% \ln|I(s)| &= s - \ln(s) + c \\
% \ln|I(s)| &= \ln(\e^s/s) + c \\
% I(s) &= c \frac{1}{s} \e^s
% \end{align}

% \begin{align}
% \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z &= c \frac{1}{s} \e^s
% \end{align}

% \begin{align}
% c \frac{1}{s} \e^s &= \int \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% c &= \int s \e^{-s} \mcL(z/s) \mcN(z;\mu_z,v_z) \dd z\\
% &= \int  \frac{\e^{-(z+s^2)/s}}{(1 + \e^{-z/s})^2} \mcN(z;\mu_z,v_z) \dd z
% \end{align}








% \newpage
% \section{\normalfont\it Verification of \eqref{eq:weight-behavior} and \eqref{eq:skill-behavior}}\label{Appendix.C}

% To illustrate this point we show in \figref{fig:fisher_matrix_skills} the  expected skills $\Ex[\theta_{k,m}]$ obtained  using a) the simplified formula \eqref{eq:skill-behavior} (dotted line), b) the approximation \eqref{eq:weight-behavior} (dashed line), and c) the simulations (solid lines), \ie randomly generating $\bx_k$ and $y_k$,  applying the \gls{sg} algorithm \eqref{eq:rating-sgd2}, and averaging the simulation results. We use $\beta=0.1$, $\eta=0.5$, and $\btheta^*=\sqrt{v}\btheta_{\tr{o}}$ with
% \begin{align*}
%     \btheta_\tr{o}=[-1.82, -1.06, -0.84, -0.29,  0.03,  0.06, 0.37, 0.75, 1.16, 1.64]\T,
% \end{align*}
% which satisfies $\bone\T\btheta_{\tr{o}}=0$ and $\frac{1}{M}\|\btheta_{\tr{o}}\|^2=1$. 
% The low-variance case, $v=1$ is shown in \figref{fig:fisher_matrix_skills}a and, the high-variance case, $v=5$ in \figref{fig:fisher_matrix_skills}b.

% % v=1
% % alpha_1: 0.9961924922630578
% % 1 - alpha_1: 0.0038075077369421617

% % v = 5
% % alpha_1: 0.9977554567984103
% % 1 - alpha_1: 0.0022445432015897326

% Since the same adaptation step $\beta$ is used in the examples, the convergence rate, depending on $\beta\ov{h}$ will vary. In fact, for $v=1$ we have $(1-\alpha_1) \approx 3.81 \times 10^{-3}$, while for $v=5$ we calculate $(1-\alpha_1) \approx 2.24 \times 10^{-3}$. This explains why the convergence appears slower in \figref{fig:fisher_matrix_skills}b. More importantly, we see that, despite two-step approximations, \eqref{eq:skill-behavior2} is close to the actual mean and its advantage over \eqref{eq:weight-behavior} is particularly clear for larger $v$.

% We refer to the initial parts of the curves as the \emph{transients} and the last part, as the \emph{steady-state}. Quite obviously, the differences between the approximations appear more clearly in the transient part of the curves.

% \begin{figure}[t!]
% \centering
% \subfloat[]{\includegraphics[scale=1]{figures/fisher_matrix_skills.pdf}}%
% \qquad
% \subfloat[]{\includegraphics[scale=1]{figures/fisher_matrix_skills(high_v).pdf}}%
% \caption{Mean behavior of the skills: obtained by simulations (solid lines), predicted from \eqref{eq:weight-behavior} (dashed lines), and calculated via the approximation \eqref{eq:skill-behavior} (dotted lines); $M = 10$, $\beta = 0.1$, $\eta = 0.5$, and (a) $v = 1$, (b) $v = 5$}%
% \label{fig:fisher_matrix_skills}%
% \end{figure}



%\dz{I noticed $\matH \matH^+ = \matH^+ \matH = 2\matR$, where $\matH^+$ is the Moore-Penrose pseudo-inverse of $\matH$.\\ Also, $\matH = 2 \matH\matR = 2 \matR\matH$.}
%\dz{Alternative formulation:
%\begin{align}
%\matH &= \frac{1}{K} \matX\T \tr{diag}(\bh) \matX
%\end{align}
%where $\matX = [\bx_1, ..., \bx_K]\T$ and $\bh = [h_1, ..., %h_K]\T$. By the way, $\matR = \matX\T \matX / K$, which is also true for a generic scheduling. See %\url{https://web.stanford.edu/class/archive/stats/stats200/stats200.1172/Lecture26.pdf}.
%}
% \dz{whose elements are given by
% \begin{align}
% [\matH]_{m,n} & = 
% \Ex_{\bx_k}[\mcL(\bx_k\T\btheta^*+\eta)x_{k,m} x_{k,n}]\\
% &=\frac{-1}{M(M-1)} 
% \begin{cases}
% 2\mcL(\eta) - \displaystyle\sum_{l=1}^M \mcL(\theta^*_{m}-\theta^*_{l}+\eta)+\mcL(\theta^*_{l}-\theta^*_{m}+\eta), & m = n \\
% \displaystyle \mcL(\theta^*_{m}-\theta^*_{n}+\eta)+\mcL(\theta^*_{n}-\theta^*_{m}+\eta),\quad  &\text{otherwise}.
% \end{cases}
% \end{align}
% }



% $\lim_{k\to\infty}\Ex[\tilde\btheta_{k}] = \bzero$.


% \cred{First of all, we will be able to use the ergodicity argument and approximate the sample statistics of $\btheta^*$ with the average, \ie
% \begin{align}
% \label{ergodicity.argument}
% \Ex_{\theta^*}[f(\theta^*)] \approx \frac{1}{M}\sum_{m=1}^M f(\theta^*_m)
% \end{align}
% which should hold very well for sufficiently large $M$. In particular, we may then assume that
% \begin{align}\label{ergodicity.variance}
% v \approx \frac{1}{M}\sum_{m=1}^M (\theta^*_m)^2.
% \end{align}}

% In this sense, we resort to approximations which may be seen as a reminiscence of the ergodicity condition \eqref{ergodicity.argument} by assuming $\btheta^*$ as a random variable; % and approximate the sample statistics of $\btheta^*$ with the average


% \dz{Using \eqref{eq:rating-sgd2}, we see that the sum of the skills does not change with the time $k$, which is a  \cite[Ch.~5]{Langeville12_book} the well-known property of the Elo algorithm
% \begin{align*}
%     \sum_{m=1}^M\theta_{k+1,m}  &=\bone_M\T\btheta_{k+1}\\
%                                 &= \bone_M\T\btheta_k+\beta [y_k - \sigma(\bx_k\T \btheta_k+\eta)]\bone_M\T\bx_k\\
% %\label{constant.sum}
%                              &= \bone_M\T\btheta_0\\
% \numberthis \label{eq:btheta.0}
%                             & =0,
% \end{align*}
% where we assume all-zero initialization $\btheta_0=\bzero_M$ which yields \eqref{eq:btheta.0}; $\bone_M\in\Real^M$ and $\bzero_M\in\Real^M$ are, respectively, all-ones and all-zeros vectors where, when clear from the context we will abandon the indexing with $M$.}

% \begin{align}
% \label{eq:skill-behavior1}
% % \Ex[\tilde\theta_{k+1,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\tilde\theta_{k,m}]\\
% \Ex[\theta_{k,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\theta_{k-1,m}] + \frac{2 \beta \ov{h}}{M-1} \theta^*_m \\
% % \Ex[\theta_{k,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right)^k (\Ex[\theta_{0,m}] - \Ex[\theta_{\infty,m}]) + \Ex[\theta_{\infty,m}] \\
% % \Ex[\theta_{k,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right)^k (0 - \theta^*_m) + \theta^*_m \\
% %&= (1 - \alpha_1^k)\theta^*_m
% \end{align}
% which reduces to



% and, thus, the most restrictive condition. 

% when an optimal learning rate $\beta_{\tr{opt},K}$ is used, the variance of the skills monotonically decreases with respect to the number of games $K$, that is
% \begin{equation}
% \min_{\beta} \ov{d}_K \, \leq \, \min_{\beta} \ov{d}_{K-1},
% \end{equation}
% and it follows that
% \begin{equation}
% \beta_{{\rm opt}, K} \, \leq \, \beta_{{\rm opt}, K-1}.
% \end{equation}

% Finally, we establish $\beta_{{\rm opt}, 1}$ as the most restrictive condition of the learning rate, since
% \begin{equation}
% \beta_{{\rm opt}, K} \, \leq \, \beta_{{\rm opt}, 1}, \quad \forall K \in \mathbb{N}^*.
% \end{equation}


% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[scale=1]{figures/steady_state.pdf}\\
% 	\caption{Steady-state excess loss as a function of the learning rate $\beta$ for different values of true rating variance $v$. Solid circles indicate the initial excess loss (at $k=0$) for its respective variance.}
% 	\label{fig:steady_state}
% \end{figure}


% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[scale=1]{figures/optimal_eta.pdf}\\
% 	\caption{Optimal $\beta$ with respect to the expected excess loss for a variance $v$ and a different number of games $K$. ($M = 10$).}
% 	\label{fig:optimal_eta}
% \end{figure}






% \input{figures/optimal_eta.pgf}

% \begin{itemize}
% 	\item PLOT $\Tr[\bH_{\infty}\bR]$ AS A FUNCTION OF $\beta$ FOR DIFFERENT VALUES OF $v$
% 	\medskip
	
% 	\item PLOT $\tau$ AS A FUNCTION OF $\tau$ FOR DIFFERENT VALUES OF $v$
% 	\medskip
	
% 	\item DEVELOP RELATION BETWEEN $\beta$ AND $\tau$
% 	\medskip
	
% 	\item IDENTIFY THE OPTIMAL $\beta$ WITH RESPECT TO THE NUMBER OF GAMES $K$ AND $v$

% \end{itemize}



% to  show that , \ie
% \begin{equation}
% \beta_{{\rm o}, K} \,\leq\, \ld \,\leq\, \beta_{{\rm o}, 1}.
% \end{equation}
% In particular, for the special case of $K = 1$, an upper bound can obtained [from \eqref{eq:v_k-final} and \eqref{eq:optimum-beta}] as
% % \begin{align*}
% % \frac{\dd \ov{d}_1}{\dd \beta} &= 0\\
% % \frac{\dd}{\dd \beta} \left[ \alpha_2 (\ov{d}_0 - \ov{d}_\infty) + \ov{d}_\infty \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ \alpha_2 (\ov{d}_0 - \ov{d}_\infty) + \ov{d}_\infty - v_0 \right] &= 0\\
% % \frac{\dd}{\dd \beta} \left[ (1 - \alpha_2) (\ov{d}_\infty - \ov{d}_0) \right] &= 0 \numberthis
% % % \frac{\dd}{\dd \beta} \left[ \ov{h} (M-1) \beta^2 - 2 Mv\ov{h} \beta + 2 Mv \ov{h^2} \beta^2 \right] &= 0\\
% % % \ov{h} (M-1) \beta - Mv\ov{h} + 2 Mv \ov{h^2} \beta  &= 0 \numberthis
% % \end{align*}
% % which yields
% \begin{align}\label{eq:optimum-beta1}
% \beta_{{\rm o}, 1} = \frac{v \ov{h}}{\ov{h} (1-1/M) + 2 v \ov{h^2}}.
% \end{align}
% Note that $\beta_{{\rm o}, 1}$ is half of the upper bound condition on $\beta$ for improvement over initialization [given by \eqref{ineq:improvement.condition}]; likewise, for small values of $v$, \eqref{eq:optimum-beta1} results asymptotically in
% \begin{align}\label{eq:approx-optimum-beta1}
% \beta_{{\rm o}, 1} \approx v.
% \end{align}


% Notice also from this figure that, for small number of games $k$, larger values of $\beta$ should be used in order to obtain the minimum attainable value of $\ov\ell_{\tr{ex},k}$. On the other hand, as the number of games $k$ grows, $\beta$ may be reduced accordingly, since the rating algorithm now has a larger number of games to converge to the optimal solution.


% \dz{Notice also from this figure that, for small number of games $k$, slightly larger values of $\beta$ should be used to improve the convergence speed of the rating algorithm. On the other hand, when the number of games $k$ is large, small values of $\beta$ should be used instead since the rating algorithm has a larger number of games to converge to the optimal solution. }




%\dz{\bf Older version of the subsection below:}

% Since the loss function reflects the uncertainty in the predictions of the game results $y_k$, an expression characterizing its mean behavior is derived here. To this end, let us substitute \eqref{eq:gradient-optimal} and \eqref{eq:hessian-optimal2} into  \eqref{eq:cost-taylor} and take the expected value of both sides of the resulting expression, in such a way that
% \begin{align*}
% \ov\ell_k &= \Ex[\tilde\ell_k(\btheta_k)]\\
% % &= \Ex[\ell_k(\btheta^*)] + \frac{1}{2} \Ex[\tilde\btheta_k\T \matH \tilde\btheta_k]\\
% &= \Ex[\ell_k(\btheta^*)] + \frac{1}{2} \Ex[h_k \tilde\btheta_k\T \bx_k\bx_k\T \tilde\btheta_k].
% \label{eq:loss-behavior0}\numberthis
% \end{align*}
% Note that the first term of the \gls{rhs} of \eqref{eq:loss-behavior0}, which characterizes a lower bound on the mean of the loss function, can be determined as
% \begin{align*}\label{eq:l_min}
% \ov\ell_{\rm min} &= \Ex_{\btheta^*;\bx_k;y_k}[\ell_k(\btheta^*)]\\
% &= \Ex_{\btheta^*;\bx_k;y_k}\{ -y_k \ln[\sigma(\bx_k\T\btheta^* + \eta)] - (1 - y_k) \ln[\sigma(-\bx_k\T\btheta^* + \eta)] \}\\
% &= \Ex_{z_k}\{ -\sigma(z_k + \eta)\ln[\sigma(z_k + \eta)] - \sigma(-z_k + \eta)\ln[\sigma(-z_k + \eta)] \}\\
% &\approx 2\ln(2)\sqrt{2\ln(2)\pi}\ \mcN(\eta;0,2v + 4\ln(2))\\
% &= \ln(2) \sqrt{\frac{2\ln(2)}{v + 2\ln(2)}} \exp{\left[\frac{-\eta^2}{4v + 8\ln(2)}\right]} \numberthis
% \end{align*}
% using the ergodicity argument along with the results shown in \ref{Appendix.Expectation}. In turn, the second term of the \gls{rhs} of \eqref{eq:loss-behavior}, representing the excess-loss due to randomness in $\tilde\btheta_{k}$ caused by the \gls{sg} optimization algorithm, can be obtained from \eqref{eq:expected_value1} and \eqref{eq:theta_R_theta} as
% \begin{align}\label{eq:l_ex}
% \ov\ell_{{\rm ex},k} = \frac{\ov{h}}{M-1} \ov{d}_k
% \end{align}
% which is a linear function of the total variance $\ov{d}_k$ (as derived in Section~\ref{Sec:skills.variance});  hence, results and discussions drawn out from $\ov{d}_k$ hold also to $\ov\ell_{{\rm ex},k}$. So, the mean behavior of the loss function is characterized from \eqref{eq:l_min} and \eqref{eq:l_ex} by
% \begin{empheq}[box={\fboxsep=6pt\fbox}]{align}
% \label{eq:loss-behavior}
% \ov\ell_k &\approx \ov\ell_{\rm min} + \ov\ell_{{\rm ex},k}.
% \end{empheq}




% \begin{align}
% c_2 &= \frac{\ov{d}_k - \ov{d}_\infty}{\ov{d}_\infty}\\
% &= 1 - \alpha_2^k \left( 1 - \frac{\ov{d}_0}{\ov{d}_\infty} \right)\\
% % &= 1 - \alpha_2^k \left( 1 - \frac{M v (1 - \alpha_2)}{2\beta^2\ov{h}} \right)\\
% % &= \alpha_2^k \frac{\ov{d}_0}{\ov{d}_\infty} + (1 - \alpha_2^k)\\
% &= \alpha_2^k (\ov{d}_0/\ov{d}_{\infty} - 1)
% \end{align}

% \begin{align}
% \alpha_2^k (\ov{d}_0 - \ov{d}_\infty) + \ov{d}_\infty &= (1 + c_2) \ov{d}_\infty \\
% \end{align}


% \begin{align}
% % \alpha_2^{K_c} &= \frac{c_2}{\left( \frac{\ov{d}_0}{\ov{d}_\infty} - 1 \right)}\\
% K_c &= \frac{\ln(c_2) - \ln\left( \frac{\ov{d}_0}{\ov{d}_\infty} - 1 \right)}{\ln(\alpha_2)}\\
% &\approx \frac{\ln\left( \frac{\ov{d}_0}{\ov{d}_\infty} - 1 \right) - \ln(c_2)}{1 - \alpha_2}\\
% \end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \begin{equation}
% \begin{aligned}
% \Ex[\tilde\theta_{k+1,m}] &= \Ex[\tilde\theta_{k,m}] - 2 \beta \ov{h} \left( \frac{1}{M} \Ex[\tilde\theta_{k,m}] - \frac{1}{M(M-1)} \sum_{i \neq m}^{M-1} \Ex[\tilde\theta_{k,i}] \right)\\
% &= \Ex[\tilde\theta_{k,m}] - 2 \beta \ov{h} \left( \frac{1}{M-1} \Ex[\tilde\theta_{k,m}] - \frac{1}{M(M-1)} \sum_{i=1}^{M} \Ex[\tilde\theta_{k,i}] \right)\\
% &= \Ex[\tilde\theta_{k,m}] - \frac{2 \beta \ov{h}}{M-1} \left( \Ex[\tilde\theta_{k,m}] - \frac{1}{M} \sum_{i=1}^{M} \Ex[\tilde\theta_{k,i}] \right)\\
% &= \Ex[\tilde\theta_{k,m}] - \frac{2 \beta \ov{h}}{M-1} \Ex[\tilde\theta_{k,m}]\\
% &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\tilde\theta_{k,m}]
% \end{aligned}
% \end{equation}


% \begin{equation}\label{eq:skill-behavior}
% \begin{aligned}
% \Ex[\tilde\theta_{k+1,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\tilde\theta_{k,m}]\\
% \Ex[\theta_{k+1,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right) \Ex[\theta_{k,m}] + \frac{2 \beta \ov{h}}{M-1} \theta^*_m \\
% \Ex[\theta_{0,m}] &= 0\\
% \Ex[\theta_{\infty,m}] &= \theta^*_m\\
% \Ex[\theta_{k,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right)^k (\Ex[\theta_{0,m}] - \Ex[\theta_{\infty,m}]) + \Ex[\theta_{\infty,m}] \\
% \Ex[\theta_{k,m}] &= \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right)^k (0 - \theta^*_m) + \theta^*_m \\
% \Ex[\theta_{k,m}] &=\theta^*_m \left[ 1 - \left( 1 - \frac{2 \beta \ov{h}}{M-1} \right)^k \right] \\
% \end{aligned}
% \end{equation}




% \begin{align}
% [\matH]_{m,n} &= \frac{-1}{M(M-1)} 
% \begin{cases}
% 2\mcL(\eta) - \displaystyle\sum_{l=1}^M \mcL(\theta^*_{m}-\theta^*_{l}+\eta)+\mcL(\theta^*_{l}-\theta^*_{m}+\eta), & m = n \\
% \displaystyle \mcL(\theta^*_{m}-\theta^*_{n}+\eta)+\mcL(\theta^*_{n}-\theta^*_{m}+\eta),\quad  &\text{otherwise}.
% \end{cases}\\
% [\matH']_{m,n} &= \frac{1}{M(M-1)} [ \mcL(\theta^*_{m}-\theta^*_{n}+\eta)+\mcL(\theta^*_{n}-\theta^*_{m}+\eta) ]\\
% \matH &=  \tr{diag}(\matH' \bone) - \matH'
% \end{align}




%************************************************************************************



% (COMMENT) INCLUDE THE DERIVATION SHOWING THE ALGORITHM'S STABILITY LIMIT FOR $\beta$ STARTING FROM $\alpha$ (FOR THE LINEARIZED ALGORITHM)
% \begin{equation}
% 	\begin{aligned}
% 		\alpha &< 1\\
% 		1 - \frac{4}{M-1} \beta(\ov{h} - \beta \ov{h^2}) &< 1\\
% 		\beta(\beta \ov{h^2} - \ov{h}) &< 0\\
% 		0 < \beta &< \frac{\ov{h}}{\ov{h^2}}\\
% 	\end{aligned}
% \end{equation}




% To characterize the mean behavior of the skills, we start rewriting \eqref{eq:sgd-taylor.2} in terms of the skills estimation error
% \begin{align}
% \label{tilde.btheta}
%     \tilde\btheta_k &= \btheta_k - \btheta^*
% \end{align}
% as
% \begin{align}\label{eq:param-error}
% \tilde\btheta_{k+1} &= 
% (\matI - \beta h_k \bx_k\bx_k\T) \tilde\btheta_k + \beta g_k \bx_k .
% \end{align}

% Then, taking the expected value of both sides of \eqref{eq:param-error}, one has
